A coherent full microwave scattering formulation for random layered media

We present a fully coherent, analytic model of the backscattering intensity in all HH, HV, VH and VV channels, for the volume scattering of radiation from a layer of finite thickness, such as a vegetation layer over bare soil. We aim for a simple, not numerically intensive model which could be used either as forward model in a Bayesian estimation scheme, or else as a preliminary means to identify key features of a concrete problem, for its further analysis by more sophisticated theoretical and numerical approaches.

==> Sections/not_used/H_alpha.tex <==
\section{The $\left(H,\alpha\right)$ analysis}
Given the incident field
\be
\mathbf{E}_I=\left(\begin{array}{c}E_H\\E_V\end{array}\right)
\te
The scattered field is related to the incident field through the scattering matrix
\be
\mathbf{E}_S=\mathbf{S}\mathbf{E}_I
\te
Explicitly
\be
\mathbf{S}=\left(\begin{array}{cc}S_{HH}&S_{HV}\\S_{VH}&S_{VV}\end{array}\right)
\te
or else introducing the Pauli matrices
\bea
\sigma_0&=&\frac1{\sqrt{2}}\left(\begin{array}{cc}1&0\\0&1\end{array}\right);\;\;\sigma_1=\frac1{\sqrt{2}}\left(\begin{array}{cc}0&1\\1&0\end{array}\right)\nn
\sigma_2&=&\frac1{\sqrt{2}}\left(\begin{array}{cc}0&-i\\i&0\end{array}\right);\;\;\sigma_3=\frac1{\sqrt{2}}\left(\begin{array}{cc}1&0\\0&-1\end{array}\right)
\tea
which obey
\be
\sigma_i\sigma_j=\frac12\delta_{ij}\mathbf{1}+\frac  i{\sqrt{2}}\epsilon_{ijk}\sigma_k
\te
we may introduce the Stokes representation ($\mu=0-3$)
\be
\mathbf{S}=k^{\mu}\sigma_{\mu}
\te
where
\be
k^{\mu}=\mathrm{tr}\;\sigma_{\mu}\mathbf{S}
\te
Explicitly
\be
k^{\mu}=\frac1{\sqrt{2}}\left(\begin{array}{c}S_{HH}+S_{VV}\\S_{VH}+S_{HV}\\i\left(S_{VH}-S_{HV}\right)\\S_{HH}-S_{VV}\end{array}\right)
\label{k4}
\te
So the scattered covariance matrix is
\bea
\mathbf{J}&=&\left\langle \mathbf{S}\mathbf{E}_I\mathbf{E}^{\dagger}_I\mathbf{S}^{\dagger}\right\rangle\nn
&=& \left\langle k^{\mu}k^{\nu*}\right\rangle \sigma_{\mu}\mathbf{E}_I\mathbf{E}^{\dagger}_I\sigma_{\nu}
\tea
The Hermitian matrix $\left\langle k^{\mu}k^{\nu*}\right\rangle$ may be written in terms of its eigenvectors
\be
\left\langle k^{\mu}k^{\nu*}\right\rangle =\sum_{a=1}^4\lambda_au_a^{\mu}u_a^{\nu*}
\te
where $u_a^{\mu}u_{b\nu}^*=\delta_{ab}$. Better still, define
\be
\lambda=\sum_{a=1}^4\lambda_a 
\te
\be
p_a=\frac{\lambda_a}{\lambda}
\te
Then
\be
\mathbf{J}=\sum_{a=1}^4p_a \mathbf{J}_a
\te
where
\be
\mathbf{J}_{a}=\mathbf{S}_a\mathbf{E}_I\mathbf{E}^{\dagger}_I\mathbf{S}^{\dagger}_a
\te
and
\be
\mathbf{S}_a=\sqrt{\lambda}\;u_a^{\mu}\sigma_{\mu}
\te
In this way we come to see the scattering process as an incoherent superposition of four ``scattering modes'', each characterized by the scattering matrix $\mathbf{S}_a$. In particular, for each mode we have
\be
\left(S_{HH}+S_{VV}\right)_a=\mathrm{tr}\;\mathbf{S}_a=\sqrt{2\lambda}\;u_a^{0}
\te
We define the angle $\alpha_a$ from
\be
\cos\alpha_a=\left|u_a^{0}\right|,
\te
the average angle
\be
\alpha=\sum_{a=1}^4p_a\alpha_a,
\te
and the entropy
\be
H=-\sum_{a=1}^4p_a\ln p_a
\te
It is an empirical fact that the position of a given scattering process in the $\left(H,\alpha\right)$ plane conveys relevant information about its nature.

In special cases where $S_{HV}=S_{VH}$ we can see from eq. (\ref{k4}) that $k^2\equiv 0$ and so the matrix $\left\langle k^{\mu}k^{*\nu}\right\rangle$ is missing a whole row and column. It thereby has a null eigenvalue. The null eigenvalue and its corresponding eigenvector do not contribute either to the entropy or to $\alpha$, so they may be disregarded, leaving open the diagonalization of the remaining $3\times 3$ block only.

\section{Perturbative evaluation of $\left(H,\alpha\right)$}
We now consider the above analysis in the context of the perturbative evaluation of the scattering matrix. We shall restrict ourselves to the backscattering case where $S_{HH,VV}=S^{\left(1\right)}_{HH,VV}+S^{\left(2\right)}_{HH,VV}$ have both first and second order contributions, while $S_{HV,VH}=S^{\left(2\right)}_{HV,VH}$ appears only to second order. 


\subsection{Lowest order theory}
The lowest order the $\mathbf{K}^{\left(2\right)}$ matrix takes the form

\be
\mathbf{K}^{\left(2\right)}=\frac12\left(\begin{array}{cccc}\left\langle \left|S^{\left(1\right)}_{HH}+S^{\left(1\right)}_{VV}\right|^2\right\rangle&0&0&\left\langle \left(S^{\left(1\right)}_{HH}+S^{\left(1\right)}_{VV}\right)\left(S^{\left(1\right)*}_{HH}-S^{\left(1\right)*}_{VV}\right)\right\rangle\\0&0&0&0\\0&0&0&0\\\left\langle \left(S^{\left(1\right)}_{HH}-S^{\left(1\right)}_{VV}\right)\left(S^{\left(1\right)*}_{HH}+S^{\left(1\right)*}_{VV}\right)\right\rangle&0&0&\left\langle \left|S^{\left(1\right)}_{HH}-S^{\left(1\right)}_{VV}\right|^2\right\rangle\end{array}\right)
\te
It therefore has a degenerate null block spanned by the vectors $u_2^{\left(2\right)}=\left(0,1,0,0\right)$ and $u_3^{\left(2\right)}=\left(0,0,1,0\right)$. This block does not contribute either to $H$ or $\alpha$.

The trace 
\be
K^{\left(2\right)}=K^{\left(2\right)11}+K^{\left(2\right)44}=\left\langle \left|S^{\left(1\right)}_{HH}\right|^2+\left|S^{\left(1\right)}_{VV}\right|^2\right\rangle
\te
We also define
\be
\tilde K^{\left(2\right)}=K^{\left(2\right)11}-K^{\left(2\right)44}=\left\langle \left(S^{\left(1\right)}_{HH}S^{\left(1\right)*}_{VV}+S^{\left(1\right)*}_{HH}S^{\left(1\right)}_{VV}\right)\right\rangle
\te
and
\be
\Lambda=\frac{2K^{\left(2\right)14}}{\tilde K^{\left(2\right)}}
\te
We then may write
\be
\mathbf{K}^{\left(2\right)}=\frac12\left(\begin{array}{cccc}\left(K^{\left(2\right)}+\tilde K^{\left(2\right)}\right)&0&0&\tilde K^{\left(2\right)}\Lambda\\0&0&0&0\\0&0&0&0\\\tilde K^{\left(2\right)}\Lambda^{*}&0&0&\left(K^{\left(2\right)}-\tilde K^{\left(2\right)}\right)\end{array}\right)
\te
The two nonzero eigenvalues are
\be
\lambda^{\left(2\right)}_{1,4}=\frac12\left[K^{\left(2\right)}\pm\tilde K^{\left(2\right)}\sqrt{1+\left|\Lambda\right|^2}\right]
\te
The $u_{1,4}^{\left(2\right)}$ eigenvectors obey
\be
u_{1,4}^{\left(2\right)4}=\frac{\Lambda^*}{1\pm\sqrt{1+\left|\Lambda\right|^2}}u_{1,4}^{\left(2\right)1}
\te
With the normalization
\be
\left|u_{1,4}^{\left(2\right)1}\right|^2+\left|u_{1,4}^{\left(2\right)4}\right|^2=1
\te
we get
\be
\cos\alpha^{\left(2\right)}_{1,4}=\frac1{\sqrt{2}}\sqrt{1\pm\frac1{\sqrt{1+\left|\Lambda\right|^2}}}
\te
Observe that
\be
\sin\alpha^{\left(2\right)}_{1,4}=\cos\alpha^{\left(2\right)}_{4,1}
\label{sineqcos}
\te
and therefore
\be
\alpha^{\left(2\right)}_{4}=\frac{\pi}2-\alpha^{\left(2\right)}_{1}
\label{complementarity}
\te
The weights
\be
p^{\left(2\right)}_{1,4}=\frac12\left[1\pm p^{\left(2\right)}\right]
\te
where
\be
p^{\left(2\right)}=\frac{\tilde K^{\left(2\right)}}{K^{\left(2\right)}}\sqrt{1+\left|\Lambda\right|^2}
\te
Therefore
\be
H^{\left(2\right)}=\ln 2-\frac12\left[\left(1+p^{\left(2\right)}\right)\ln\left(1+p^{\left(2\right)}\right)+\left(1-p^{\left(2\right)}\right)\ln\left(1-p^{\left(2\right)}\right)\right]
\te
while
\be
\alpha^{\left(2\right)}=\frac{\pi}4\left(1-p^{\left(2\right)}\right)+p^{\left(2\right)}\alpha^{\left(2\right)}_{1}
\te


\section{First order corrections}
We now want to include the first order corrections, whereby
\be
S_{XY}=S_{XY}^{\left(1\right)}+S_{XY}^{\left(2\right)}
\te

\be
\mathbf{K}=\mathbf{K}^{\left(2\right)}+\mathbf{K}^{\left(4\right)}
\te
{\tiny
\bea
&&\mathbf{K}^{\left(4\right)}=\frac12\nn
&&\left(\begin{array}{cccc}\left\langle \left|S^{\left(2\right)}_{HH}+S^{\left(2\right)}_{VV}\right|^2\right\rangle
&\left\langle \left(S^{\left(2\right)}_{HH}+S^{\left(2\right)}_{VV}\right)\left(S^{\left(2\right)*}_{HV}+S^{\left(2\right)*}_{VH}\right)\right\rangle
&\left\langle \left(S^{\left(2\right)}_{HH}+S^{\left(2\right)}_{VV}\right)\left(-i\right)\left(S^{\left(2\right)*}_{HV}-S^{\left(2\right)*}_{VH}\right)\right\rangle
&\left\langle \left(S^{\left(2\right)}_{HH}+S^{\left(2\right)}_{VV}\right)\left(S^{\left(2\right)*}_{HH}-S^{\left(2\right)*}_{VV}\right)\right\rangle\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\left\langle \left(S_{VH}^{\left(2\right)}+S_{HV}^{\left(2\right)}\right)\left(S^{\left(2\right)*}_{HH}+S^{\left(2\right)*}_{VV}\right)\right\rangle
&\left\langle \left|S_{VH}^{\left(2\right)}+S_{HV}^{\left(2\right)}\right|^2\right\rangle
&\left\langle \left(S_{VH}^{\left(2\right)}+S_{HV}^{\left(2\right)}\right)\left(-i\right)\left(S^{\left(2\right)*}_{HV}-S^{\left(2\right)*}_{VH}\right)\right\rangle
&\left\langle \left(S_{VH}^{\left(2\right)}+S_{HV}^{\left(2\right)}\right)\left(S^{\left(2\right)*}_{HH}-S^{\left(2\right)*}_{VV}\right)\right\rangle\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\left\langle \left(i\right)\left(S_{VH}^{\left(2\right)}-S_{HV}^{\left(2\right)}\right)\left(S^{\left(2\right)*}_{HH}+S^{\left(2\right)*}_{VV}\right)\right\rangle
&\left\langle \left(i\right)\left(S_{VH}^{\left(2\right)}-S_{HV}^{\left(2\right)}\right)\left(S^{\left(2\right)*}_{HV}+S^{\left(2\right)*}_{VH}\right)\right\rangle
&\left\langle \left|S_{VH}^{\left(2\right)}-S_{HV}^{\left(2\right)}\right|^2\right\rangle
&\left\langle \left(i\right)\left(S_{VH}^{\left(2\right)}-S_{HV}^{\left(2\right)}\right)\left(S^{\left(2\right)*}_{HH}-S^{\left(2\right)*}_{VV}\right)\right\rangle\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\left\langle \left(S^{\left(2\right)}_{HH}-S^{\left(2\right)}_{VV}\right)\left(S^{\left(2\right)*}_{HH}+S^{\left(2\right)*}_{VV}\right)\right\rangle&
\left\langle \left(S^{\left(2\right)}_{HH}-S^{\left(2\right)}_{VV}\right)\left(S^{\left(2\right)*}_{HV}+S^{\left(2\right)*}_{VH}\right)\right\rangle&
\left\langle \left(S^{\left(2\right)}_{HH}-S^{\left(2\right)}_{VV}\right)\left(-i\right)\left(S^{\left(2\right)*}_{HV}-S^{\left(2\right)*}_{VH}\right)\right\rangle&
\left\langle \left|S^{\left(2\right)}_{HH}-S^{\left(2\right)}_{VV}\right|^2\right\rangle\end{array}\right)
\tea
}
Because the lowest order matrix $\mathbf{K}^{\left(2\right)}$ is degenerate, it is convenient to adopt a Brillouin-Wigner type perturbation scheme, rather than a Rayleigh-Schr\"odinger one. This works as follows.

We want to solve 
\be
\left(\mathbf{K}^{\left(2\right)}+\mathbf{K}^{\left(4\right)}\right)^{\mu\nu}u_{a\nu}=\lambda_au_a^{\mu}
\label{seq}
\te
We write (we leave the normalization for later)
\be
u_a^{\mu}=u_a^{\left(2\right)\mu}+u_a^{\left(4\right)\mu}
\te
where $u_a^{\left(2\right)\mu}$ is the corresponding eigenvector of the unperturbed matrix $\mathbf{K}^{\left(2\right)}$, and
\be
u_a^{\left(4\right)\mu}=\sum_{b\not= a}c_{ab}u_b^{\left(2\right)\mu}
\te
So, writing eq. (\ref{seq}) as
\be
\left(\mathbf{K}^{\left(2\right)}-\lambda_a\mathbf{1}\right)^{\mu\nu}u_{a\nu}=-\mathbf{K}^{\left(4\right)\mu\nu}u_{a\nu}
\label{seq2}
\te
and
\be
\lambda_a=\lambda_a^{\left(2\right)}+\lambda_a^{\left(4\right)}
\te
we get, contracting eq. (\ref{seq2}) with each unperturbed eigenvector
\bea
c_{ab}&=&\frac{\mathbf{K}^{\left(4\right)\mu\nu}u_{b\mu}^{\left(2\right)*}u_{a\nu}}{\lambda^{\left(2\right)}_a-\lambda_b^{\left(2\right)}+\lambda_a^{\left(4\right)}}\nn
\lambda_a^{\left(4\right)}&=&\mathbf{K}^{\left(4\right)\mu\nu}u_{a\mu}^{\left(2\right)*}u_{a\nu}
\label{WB}
\tea
Equations (\ref{WB}) are meant to be solved iteratively in $u_{a\nu}$. We shall only consider the first iteration, where we approximate $u_{a\nu}=u_{a\nu}^{\left(2\right)}$ in the right hand side. 

\subsection{The change in the entropy}
We want to see how the first order correction modifies the entropy. The sum of the eigenvalues gives
\be
\sum_{a=1}^4\lambda_a=K^{\left(2\right)}+K^{\left(4\right)}
\te
where
\be
K^{\left(4\right)}=\left\langle \left|S^{\left(2\right)}_{HH}\right|^2+\left|S^{\left(2\right)}_{VV}\right|^2+\left|S^{\left(2\right)}_{VH}\right|^2+\left|S^{\left(2\right)}_{HV}\right|^2\right\rangle
\te
and so the weights
\bea
p_a&=&\frac{\lambda_a^{\left(2\right)}+\lambda_a^{\left(4\right)}}{K^{\left(2\right)}+K^{\left(4\right)}}\nn
&=&p_a^{\left(2\right)}+p_a^{\left(4\right)}
\tea
where
\be
p_a^{\left(4\right)}=\frac{\lambda_a^{\left(4\right)}}{K^{\left(2\right)}}-p_a^{\left(2\right)}\frac{K^{\left(4\right)}}{K^{\left(2\right)}}
\te
as expected
\be
\sum_{a=1}^4p_a^{\left(4\right)}=0
\te
We now get
\bea
H&=&-\left(p_1^{\left(2\right)}+p_1^{\left(4\right)}\right)\ln\left(p_1^{\left(2\right)}+p_1^{\left(4\right)}\right)-\left(p_4^{\left(2\right)}+p_4^{\left(4\right)}\right)\ln\left(p_4^{\left(2\right)}+p_4^{\left(4\right)}\right)-p_2^{\left(4\right)}\ln p_2^{\left(4\right)}-p_3^{\left(4\right)}\ln p_3^{\left(4\right)}\nn
&=&H^{\left(2\right)}+H^{\left(4\right)}
\tea
where
\be
H^{\left(4\right)}=-p_1^{\left(4\right)}\ln p_1^{\left(2\right)}-p_4^{\left(4\right)}\ln p_4^{\left(2\right)}-p_2^{\left(4\right)}\left(\ln p_2^{\left(4\right)}-1\right)-p_3^{\left(4\right)}\left(\ln p_3^{\left(4\right)}-1\right)
\te

\subsection{The change in $\alpha$}
As in the previous considerations, the idea is to write
\be
\alpha_a=\alpha_a^{\left(2\right)}+\alpha_a^{\left(4\right)}
\te
and then
\bea
\alpha&=&\sum_{a=1}^4p_a\alpha_a\nn
&=&\alpha^{\left(2\right)}+\sum_{a=1}^4\left(p^{\left(2\right)}_a\alpha^{\left(4\right)}_a+p^{\left(4\right)}_a\alpha^{\left(2\right)}_a\right)
\tea
We see that $\alpha_2^{\left(4\right)}$ and $\alpha_3^{\left(4\right)}$ do not appear in this expression. Also, use eq. (\ref{complementarity}) and that
\be
\alpha^{\left(2\right)}_2=\alpha^{\left(2\right)}_3=\frac{\pi}2
\te
to get
\be
\sum_{a=1}^4p^{\left(4\right)}_a\alpha^{\left(2\right)}_a=\left(p^{\left(4\right)}_1-p^{\left(4\right)}_4\right)\alpha^{\left(2\right)}_1-p^{\left(4\right)}_1\frac{\pi}2
\te
To compute $\alpha_1^{\left(4\right)}$ and $\alpha_4^{\left(4\right)}$ observe that the eigenvectors we have defined in the previous section are well normalized to first order. So we have
\be
\cos\left(\alpha_1^{\left(2\right)}+\alpha_1^{\left(4\right)}\right)=\cos\alpha_1^{\left(2\right)}+\frac{\mathbf{K}^{\left(4\right)\mu\nu}u_{4\mu}^{\left(2\right)*}u_{1\nu}}{\tilde K^{\left(2\right)}\sqrt{1+\left|\Lambda\right|^2}}\cos\alpha_4^{\left(2\right)}
\te
where we have neglected $\lambda_1^{\left(4\right)}$ in the denominator in the second term, as it gives a higher order contribution. Expanding the left hand side and using eq. (\ref{sineqcos}) we get
\be
\alpha_1^{\left(4\right)}=-\frac{\mathbf{K}^{\left(4\right)\mu\nu}u_{4\mu}^{\left(2\right)*}u_{1\nu}^{\left(2\right)}}{\tilde K^{\left(2\right)}\sqrt{1+\left|\Lambda\right|^2}}
\label{a14}
\te
In the same way
\be
\alpha_4^{\left(4\right)}=\frac{\mathbf{K}^{\left(4\right)\mu\nu}u_{1\mu}^{\left(2\right)*}u_{4\nu}^{\left(2\right)}}{\tilde K^{\left(2\right)}\sqrt{1+\left|\Lambda\right|^2}}
\label{a44}
\te
It is remarkable that $S_{HV}$ and $S_{VH}$ do not appear in eqs. (\ref{a14}) and (\ref{a44}). Actually, the conclusion is that only $\mathbf{K}^{\left(4\right)11},\mathbf{K}^{\left(4\right)14},\mathbf{K}^{\left(4\right)22},\mathbf{K}^{\left(4\right)33},\mathbf{K}^{\left(4\right)41}$ and $\mathbf{K}^{\left(4\right)44}$ are necessary to compute the corrections to $H$ and $\alpha$.

==> Sections/not_used/basics.tex <==
\section{Basic Maxwell}
Maxwell equations with $\mu=1$ and position dependent $\epsilon$ \cite{calzetta2008nonequilibrium}

\bea 
\nabla\epsilon\mathbf{E}&=&0\nn
\nabla\mathbf{B}&=&0\nn
\nabla\times\mathbf{E}-i\frac{\omega}{c}\mathbf{B}&=&0\nn
\nabla\times\mathbf{B}+i\epsilon\frac{\omega}{c}\mathbf{E}&=&0
\tea
so 

\be 
\nabla\times\nabla\times\mathbf{E}-\epsilon\left(\frac{\omega}{c}\right)^2\mathbf{E}=0
\te 
but

\be 
\nabla\times\nabla\times\mathbf{E}=-\mathbf{\Delta}\mathbf{E}+\nabla\left(\nabla\mathbf{E} \right) 
\te
So

\be 
\mathbf{\Delta}\mathbf{E}-\nabla\left(\nabla\mathbf{E} \right) +\epsilon\left(\frac{\omega}{c}\right)^2\mathbf{E}=0
\te 
 Decomposing into cartesian coordinates we get

\bea
\left(\frac {\partial^2}{\partial z^2}+\frac {\partial^2}{\partial y^2}\right)E_x-\frac {\partial}{\partial x}\left(\frac {\partial E_y}{\partial y}+\frac {\partial E_z}{\partial z}\right) +\epsilon \left(\frac{\omega}{c}\right)^2E_x&=&0\nn
\left(\frac {\partial^2}{\partial z^2}+\frac {\partial^2}{\partial x^2}\right)E_y-\frac {\partial}{\partial y}\left(\frac {\partial E_x}{\partial x}+\frac {\partial E_z}{\partial z}\right) +\epsilon \left(\frac{\omega}{c}\right)^2E_y&=&0\nn
\left(\frac {\partial^2}{\partial x^2}+\frac {\partial^2}{\partial y^2}\right)E_z-\frac {\partial}{\partial z}\left(\frac {\partial E_x}{\partial x}+\frac {\partial E_y}{\partial y}\right) +\epsilon \left(\frac{\omega}{c}\right)^2E_z&=&0
\tea





Let us first consider the case where $\epsilon=\epsilon\left(z\right)$.
We look for solutions of the form $e^{i\vec{p}\vec{x}}\mathbf{E}_{\vec{p}}$, $\vec x=\left(x,y\right)$, $\vec p=\left(p_x,p_y\right)$. We call $\mathbf{E}_{\vec{p}}=\left(E_{\vec p},E_{\vec{p}z}\right)$ where further $E_{\vec p}=\left(E_{\vec{p}x},E_{\vec{p}y}\right)$

\bea
\left(\frac {\partial^2}{\partial z^2}-p_y^2\right)E_{\vec{p}x}-ip_x\left(ip_yE_{\vec{p}y}+\frac {\partial E_{\vec{p}z}}{\partial z}\right) +\epsilon \left(\frac{\omega}{c}\right)^2E_{\vec{p}x}&=&0\nn
\left(\frac {\partial^2}{\partial z^2}-p_x^2\right)E_{\vec{p}y}-ip_y\left(ip_xE_{\vec{p}x}+\frac {\partial E_{\vec{p}z}}{\partial z}\right)+\epsilon \left(\frac{\omega}{c}\right)^2E_{\vec{p}y}&=&0\nn
-i\frac {\partial}{\partial z}\left(\vec{p}\vec{E}_{\vec{p}}\right) +\left(\epsilon \left(\frac{\omega}{c}\right)^2-p^2\right)E_{\vec{p}z}&=&0
\tea
$\vec{E}_{\vec{p}}$ can be decomposed into $H$ polarized modes where $\mathbf{E}_{H\vec{p}}=\left(\mathbf{K}\times\hat{p}\right)\varphi\left(z\right)$ and $V$ polarized modes where $\vec{E}_{V\vec{p}}=\hat{p}\psi\left(z\right)$, where $\hat{p}=\vec{p}/p$. For the $H$ modes $E_{H\vec{p}z}=\vec{p}\vec{E}_{H\vec{p}}=0$ and 

\be
\frac {\partial^2}{\partial z^2}\varphi +P^2\varphi =0
\label{KG}
\te
$P^2=\epsilon \left(\frac{\omega}{c}\right)^2-p^2$. For the $V$ modes 

\be
E_z=\frac{ip}{P^2}\frac {\partial\psi}{\partial z}
\te
and 

\be
\frac {\partial^2\psi}{\partial z^2}+\frac {\partial}{\partial z}\frac{p^2}{P^2}\frac {\partial\psi}{\partial z} +\epsilon \left(\frac{\omega}{c}\right)^2\psi=0
\label{KGV}
\te


\section{Matching conditions}
Let us consider the case where $\epsilon$ is piece-wise constant, with a discontinuity at $z=-h$. For the $H$ modes the matching conditions are just that $\varphi$ and $\varphi'$ are continuous accross the interface. Let us write

\be
\varphi=\frac 1{\sqrt{2P_{\alpha}}}\left[A_{\alpha}e^{-iP_{\alpha}z}+B_{\alpha}e^{iP_{\alpha}z}\right]
\te
where $\alpha =>\left(<\right)$ above (below) the interface. Then we get

\be 
\left( \begin{array}{cc}
\frac{e^{-iP_<h}}{\sqrt{P_<}} & \frac{e^{iP_<h}}{\sqrt{P_<}} \\
\sqrt{P_<}e^{-iP_<h}          & -\sqrt{P_<}e^{iP_<h}
\end{array}\right) \left( 
\begin{array}{c}
A_< \\
B_<
\end{array}\right)  =
\left( \begin{array}{cc}
\frac{e^{-iP_>h}}{\sqrt{P_>}} & \frac{e^{iP_>h}}{\sqrt{P_>}} \\
\sqrt{P_>}e^{-iP_>h}          & -\sqrt{P_>}e^{iP_>h}
\end{array}\right) \left( 
\begin{array}{c}
A_> \\
B_>
\end{array}\right)
\te
For $V$ modes we get that $\psi$ and $\epsilon E_z$ are continuous, so

\be 
\left(1+\frac{p^2}{P^2}\right)\psi'= \left(\frac{\omega}{c}\right)^2\frac{\epsilon}{P^2}\psi'
\te
must also be continuous. Above and below the interface, we write 

\be
\psi=\sqrt{\frac {P_{\alpha}}{2\epsilon_{\alpha} \left(\frac{\omega}{c}\right)^2}}\left[A_{\alpha}e^{-iP_{\alpha}z}+B_{\alpha}e^{iP_{\alpha}z}\right]
\te
therefore 

\be
E_z=\frac {p}{\sqrt{2P_{\alpha}\epsilon_{\alpha} \left(\frac{\omega}{c}\right)^2}}\left[A_{\alpha}e^{iP_{\alpha}z}-B_{\alpha}e^{-iP_{\alpha}z}\right]
\te
and

\be 
\left( \begin{array}{cc}
\sqrt{\frac{P_<}{\epsilon_<}}{e^{-iP_<h}} &\sqrt{\frac{P_<}{\epsilon_<}}{e^{iP_<h}} \\
\sqrt{\frac{\epsilon_<}{P_<}}{e^{-iP_<h}} & -\sqrt{\frac{\epsilon_<}{P_<}}{e^{iP_<h}} 
\end{array}\right) \left( 
\begin{array}{c}
A_< \\
B_<
\end{array}\right)  =
\left( \begin{array}{cc}
\sqrt{\frac{P_>}{\epsilon_>}}{e^{-iP_>h}} &\sqrt{\frac{P_>}{\epsilon_>}}{e^{iP_>h}} \\
\sqrt{\frac{\epsilon_>}{P_>}}{e^{-iP_>h}} & -\sqrt{\frac{\epsilon_>}{P_>}}{e^{iP_>h}} 
\end{array}\right) \left( 
\begin{array}{c}
A_> \\
B_>
\end{array}\right)
\te
and then the matching conditions for the derivatives follow.

\section{Green functions}
The Green functions are the solutions to
\bea
\left[\frac {\partial^2}{\partial z^2}+P^2\right]G_{H\vec p}\left(z,z'\right) &=&-\delta\left(z-z'\right)\nn
\left[\frac {\partial^2}{\partial z^2}+\frac {\partial}{\partial z}\frac{p^2}{P^2}\frac {\partial}{\partial z} +\epsilon \left(\frac{\omega}{c}\right)^2\right]G_{V\vec p}\left(z,z'\right) &=&-\delta\left(z-z'\right)
\tea
with outgoing boundary conditions; they obey the reciprocity condition

\be
G_{\left(H,V\right) \vec{p}}\left(z,z'\right)=G_{\left(H,V\right) \left(-\vec{p}\right)}\left(z',z\right)
\te
which, since by rotation symmetry $G_{\left(H,V\right) \vec{p}}\left(z,z'\right)=G_{\left(H,V\right) {p}}\left(z,z'\right)$, reduces to symmetry under the exchange of $z$ and $z'$. Therefore

\be
G_{\left(H,V\right) \vec{p}}\left(z,z'\right)=iF^{UP}_{\left(H,V\right)p}\left(z_>\right)F^{DOWN}_{\left(H,V\right)p}\left(z_<\right)
\te
The $UP$ ($DOWN$) modes are purely outgoing solutions normalized to unit Wronskian. For $H$ modes the Wronskian of two solutions is 
\be
W_{H1,2}=\left(-i\right)\left[\varphi_2\varphi'_1-\varphi_1\varphi'_2\right]
\te
We have
\bea
F^{UP}_{HpI}&=&\frac {1}{\sqrt{2P_{I}}}e^{iP_{I}z}\nn
F^{UP}_{HpII}&=&\frac {1}{\sqrt{2P_{II}}}\left[r^{UP}_{HpII}e^{iP_{II}z}+t^{UP}_{HpII}e^{-iP_{II}z}\right]\nn
F^{UP}_{HpIII}&=&\frac {1}{\sqrt{2P_{III}}}\left[\frac1{t^{DOWN}_{HpIII}}e^{iP_{III}z}+t^{UP}_{HpIII}e^{-iP_{III}z}\right]
\tea

\bea
F^{DOWN}_{HpI}&=&\frac {1}{\sqrt{2P_{I}}}\left[r^{DOWN}_{HpI}e^{iP_{I}z}+e^{-iP_{I}z}\right]\nn
F^{DOWN}_{HpII}&=&\frac {1}{\sqrt{2P_{II}}}\left[r^{DOWN}_{HpII}e^{iP_{II}z}+t^{DOWN}_{HpII}e^{-iP_{II}z}\right]\nn
F^{DOWN}_{HpIII}&=&\frac {1}{\sqrt{2P_{III}}}t^{DOWN}_{HpIII}e^{-iP_{III}z}
\tea
For $V$ modes the Wronskian of two solutions is defined as

\be
W_{V1,2}=\left(-i\right)\left[1+\frac{p^2}{P^2}\right]\left\{\psi'_1\psi_2-\psi_1\psi'_2\right\}=\left(-i\right) \left(\frac{\omega}{c}\right)^2\frac{\epsilon_0}{P^2}\left\{\psi'_1\psi_2-\psi_1\psi'_2\right\}
\te
so 

\bea
F^{UP}_{VpI}&=&\sqrt{\frac{P_{I}}{2\epsilon_{0I} \left(\frac{\omega}{c}\right)^2}}e^{iP_{I}z}\nn
F^{UP}_{VpII}&=& \sqrt{\frac{P_{II}}{2\epsilon_{0II} \left(\frac{\omega}{c}\right)^2}}\left[r^{UP}_{VpII}e^{iP_{II}z}+t^{UP}_{VpII}e^{-iP_{II}z}\right]\nn
F^{UP}_{VpIII}&=& \sqrt{\frac{P_{III}}{2\epsilon_{0III} \left(\frac{\omega}{c}\right)^2}}\left[\frac1{t^{DOWN}_{VpIII}}e^{iP_{III}z}+t^{UP}_{VpIII}e^{-iP_{III}z}\right]
\tea

\bea
F^{DOWN}_{VpI}&=&\sqrt{\frac{P_{I}}{2\epsilon_{0I} \left(\frac{\omega}{c}\right)^2}}\left[r^{DOWN}_{VpI}e^{iP_{I}z}+e^{-iP_{I}z}\right]\nn
F^{DOWN}_{VpII}&=& \sqrt{\frac{P_{II}}{2\epsilon_{0II} \left(\frac{\omega}{c}\right)^2}}\left[r^{DOWN}_{VpII}e^{iP_{II}z}+t^{DOWN}_{VpII}e^{-iP_{II}z}\right]\nn
F^{DOWN}_{VpIII}&=& \sqrt{\frac{P_{III}}{2\epsilon_{0III} \left(\frac{\omega}{c}\right)^2}}t^{DOWN}_{VpIII}e^{-iP_{III}z}
\tea

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Some properties of the basis functions}
From the fact that the complex conjugate of a solution to eqs. (\ref{KG}) and (\ref{KGV}) is also a solution, we may derive some basic properties of the basis functions $F^{UP}_X$ and $F^{DOWN}_X$, where $X$ is either $Hp$ or $Vp$.

First, from flux conservation we get

\bea
1&=&\left|r^{UP}_{XII}\right|^2-\left|t^{UP}_{XII}\right|^2=\frac1{\left|t^{DOWN}_{XIII}\right|^2}-\left|t^{UP}_{XIII}\right|^2\nn
1-\left|r^{DOWN}_{XI}\right|^2&=&\left|t^{DOWN}_{XII}\right|^2-\left|r^{DOWN}_{XII}\right|^2=\left|t^{DOWN}_{XIII}\right|^2
\tea
Next, observe that because $F_X^{DOWN}$, $F_X^{UP}$ and $F_X^{UP*}$ are  solutions, then there must be coefficients $\alpha$ and $\beta$ such that
\be
F_X^{DOWN}=\alpha F^{UP}_X+\beta F^{UP*}_X
\te
It may be seen by inspection that
\bea
\alpha&=&r^{DOWN}_{XI}\nn
\beta&=&1
\tea
This determines the $DOWN$ solution from the $UP$ one. We still have no generic way to relate the $H$ and $V$ solutions to each other.

==> Sections/not_used/first_order.tex <==
\section{First order solution}

\subsection{TE incident mode}

In this case we use as source field equation (\ref{TE-incidence}).

For the scattered field in H-mode, we have 

\bea
\frac {\partial^2}{\partial z^2}\varphi^{\left(1\right)}_{\vec{p}} +P^2\varphi^{\left(1\right)}_{\vec{p}} &=&\left(\frac{\omega}{c}\right)^2\,\int\frac{d^2q}{\left(2\pi\right)^2}\epsilon_{1\left(\vec{p}-\vec{q}\right)}\,\left(\hat{p}\cdot\hat{q}\right)\;\varphi^{\left(0\right)}_{\vec{q}}(z)\nn
&=&\sqrt{2K_I}\,\left(\frac{\omega}{c}\right)^2\left(\hat{p}\cdot\hat{k}\right)\epsilon_{1\left(\vec{p}-\vec{k}\right)}\; F^{DOWN}_{HKII}
\tea

Therefore

\bea
&& S_{HH}(z) \equiv \varphi^{\left(1\right)}_{\vec{p}}\left( z\right) = -\sqrt{2KI}\,\left(\frac{\omega}{c}\right)^2\left(\hat{p}\cdot\hat{k}\right)\int_{-h}^0dz'\;G_{HP}\left( z,z'\right)  \epsilon_{1\left(\vec{p}-\vec{k}\right)}\left( z'\right) F^{DOWN}_{HKII}\left( z'\right) \nn 
&& \varphi^{\left(1\right)}_{\vec{p}}\left( z\right) = -\sqrt{2K_I}\,\left(\frac{\omega}{c}\right)^2\left(\hat{p}\cdot\hat{k}\right)\,F^{PU}_{HPI}( z)\int_{-h}^0dz'\,  \epsilon_{1\left(\vec{p}-\vec{k}\right)}\left( z'\right) F^{DOWN}_{HpII}( z')\,F^{DOWN}_{HKII}( z')
\tea

As the fluctuation of the dielectric permitivity in medium II has 
translational invariance, the mean value of the scattered field vanishes. 

For the energy flux we have,

\bea
&&\langle |\varphi^{(1)}|^2_{\vec{p}}\left( z\right) \rangle = 2KI\,\left(\frac{\omega}{c}\right)^4\left(\hat{p}\cdot\hat{k}\right)^2\,\big\vert F^{UP}_{HPI}(z)\big\vert^2 \nn 
&& \int^0_{-h} d\xi\int^0_{-h}d\xi'\,\langle \epsilon_{1(\mbp-\mbk)}(\xi)\,\epsilon^*_{1(\mbp-\mbk)}(\xi')\rangle \,F^{DOWN}_{HpII}(\xi)\,F^{DOWN}_{HKII}(\xi)\,\left[F^{DOWN}_{HpII}(\xi')\,F^{DOWN}_{HKII}(\xi')\right]^*\nn
&& \nn
&&\langle |\varphi^{(1)}|^2_{\vec{p}}\left( z\right) \rangle = 2KI\,\left(\frac{\omega}{c}\right)^4\left(\hat{p}\cdot\hat{k}\right)^2\,\big\vert F^{UP}_{HPI}(z)\big\vert^2\,\delta(\mbp-\mbk-\mbp+\mbk)\nn 
&& \int^0_{-h} d\xi\int^0_{-h}d\xi'\,C_{\mbp-\mbk}(\xi-\xi') \,F^{DOWN}_{HpII}(\xi)\,F^{DOWN}_{HKII}(\xi)\,\left[F^{DOWN}_{HPII}(\xi')\,F^{DOWN}_{HKII}(\xi')\right]^* \label{HH-O1}
\tea

From now on $\delta(\mbp-\mbk-\mbp+\mbk) = \delta(\mathbf{0})$.

From equation (\ref{HH-O1}) we conclude that, for get a square mean value with units of length$\times$length ($\sim L^2$), the units of the correlation function $C_{\mbp-\mbk}(\xi-\xi')$ must be also $L^2$.

\bigskip 


To compute the V-scattered modes from a TE incident wave (i.e. $S_{VH}$) first we need 

\be 
E_{\vec{p}z}^{\left(1\right)}=\frac{\imath\,p^2}{P^2}\psi'^{\left(1\right)}_{\vec{p}}
\te

Using this in equation (35
), we have

\be
\frac {\partial}{\partial z}\left(\frac{\omega}{c}\right)^2\frac{\epsilon_0}{P^2}   \frac{\partial}{\partial z}\psi^{\left(1\right)}_{\vec{p}} +\epsilon_0\left(\frac{\omega}{c}\right)^2\psi^{\left(1\right)}_{\vec{p}}=\sqrt{2K_I}\,\left(\frac{\omega}{c}\right)^2\,\left(\mathbf{K}\cdot\left(\hat{p}\times\hat{k}\right)\right)\epsilon_{1\left(\vec{p}-\vec{k}\right)}F^{DOWN}_{HKII}(z)
\te

Therefore, 

\bea
&& S_{VH}(z) \equiv \psi^{\left(1\right)}_{\vec{p}}\left( z\right) = -\sqrt{2KI}\,\left(\frac{\omega}{c}\right)^2\left(\mathbf{K}\cdot\left(\hat{p}\times\hat{k}\right)\right)\int_{-h}^0dz'\;G_{Vp}\left( z,z'\right)  \epsilon_{1\left(\vec{p}-\vec{k}\right)}\left( z'\right)F^{DOWN}_{HKII} \left( z'\right)\nn
&& \nn 
&& \psi^{\left(1\right)}_{\vec{p}}\left( z\right) = -\sqrt{2K_I}\,\left(\frac{\omega}{c}\right)^2\left(\mathbf{K}\cdot\left(\hat{p}\times\hat{k}\right)\right)\,F^{UP}_{VpI}(z)\,\int_{-h}^0dz'\, \epsilon_{1\left(\vec{p}-\vec{k}\right)}(z')\,F^{DOWN}_{VpII}(z')\,F^{DOWN}_{HKII}(z')
\tea

Mean energy flux:

\bea 
&& \langle |\psi^{\left(1\right)}_{\vec{p}}\left( z\right)|^2 \rangle =  2K_I\,\left(\frac{\omega}{c}\right)^4\left(\mathbf{K}\cdot\left(\hat{p}\times\hat{k}\right)\right)^2\,\big\vert F^{UP}_{VpI}(z)\big\vert^2\,\delta(\mathbf{0}) \nn 
&& \int^0_{-h} d\xi\int^0_{-h}d\xi'\,C_{\vec{p}-\vec{k}}(\xi,\xi')\,F^{DOWN}_{VpII}(\xi)\,F^{DOWN}_{HKII}(\xi)\,\left[F^{DOWN}_{VpII}(\xi')\,F^{DOWN}_{HKII}(\xi') \right]^* \label{VH-O1}
\tea


\subsection{TM incident mode}

Now we use equation (\ref{TM-incidence}) as source.

For the H-mode scattered field ($S_{HV}$) we have


\bea
\frac{\partial^2}{\partial z^2}\varphi^{\left(1\right)}_{\vec{p}} +P^2\varphi^{\left(1\right)}_{\vec{p}} &=&\left(\frac{\omega}{c}\right)^2\int\frac{d^2q}{\left(2\pi\right)^2}\epsilon_{1\left(\vec{p}-\vec{q}\right)}\left(\mathbf{K}\cdot\left(\hat{p}\times\hat{k}\right)\right)\psi^{(0)}_{\vec{q}}\nn
&=&\sqrt{2K}\,\left(\frac{\omega}{c}\right)^2\left(\mathbf{K}\cdot\left(\hat{p}\times\hat{k}\right)\right)\epsilon_{1\left(\vec{p}-\vec{k}\right)}\; F^{DOWN}_{VKII}
\tea
\\
which leads to a analogous expression for $\psi^{(1)}_{\vec{p}}(z)$ in TE-incident case. 

Now we obtain

\bea
&& \langle |\varphi^{\left(1\right)}_{\vec{p}}\left( z\right)|^2 \rangle =  2KI\,\left(\frac{\omega}{c}\right)^4\left(\mathbf{K}\cdot\left(\hat{p}\times\hat{k}\right)\right)^2\,\big\vert F^{UP}_{HPI}(z)\big\vert^2 \,\delta(\mathbf{0})\nn 
&& \int^0_{-h} d\xi\int^0_{-h}d\xi'\,C_{\vec{p}-\vec{k}}(\xi,\xi')\,F^{DOWN}_{HPII}(\xi)\,F^{DOWN}_{VKII}(\xi)\,\left[F^{DOWN}_{HPII}(\xi')\,F^{DOWN}_{VKII}(\xi') \right]^* \label{HV-O1}
\tea




In the case of V-mode scattered field we have the source with a term that depends on the derivative of $\epsilon_{1\left(\vec{p}-\vec{q}\right)}$. Here we must procedure carefully.

\bea
&& \frac{\partial}{\partial z} \left(\frac{\omega}{c}\right)^2\frac{\epsilon_0}{P^2}\frac{\partial\psi^{(1)}_\mbp}{\partial z}+\epsilon_0\left(\frac{\omega}{c}\right)^2\,\psi^{(1)}_\mbp 
=\nn 
&& = \left(\frac{\omega}{c}\right)^2\,\int\frac{d^2q}{(2\pi)^2}\,\EPpq\,\left(-\hat{p}\cdot\hat{q}\right)\psi^{(0_)}_\mbq(z) -\imath \frac{\partial}{\partial z}\left(\frac{\omega}{c}\right)^2\frac{p}{P^2}\int\frac{d^2q}{(2\pi)^2}\,\EPpq\,E^{(1)}_{z\mbq}(z)\nn
&& \nn
&& \frac{\partial}{\partial z} \left(\frac{\omega}{c}\right)^2\frac{\epsilon_0}{P^2}\frac{\partial\psi^{(1)}_\mbp}{\partial z}+\epsilon_0\left(\frac{\omega}{c}\right)^2\,\psi^{(1)}_\mbp = 
\left(\frac{\omega}{c}\right)^2\,\int\frac{d^2q}{(2\pi)^2}\,\EPpq\,\left(-\hat{p}\cdot\hat{q}\right)\,(2\pi)^2\,\sqrt{2KI}\,\delta(\mbq-\mbk)\,F^{DOWN}_{VKII}(z) \nn
&& -\imath \frac{\partial}{\partial z}\left(\frac{\omega}{c}\right)^2\frac{p}{P^2}\,\int\frac{d^2q}{(2\pi)^2}\,\EPpq\,\imath\frac{q}{Q^2}\,\frac{\partial}{\partial z}(2\pi)^2\,\sqrt{2KI}\delta(\mbp-\mbk)\,F^{DOWN}_{VKII}(z)\nn
&& \nn 
&& \frac{\partial}{\partial z} \left(\frac{\omega}{c}\right)^2\frac{\epsilon_0}{P^2}\frac{\partial\psi^{(1)}_\mbp}{\partial z}+\epsilon_0\left(\frac{\omega}{c}\right)^2\,\psi^{(1)}_\mbp = -\sqrt{2KI}\,
\left(\frac{\omega}{c}\right)^2\,\EPpk\,\left(\hat{p}\cdot\hat{q}\right)\,F^{DOWN}_{VKII}(z) \nn
&& -\imath \sqrt{2KI}\,\frac{\partial}{\partial z}\,\left(\frac{\omega}{c}\right)^2\frac{p}{P^2}\EPpk\,\imath\frac{k}{K^2}\frac{\partial}{\partial z}F^{DOWN}_{VKII}(z)\nn
\tea 

Now we use

\be 
\frac{\partial}{\partial z}F^{DOWN}_{VKII}(z) = \imath KII\,\tilde{F}^{DOWN}_{VKII}(z)
\te 

thus

\bea
&& \frac{\partial}{\partial z}\left(\frac{\omega}{c}\right)^2 \frac{\epsilon_0}{P^2}\frac{\partial\psi^{(1)}_\mbp}{\partial z}+\epsilon_0\left(\frac{\omega}{c}\right)^2\,\psi^{(1)}_\mbp =\nn 
&& =-\sqrt{2KI}\,
\left(\frac{\omega}{c}\right)^2 \left\lbrace \EPpk\,\left(\hat{p}\cdot\hat{q}\right)\,F^{DOWN}_{VKII}(z) +\imath \frac{\partial}{\partial z}\,\frac{p}{P^2}\EPpk\,\frac{k}{K^2}\,KII\tilde{F^{DOWN}_{VkI}}(z)\right\rbrace
\tea 

The V-mode scattered field ($S_{VV}$) results

\bea
&& \psi^{(1)}_\mbp(z) = -\sqrt{2KI}\,\left(\frac{\omega}{c}\right)^2\,F^{UP}_{VPI}(z)\nn 
&& \int^0_{-h}\,dz'\,F^{DOWN}_{VPII}(z')\,\left\lbrace \EPpk\,\left(\hat{p}\cdot\hat{q}\right)\,F^{DOWN}_{VKII}(z') +\imath \frac{\partial}{\partial z}\,\frac{p}{P^2}\EPpk\,\frac{k\,KII}{K^2}\tilde{F}^{DOWN}_{VKII}(z)\right\rbrace 
\tea

We integrate by parts the second term:

\bea
&& \psi^{(1)}_\mbp(z) = -\sqrt{2KI}\,\left(\frac{\omega}{c}\right)^2\,\left(\hat{p}\cdot\hat{q}\right)\,F^{UP}_{VPI}(z)\,\int^0_{-h}\,dz'\,\EPpk\,F^{DOWN}_{VPII}(z')\,F^{DOWN}_{VKII}(z') \nn
&& +\sqrt{2KI}\,\left(\frac{\omega}{c}\right)^2\,\frac{k}{KII}\frac{p}{PII}\,F^{UP}_{VPI}(z)\,\int^0_{-h}\,dz'\,\EPpk\,\tilde{F}^{DOWN}_{VPII}(z')\,\tilde{F}^{DOWN}_{VKII}(z') \nn 
&& +\imath\,\sqrt{2KI}\,\left(\frac{\omega}{c}\right)^2\,\frac{k\,KII}{K^2}\frac{p}{P^2}\,F^{UP}_{VPI}(z)\,
\left[\left(\EPpk\,F^{DOWN}_{VPII}\right)\,\tilde{F}^{DOWN}_{VKII} \right]\Big\vert^{z'=0}_{z'=-h} 
\tea 

In the last term $\EPpk\,F^{DOWN}_{VpII}$ represents $D_z$ evaluated on the interfaces. Due to the matching conditions on this field there is no ambiguity to compute it. Wwe can not give a closed expression for thus quantity because we only know statistical properties of $\EPpk$. \textbf{However, this term already evaluated at some specific value of $z'$ does not must taking into account when mean values are computed.}


\bea
&& \psi^{(1)}_\mbp(z) = -\sqrt{2KI}\,\left(\frac{\omega}{c}\right)^2\,F^{UP}_{VPI}(z)\nn 
&& \int^0_{-h}\,dz'\,\EPpk\,\left\lbrace \,\left(\hat{p}\cdot\hat{q}\right)\,F^{DOWN}_{VPII}(z')\,F^{DOWN}_{VKII}(z') +\frac{k}{KII}\frac{p}{PII}\,\tilde{F}^{DOWN}_{VPII}(z')\,\tilde{F}^{DOWN}_{VKII}(z') \right\rbrace \nn \label{VV-O1}
\tea 

The functions $\tilde{F}$ differs from $F$ just in the sign of the transmission coefficients. Thus it is possible to rearrange the expression (\ref{VV-O1}) in a similar form of (\ref{HH-O1}), (\ref{VH-O1}) and (\ref{HV-O1}).


\bea 
&& \langle \big\vert \psi^{(1)}_\mbp(z) \big\vert^2 \rangle = 2KI\,\left(\frac{\omega}{c}\right)^4\,\vert F^{UP}_{VPI}(z)\vert^2 \,\delta(\mathbf{0})\,\int^0_{-h}\,d\xi \,\int^0_{-h}\,d\xi'\,C_{\vec{p}-\vec{k}}(\xi,\xi') \nn 
&& \left\lbrace \,\left(\hat{p}\cdot\hat{q}\right)\,F^{DOWN}_{VPII}(\xi)\,F^{DOWN}_{VKII}(\xi) +\frac{k}{KII}\frac{p}{PII}\,\tilde{F}^{DOWN}_{VPII}(\xi)\,\tilde{F}^{DOWN}_{VKII}(\xi) \right\rbrace \nn
&& \left\lbrace \,\left(\hat{p}\cdot\hat{q}\right)\,F^{DOWN}_{VPII}(\xi')\,F^{DOWN}_{VKII}(\xi') +\frac{k}{KII}\frac{p}{PII}\,\tilde{F}^{DOWN}_{VPII}(\xi')\,\tilde{F}^{DOWN}_{VKII}(\xi') \right\rbrace^*
\tea


\subsection{Computing mean values}

The scattering amplitude for HH, HV and VH channels can be written as

\bea
S^{(1)}_{ab}(z) = \sqrt{2KI}\,\left(\frac{\omega}{c}\right)^2\,F^{UP}_{aPI}(z)\int^0_{-h}\,dz'\,\EPpk(z')\,\mathcal{C}_{ab}\, 
\left[r_a\,e"{\imath PII z'} + t_a\,e^{-\imath PII z'} \right]\,
\left[r_b\,e"{\imath KII z'} + t_b\,e^{-\imath KII z'} \right]
\tea 

where $a\,(b)$ is the polarization of the scattered (incident) wave, $\mathcal{C}_{ab}$ is a factor coming from the product between the Green's functions. From now on we will replace $\omega/c$ by $k_i$.

The scattered mean energy results:

\bea 
&& \langle \big\vert S^{(1)}_{ab}(z) \big\vert^2 \rangle = \delta(\mathbf{0})\,2 KI \, k^4_i\,\vert \mathcal{C}_{ab}\vert^2 \,\vert F^{UP}_{a PI} \vert^2 \int^0_{-h}\,d\xi\,\int^0_{-h}\,d\xi'\,C_{\mbp-\mbk}(\xi-\xi') \nn
&& \left[|r_a|^2\, e^{\imath (\xi-\xi')PII} + |t_a|^2\, e^{-\imath (\xi-\xi')PII} + 2  \Re\left\lbrace r_a\,t^*_a e^{\imath (\xi+\xi')PII} \right\rbrace \right] \nn
&& \left[|r_b|^2\, e^{\imath (\xi-\xi')KII} + |t_b|^2\, e^{-\imath (\xi-\xi')KII} + 2  \Re\left\lbrace r_b\,t^*_b e^{\imath (\xi+\xi')KII} \right\rbrace\right]
\tea

Rearranging,

\bea 
&& \langle \big\vert S^{(1)}_{ab}(z) \big\vert^2 \rangle = \delta(\mathbf{0})\,2 KI \, k^4_i\,\vert \mathcal{C}_{ab}\vert^2 \,\vert F^{UP}_{a PI} \vert^2 \int^0_{-h}\,d\xi\,\int^0_{-h}\,d\xi'\,C_{\mbp-\mbk}(\xi-\xi') \nn
&& \left\lbrace |r_a|^2\,|r_b|^2\, e^{\imath (\xi-\xi')P^+} + |t_a|^2\,|t_b|^2 e^{-\imath (\xi-\xi')P^+} + |r_a|^2\,|t_b|^2\, e^{\imath (\xi-\xi')P^-} + |t_a|^2\,|r_b|^2 e^{-\imath (\xi-\xi')P^-} \right.\nn
&& \left. +4 \Re\left\lbrace r_a\,t^*_a e^{\imath (\xi-\xi')PII} \right\rbrace \,\Re\left\lbrace r_b\,t^*_b e^{\imath (\xi+\xi')KII} \right\rbrace \right.\nn
&&\left. + 2\Re\left\lbrace r_b\,t^*_b e^{\imath (\xi+\xi')KII} \right\rbrace \, \left[|r_a|^2\, e^{\imath (\xi-\xi')PII} + |t_a|^2\, e^{-\imath (\xi-\xi')PII} \right] \right. \nn
&& \left. + 2\Re\left\lbrace r_a\,t^*_a e^{\imath (\xi+\xi')PII} \right\rbrace \, \left[|r_b|^2\, e^{\imath (\xi-\xi')KII} + |t_b|^2\, e^{-\imath (\xi-\xi')KII} \right] \right\rbrace \nn 
&& \nn
&& \Rightarrow \langle \big\vert S^{(1)}_{ab}(z) \big\vert^2 \rangle = \delta(\mathbf{0})\,2 KI \, k^2_i\,\vert \mathcal{C}_{ab}\vert^2 \,\vert F^{UP}_{a PI} \vert^2 \int^0_{-h}\,d\xi\,\int^0_{-h}\,d\xi'\,C_{\mbp-\mbk}(\xi-\xi')\,f(\xi,\xi')
\tea

where we have defined $P^\pm = PII \pm KII$.

Instead of doing the integral in $\left[-h,0\right]\times\left[-h,0\right]$ we make the following change of variables: $\xi-\xi'=x$ and $\xi+\xi'=y$. Then, we get,

\bea
&& \langle \big\vert S^{(1)}_{ab}(z) \big\vert^2 \rangle = \delta(\mathbf{0})\,2 KI \, k^4_i\,\vert \mathcal{C}_{ab}\vert^2 \,\vert F^{UP}_{a PI} \vert^2 \,\left[I_1 + I_2 \right] \nn
&& \nn
&& I_1 = \frac{1}{2} \int^0_{-h} dx\,C_{\mbp-\mbq}(x)\,\int^{x}_{-x-2h} dy\,f(x,y)\nn
&& I_2 = \frac{1}{2} \int^h_{0} dx\,C_{\mbp-\mbq}(x)\,\int^{-x}_{x-2h} dy\,f(x,y)
\tea

As $C_{\mbp-\mbq}(x) = C_{\mbp-\mbq}(-x) $ in $I_2$ we can change $x$ by $-x$ to obtain

\bea 
&& I_1 + I_2 = \frac{1}{2} \int^0_{-h} dx\,C_{\mbp-\mbq}(x)\,\int^{x}_{-r-2h} dy\,\left[f(x,y) + f(-x,y) \right]\nn
&& I_1 + I_2 = \frac{1}{2} \int^0_{-h} dx\,C_{\mbp-\mbq}(x)\,\int^{x}_{-r-2h} dy\, 2 \Re \left\lbrace f(x,y) \right\rbrace
\tea

The integral over $y$ has an analytic expression and we get, at first order in perturbations, a mean energy flux expressed as an integral over the thickness of the random media and it is a function of the correlation fluctuations of the dielectric permittivity:

\bea
&& \langle \big\vert S^{(1)}_{ab}(z) \big\vert^2 \rangle = \delta(\mathbf{0})\,2 KI \, k^4_i\,\vert \mathcal{C}_{ab}\vert^2 \,\vert F^{UP}_{a PI} \vert^2 \int^0_{-h}\,dx\,C_{\mbp-\mbk}(x)\,\sum^5_{j=1} \,T_j(\mbp,\mbk,x) \nn
&& \nn 
&& T_1 = 2(x+h)\,\left[|r_a|^2\,|r_b|^2 + |t_a|^2\,|t_b|^2\right]\,\cos(P^+\,x)\nn 
&& T_2 = 2(x+h)\,\left[|r_a|^2\,|t_b|^2 + |t_a|^2\,|r_b|^2\right]\,\cos(P^-\,x)\nn 
&& T_3 = 2\frac{|r_b\,t^*_b|}{KII}\,\left[|r_a|^2+|t_a|^2 \right]\,\cos(PII\,x)\,\left[\sin(KII\,x+\phi_b)+\sin(KII\,(x+2h)-\phi_b) \right] \nn
&& T_4 = 2\frac{|r_a\,t^*_a|}{PII}\,\left[|r_b|^2+|t_b|^2 \right]\,\cos(KII\,x)\,\left[\sin(PII\,x+\phi_a)+\sin(PII\,(x+2h)-\phi_a) \right] \nn 
&& T_5 = 4|r_a\,t^*_a|\,|r_b\,t^*_b|
  \begin{cases} 
   x+h+\frac{1}{PII}\left[\sin(2PII\,x+\phi_a)+\sin(2PII(x+2h)+2\phi_a) \right], & \text{if}\, PII = KII \\
   \\
   \frac{1}{P^+}\left[\sin(P^+\,x+\phi^+)+\sin(P^+(x+2h)-\phi^+) \right] \\
   + \frac{1}{P^-}\left[\sin(P^-\,x+\phi^-)+\sin(P^-(x+2h)-\phi^-) \right],       & \text{if } PII \neq KII
  \end{cases} \nn 
\tea 

where $\phi_a$ is the argument of the complex coefficient $r_a\,t^*_a$ (the same for $\phi_b$), $\phi^\pm = \phi_a \pm \phi_b$; it seems that the last term can be rewritten as \textit{sinc} function.

With VV channel we must be careful because it has a second term that depends on $\tilde{F}$. After some manipulation we found that: $T_1 \rightarrow |\alpha_+|^2\,T_1$; $T_2 \rightarrow |\alpha_-|^2\,T_2$; $T_3(|r_a|^2, \phi_b) \rightarrow |\alpha_+\,\alpha^*_-|\,T_3(|r_a|^2, \phi_b+\phi_\alpha)$, $T_3(|t_a|^2, \phi_b) \rightarrow |\alpha_+\,\alpha^*_-|\,T_3(|t_a|^2, \phi_b-\phi_\alpha)$; $T_4(|r_b|^2, \phi_a) \rightarrow |\alpha_+\,\alpha^*_-|\,T_4(|r_b|^2, \phi_a+\phi_\alpha)$, $T_4(|t_b|^2, \phi_a) \rightarrow |\alpha_+\,\alpha^*_-|\,T_4(|t_b|^2, \phi_a-\phi_\alpha)$; $T_5(P^+) \rightarrow |\alpha_+|^2\,T_5(P^+)$, $T_5(P^-) \rightarrow |\alpha_-|^2\,T_5(P^-)$, being $\alpha_\pm = \hat{p}\cdot\hat{k} \pm \frac{p\,k}{PII\,KII}$.

==> Sections/not_used/getting_HV.tex <==
\section{HV is a thing of nothing}
We now consider the case where $\epsilon=\epsilon_0\left(z\right)+\epsilon_1\left(\vec{x},z\right)$. We get 

\bea
\left(\frac {\partial^2}{\partial z^2}+\frac {\partial^2}{\partial y^2}\right)E_x-\frac {\partial}{\partial x}\left(\frac {\partial E_y}{\partial y}+\frac {\partial E_z}{\partial z}\right) +\epsilon_0\left(\frac{\omega}{c}\right)^2E_x&=&-\epsilon_1\left(\frac{\omega}{c}\right)^2E_x\nn
\left(\frac {\partial^2}{\partial z^2}+\frac {\partial^2}{\partial x^2}\right)E_y-\frac {\partial}{\partial y}\left(\frac {\partial E_x}{\partial x}+\frac {\partial E_z}{\partial z}\right) +\epsilon_0\left(\frac{\omega}{c}\right)^2E_y&=&-\epsilon_1\left(\frac{\omega}{c}\right)^2E_y\nn
\left(\frac {\partial^2}{\partial x^2}+\frac {\partial^2}{\partial y^2}\right)E_z-\frac {\partial}{\partial z}\left(\frac {\partial E_x}{\partial x}+\frac {\partial E_y}{\partial y}\right) +\epsilon_0\left(\frac{\omega}{c}\right)^2E_z&=&-\epsilon_1\left(\frac{\omega}{c}\right)^2E_z
\tea
Performing a two dimensional Fourier transform 

\bea
&&\left(\frac {\partial^2}{\partial z^2}-p_y^2\right)E_{\vec{p}x}-ip_x\left(ip_yE_{\vec{p}y}+\frac {\partial E_{\vec{p}z}}{\partial z}\right) +\epsilon_0\left(\frac{\omega}{c}\right)^2E_{\vec{p}x}=-\left(\frac{\omega}{c}\right)^2\int\frac{d^2q}{\left(2\pi\right)^2}\epsilon_{1\left(\vec{p}-\vec{q}\right)}E_{\vec{q}x}\nn
&&\left(\frac {\partial^2}{\partial z^2}-p_x^2\right)E_{\vec{p}y}-ip_y\left(ip_xE_{\vec{p}x}+\frac {\partial E_{\vec{p}z}}{\partial z}\right)+\epsilon_0\left(\frac{\omega}{c}\right)^2E_{\vec{p}y}=-\left(\frac{\omega}{c}\right)^2\int\frac{d^2q}{\left(2\pi\right)^2}\epsilon_{1\left(\vec{p}-\vec{q}\right)}E_{\vec{q}y}\nn
&&-i\frac {\partial}{\partial z}\left(\vec{p}\vec{E}_{\vec{p}}\right) +\left(\epsilon_0\left(\frac{\omega}{c}\right)^2-p^2\right)E_{\vec{p}z}=-\left(\frac{\omega}{c}\right)^2\int\frac{d^2q}{\left(2\pi\right)^2}\epsilon_{1\left(\vec{p}-\vec{q}\right)}E_{\vec{q}z}
\tea
We may always decompose

\be 
\vec{E}_{\vec{p}}=\left(\mathbf{K}\times\hat{p}\right)\varphi_{\vec{p}}+\hat{p}\psi_{\vec{p}}
\label{decomp}
\te
so 

\be 
\left[P^2E_{\vec{p}z}+\left(\frac{\omega}{c}\right)^2\int\frac{d^2q}{\left(2\pi\right)^2}\epsilon_{1\left(\vec{p}-\vec{q}\right)}E_{\vec{q}z}\right]=ip\psi'_{\vec{p}}
\label{easy}
\te
Where $P^2=\epsilon_0\left(\frac{\omega}{c}\right)^2-p^2$. Observe that this equation is local in $z$, meaning that $E_{\vec{p}z}$ is defined from $\psi'$ evaluated at the same height.

Eq. (\ref{decomp}) may be inverted

\bea
\varphi_{\vec{p}}&=&\mathbf{K}\cdot\left(\hat{p}\times\vec E_{\vec p}\right)=-\hat{p}_yE_{\vec{p}x}+\hat{p}_xE_{\vec{p}y}\nn
\psi_{\vec{p}}&=&\hat{p}\cdot\vec E_{\vec p}=\hat{p}_xE_{\vec{p}x}+\hat{p}_yE_{\vec{p}y}
\tea
so 
\bea
\frac {\partial^2}{\partial z^2}\varphi_{\vec{p}} +P^2\varphi_{\vec{p}} &=&-{\left(\frac{\omega}{c}\right)^2}\int\frac{d^2q}{\left(2\pi\right)^2}\epsilon_{1\left(\vec{p}-\vec{q}\right)}\;\mathbf{K}\cdot\left(\hat{p}\times\vec E_{\vec q}\right)\nn
&=&-{\left(\frac{\omega}{c}\right)^2}\int\frac{d^2q}{\left(2\pi\right)^2}\epsilon_{1\left(\vec{p}-\hat{q}\right)}\left[\hat{p}\cdot\hat{q}\;\varphi_{\vec{q}}+\mathbf{K}\cdot\left(\hat{p}\times\hat{q}\right)\psi_{\vec{q}}\right]
\label{KGC}
\tea
and 
\bea
\frac {\partial^2}{\partial z^2}\psi_{\vec{p}} -ip \frac {\partial}{\partial z}E_{\vec{p}z}+\epsilon_0\left(\frac{\omega}{c}\right)^2\psi_{\vec{p}}&=&-{\left(\frac{\omega}{c}\right)^2}\int\frac{d^2q}{\left(2\pi\right)^2}\epsilon_{1\left(\vec{p}-\vec{q}\right)}\;\hat{p}\cdot\vec E_{\vec{q}}\nn
&=&{\left(\frac{\omega}{c}\right)^2}\int\frac{d^2q}{\left(2\pi\right)^2}\epsilon_{1\left(\vec{p}-\vec{q}\right)}\left[\mathbf{K}\cdot\left(\hat{p}\times\hat{q}\right)\varphi_{\vec{q}}-\hat{p}\cdot\hat{q}\;\psi_{\vec{q}}\right]
\label{KGE}
\tea
or else, using eq. (\ref{easy})

\bea
&& \frac {\partial^2}{\partial z^2}\psi_{\vec{p}} + \frac {\partial}{\partial z}\frac{p^2}{P^2}\frac {\partial}{\partial z}\psi_{\vec{p}}+\epsilon_0\left(\frac{\omega}{c}\right)^2\psi_{\vec{p}}=\nn 
&& = {\left(\frac{\omega}{c}\right)^2}\int\frac{d^2q}{\left(2\pi\right)^2}\epsilon_{1\left(\vec{p}-\vec{q}\right)}\left[\mathbf{K}\cdot\left(\hat{p}\times\hat{q}\right)\varphi_{\vec{q}}-\hat{p}\cdot\hat{q}\;\psi_{\vec{q}}\right]-ip\frac {\partial}{\partial z}\left(\frac{\omega}{c}\right)^2\frac{1}{P^2}\int\frac{d^2q}{\left(2\pi\right)^2}\epsilon_{1\left(\vec{p}-\vec{q}\right)}E_{\vec{q}z}
\label{KGE2}
\tea

Eq (\ref{KGE}) shows that it is possible to generate $V$ polarization from $H$ polarization, though not in backscattering to first order.

==> Sections/not_used/results_old.tex <==
\section{Results}

\subsection{Funciones de Correlación}

Para terminar las cuentas vamos a usar tres tipos de funciones de correlación:

\bea 
 && \langle \epsilon_\mbp(z)\,\epsilon^*_\mbq(z')\rangle = \delta(\mbp-\mbq)\,C_\mbp(z-z') \nn 
 && = \delta(\mbp-\mbq)\,C_\mbp\,C(z-z') = 
  \begin{cases} 
   \frac{s\,l^2_r}{(2\pi)^2}\,e^{-(\mbp\,l_r/2)^2}\,e^{-((z-z')/(2l_z))^2}, & \text{Gaussian ACF}\\
   \frac{s\,l^2_r}{(2\pi)^2}\,e^{-(\mbp\,l_r/2)^2}\,e^{-((z-z')/(2l_z))^2}\,e^{-|z-z'|/l_z},       & \text{Exponential ACF}\\
   f_v\,\frac{2\pi\,l_r}{p}\,J_1(l_r\,p)\,\Theta(l^2_z-(z-z')^2),      & \text{Heaviside-like ACF}
  \end{cases}
\tea 

donde $s$ indica la intensidad de las fluctuaciones en el dieléctrico (valor rms), $f_v$ es la densidad de 'latas' y $J_1$ la función de Bessel de primer orden.

En la expresión del término Ladder (o Cross) debemos integrar la parte en $z$ sobre el espesor de la capa dieléctrica. Esto lo podemos hacer de manera explícita.


\textit{Gaussian ACF:}

\bea
\int^0_{-h}\,dz\,C(z)\,e^{\imath Q z} = 
 \begin{cases}
     \sqrt{\pi}\,l_z\,\text{Erf}(0.5 h/l_z), & \text{si} Q = 0 \\
     \sqrt{\pi}\,l_z\,e^{-(l_z\,Q)^2}\,\left[\text{Erf}(h/l_z+\imath l_z\,Q/2)-\imath\,\text{Erfi}(l_z\,Q) \right], & \text{si} Q \neq 0
 \end{cases}
\tea

\textit{Exponential ACF:}

\bea
\int^0_{-h}\,dz\,C(z)\,e^{\imath Q z} = 
 \begin{cases}
     l_z\,\left(1-e^{-h/l_z} \right), & \text{si} Q = 0 \\
     \frac{l_z}{1+\imath l_z\,Q}\left(1-e^{-h(1/l_z+\imath Q)} \right), & \text{si} Q \neq 0
 \end{cases}
\tea


\textit{Heaviside-like ACF:}

\bea
\int^0_{-h}\,dz\,C(z)\,e^{\imath Q z} = 
 \begin{cases}
     h-l_z, & \text{si} Q = 0 \\
     \frac{1}{\imath \,Q}\left[e^{-\imath l_z\,Q} - e^{-\imath h\,Q} \right], & \text{si} Q \neq 0
 \end{cases}
\tea


\subsection{Backscattering como función del ángulo de incidencia}

Escenario general:

Onda incidente: $\lambda = 0.235$ m; Medios dieléctricos homogeneos: $\epsilon_1 = 1.05$, $\epsilon_2 = 12$; Fluctuaciones: $S = 9\times 10^{-3}$, $l_r = 0.07$ m, $l_z = 0.004$ m, $f_v = 2.5\times 10^{-6}$. Tres espesores para el medio aleatorio: $D = \left\lbrace 0.05; 0.85; 2.85 \right\rbrace$ m.

\begin{figure}
    \centering
    \includegraphics[width = 0.86\textwidth]{figures/BS_total/BS_d1.jpg}
    \caption{Backscattering as a function of incident angle. SAOCOM operates at $\theta \sim 30$. Thickness layer = 0.05 m.}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width = 0.86\textwidth]{figures/BS_total/BS_d2.jpg}
    \caption{Backscattering as a function of incident angle. Thickness layer = 0.85 m.}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width = 0.86\textwidth]{figures/BS_total/BS_d3.jpg}
    \caption{Backscattering as a function of incident angle. Thickness layer = 2.85 m.}
\end{figure}


% We will use three kind of correlation functions:

% \bea 
% && \text{-- Gaussian: }\,\,C_{\mbp}(z) = \frac{s\,l^2_r}{(2\pi)^2}\,\exp{\left[-\frac{1}{4}l^2_r\,q^2_\perp\right]}\,\exp{\left[-\frac{z^2}{(2l_z)^2} \right]} \nn
% && \text{-- Exponential: }\,\,C_{\mbp}(z) = \frac{s\,l^2_r}{(2\pi)^2}\,\exp{\left[-\frac{1}{4}l^2_r\,q^2_\perp\right]}\,\exp{\left[-\frac{|z|}{l_z} \right]} \nn
% && \text{-- Tuna can:}\,\, C_{\mbp}(z) = \frac{f_v\,2\pi l_r}{q_\perp}\,J_1(q_\perp\,l_r)\,\Theta(l^2_z-z^2) \nonumber
% \tea 

% where $q_\perp = \sqrt{q^2_x + q^2_y}$ and $J_1$ is the Bessel function of first kind.


% \subsubsection{Backscattering as a function of incident angle}

% Parameters used: $\lambda = 23.5$ cm (SAOCOM wavelength), $\epsilon_1 = 3$ (typical value of dry semi-arid soil as Cordoba), $\epsilon_2 = 14$, thickness layer $D = 0.85$ m, $l_r=7$ cm, $l_z = 0.4$cm, $s = 0.009$ (intensity of fluctuations) and $fv = 0.005$ (densidad de latas).

% % \begin{figure}
% %     \centering
% %     \includegraphics[width = 0.6\textwidth]{figures/Orden_1/BS_theta_O1.jpg}
% %     \caption{Backscattering as a function of incident angle. SAOCOM operates at $\theta \sim 30$.}
% % \end{figure}


% \subsubsection{Backscattering as a function of the thickness of the layer}

% Parameters used: $\lambda = 23.5$ cm $\theta_i = 30$, $\epsilon_1 = 4$, $\epsilon_2 = 12$, $l_r=5$ cm, $l_z = 0.2$cm, $s = 0.009$ (intensity of fluctuations) and $fv = 0.001$ (densidad de latas).

% % \begin{figure}
% %     \centering
% %     \includegraphics[width = 0.6\textwidth]{figures/Orden_1/BS_D_O1.jpg}
% %     \caption{Backscattering as a function of the thickness of the layer.}
% % \end{figure}


% \subsubsection{Backscattering as a function of the vertical correlation length}

% Parameters used: $\lambda = 23.5$ cm $\theta_i = 30$, $\epsilon_1 = 4$, $\epsilon_2 = 12$, $l_r=8$ cm, $D = l_z/0.75$, $s = 0.009$ (intensity of fluctuations) and $fv = 0.001$ (densidad de latas).

% % \begin{figure}
% %     \centering
% %     \includegraphics[width = 0.6\textwidth]{figures/Orden_1/BS_Lz_O1.jpg}
% %     \caption{Backscattering as a function of the vertical correlation length.}
% % \end{figure}


% \subsubsection{Heatmap $(\epsilon 1,\epsilon 2)$ at backscattering}

% Parameters used: $\lambda = 23.5$ cm $\theta_i = 32$,  $D = 1.25$ m,$l_r=4$ cm, $l_z = 2.5$ cm, $s = 0.009$ (intensity of fluctuations) and $fv = 0.001$ (densidad de latas).

% % \begin{figure}
% %     \centering
% %     \includegraphics[width = 0.9\textwidth]{figures/Orden_1/heatmap_ep1_ep2.jpg}
% %     \caption{Heatmap $(\epsilon_1,\epsilon_2)$ at backscattering.}
% % \end{figure}


% \subsubsection{Heatmap $(D,lz)$ at backscattering}

% Parameters used: $\lambda = 23.5$ cm $\theta_i = 40$, $\epsilon_1 = 4$, $\epsilon_2 = 15$, $l_r=5$ cm, $s = 0.09$ (intensity of fluctuations) and $fv = 0.001$ (densidad de latas).

% % \begin{figure}
% %     \centering
% %     \includegraphics[width = 0.9\textwidth]{figures/Orden_1/heatmap_D1_Lz.jpg}
% %     \caption{Heatmap $(D,l_z)$ at backscattering.}
% % \end{figure}

==> Sections/not_used/second_order.tex <==
\section{Second order solution}

Here we need compute the source terms gave in Section 5 using as input the first order scattered fields.

\subsection{TE incident mode}

Equation for $S^{(2)}_{HH}$:

\be
\frac{d^2}{dz^2}\vpp^{(2)}+P^2\vpp{(2)} = -J^{(2)}_{HH\mbp}(z) \label{vpp_O2}
\te

\bea
J^{(2)}_{HH\mbp}(z) &=& \left(\frac{\omega}{c}\right)^2\,\int\,\frac{d^2q}{(2\pi)^2}\,\EPpq(z)\,\left[\hat{p}\cdot\hat{q}\,\vpq^{(1)}(z)+\mbK\cdot\left(\hat{p}\times\hat{q}\right)\,\psiq^{(1)}(z)\right]\nn
&& \nn
J^{(2)}_{HH\mbp}(z) &=&  \sqrt{2K_I}\,\left(\frac{\omega}{c}\right)^4\,\int\,\frac{d^2q}{(2\pi)^2}\,\EPpq(z)\,\int^0_{-h}\,dz'\,\EPqki(z')\nn
&& \left[(\hat{p}\cdot\hat{q})\,(\hat{q}\cdot\hat{k})\,\sum_\mu\,F^\mu_{H QII}(z)\,F^{\bar{\mu}}_{H QII}(z')\,F^{DOWN}_{HKII}(z')\Theta_\mu(z,z')\right.\nn
&&\left. +\mbK\cdot\left(\hat{p}\times\hat{q}\right)\,\mbK\cdot\left(\hat{q}\times\hat{k}\right)\,\sum_{\mu = U, D}\,F^\mu_{V QII}(z)\,F^{\bar{\mu}}_{V QII}(z')\,F^{DOWN}_{HKII}(z')\,\Theta_\mu(z,z')\right]\,\,F^{D}_{HKII}(z')
\tea

where if $\mu=\{UP, DOWN\}\,\,\Rightarrow\,\,\bar{\mu}=\{DOWN, UP\}$ and $\Theta_{UP}(z,z') = \Theta(z>z')$ and $\Theta_{DOWN}(z,z') = \Theta(z<z')$.

We define another index, $m=\{H, V\}$ which indicates the polarization of waves in medium II. Together to this index we have $\beta_H = (\hat{p}\cdot\hat{q})\,(\hat{q}\cdot\hat{k})$ and $\beta_V = \mbK\cdot\left(\hat{p}\times\hat{q}\right)\,\mbK\cdot\left(\hat{q}\times\hat{k}\right)$.

Then, the current HH to second order can be rearranged as

\bea
&& J^{(2)}_{HH\mbp}(z) = \sqrt{2K_I}\,\left(\frac{\omega}{c}\right)^4\,\int\,\frac{d^2q}{(2\pi)^2}\,\EPpq(z)\,\int^0_{-h}\,dz'\,\EPqki(z')\nn 
&& \sum_\mu\,\sum_m\,\beta_m\,F^\mu_{mQII}(z)\,F^{\bar{\mu}}_{mQII}(z')\,\Theta_\mu(z,z')\,F^{DOWN}_{HKII}(z')
\tea

Then,

\bea
&& S^{(2)}_{HH}(z) = \vpp^{(2)}(z) = -\int^0_{-h}\,d\xi\,G_{Hp}(z,\xi)\,J^{(2)}_{HH\mbp}(\xi) \nn
&& S^{(2)}_{HH}(z) = -\int^0_{-h}\,dz_1\,F^{UP}_{HPI}(z)\,F^{D}_{HPII}(z_1)\,\,J^{(2)}_{HH\mbp}(z_1) \nonumber
\tea

% \bea
% S^{(2)}_{HH}(z) &=& -\sqrt{2K_I}\,\left(\frac{\omega}{c}\right)^4\,F^{UP}_{HPI}(z)\,\int\,\frac{d^2q}{(2\pi)^2}\,\int^0_{-h}\,d\xi\,\EPpq(\xi)\,F^{D}_{HPII}(\xi)\,\int^0_{-h}\,dz'\,\EPqki(z')\,F^{D}_{HK_I}(z')\nn
% &&\left[(\hat{p}\cdot\hat{q})\,(\hat{q}\cdot\hat{k})\,F^{UP}_{HPI}(\xi)F^{D}_{HPII}(z') +\mbK\cdot\left(\hat{p}\times\hat{q}\right)\,\mbK\cdot\left(\hat{q}\times\hat{k}\right)\,F^{UP}_{VPI}(\xi)F^{D}_{VPII}(z')\right]
% \tea 

\bea
S^{(2)}_{HH}(z) &=& -\sqrt{2K_I}\,\left(\frac{\omega}{c}\right)^4\,F^{UP}_{HPI}(z)\,\int\,\frac{d^2q}{(2\pi)^2}\,\int^0_{-h}\,dz_1\,\int^{Ls(z1)}_{Li(z1)}\,dz_2\,\,\EPpq(z_1)\,\EPqki(z_2)\nn
&& \sum_\mu\,\sum_m\,\beta_m\,F^{D}_{HPII}(z_1)\,F^\mu_{mQII}(z_1)\,F^{\hat{\mu}}_{mQII}(z_2)\,F^{DOWN}_{HKII}(z_2)\,\Theta_\mu(z_1,z_2) \label{HH_O2}
\tea

% \bea
% S^{(2)}_{HH}(z) = -\sqrt{2K_I}\,\left(\frac{\omega}{c}\right)^4\,F^{UP}_{HPI}(z)\,&&\int\,\frac{d^2q}{(2\pi)^2}\,\int^0_{-h}\,dz_1\,\int^{Ls(z1)}_{Li(z1)}\,dz_2\,\,\EPpq(z_1)\,\EPqki(z_2)\nn
% &&\sum_{\mu,m}\,F^{D}_{HPII}(z_1)\,\mathcal{H}^{\mu,m}_{\mbp,\mbq}(z_1,z_2)\,F^{DOWN}_{HKII}(z_2)
% \tea

where the integration limits over $dz_2$ depends of $\Theta_\mu(z_1,z_2)$. For the case $\Theta(z_1>z_2)\,\,\Rightarrow\,\,-h<z_2<z_1$, its complement is $\Theta(z_1<z_2)\,\,\Rightarrow\,\,z_1<z_2<0$.


Equation for $S^{(2)}_{VH}$:

\be
\frac{d}{dz}\left(\frac{\omega}{c}\right)^2\frac{\epsilon}{P^2}\frac{}d{dz}\psi^{(2)}_\mbp + \epsilon\left(\frac{\omega}{c}\right)^2\psi^{(2)}_\mbp = J^{(2)}_{VH\mbp}(z) \label{psi_O2}
\te 

with

\bea
J^{(2)}_{VH\mbp}(z) &=& \left(\frac{\omega}{c}\right)^2\,\int\,\frac{d^2q}{(2\pi)^2}\,\EPpq(z)\,\left[-\mbK\cdot\left(\hat{p}\times\hat{q}\right)\,\vpq^{(1)}(z)+\hat{p}\cdot\hat{q}\,\psiq^{(1)}(z)\right]\nn
&& +\imath p\frac{\partial}{\partial z}\left(\frac{\omega}{c}\right)^2\frac{1}{P^2}\int\,\frac{d^2q}{(2\pi)^2}\EPpq(z)\,\imath\frac{q}{Q^2}\frac{d}{dz}\psi^{(1)}_\mbq(z)
\tea

In the following we use $\frac{d}{dz}\psi^{(1)}_\mbq(z) = \tilde{\psi}^{(1)}_\mbq(z)$.


Then,

\be
\psi^{(2)}_\mbp(z) = S^{(2)}_{VH}(z) = -\int^0_{-h}\,d\xi\,F^{UP}_{VPI}(z)\,F^D_{VPII}(\xi)\,J^{(2)}_{VH\mbp}(\xi)
\te 

\bea
\psi^{(2)}_\mbp(z) &=& -\left(\frac{\omega}{c}\right)^2\,F^{UP}_{VPI}(z)\,\int^0_{-h}\,dz'\,\int \frac{d^2q}{(2\pi)^2}\EPpq(z')\,F^{D}_{VPII}(z')\,\left[-\mbK\cdot\left(\hat{p}\times\hat{q}\right)\,\vpq^{(1)}(z)+\hat{p}\cdot\hat{q}\,\psiq^{(1)}(z)\right]\nn
&& - F^{UP}_{VPI}(z)\,\int^0_{-h}\,dz'\,F^{D}_{VPII}(z')\imath p \frac{\partial}{\partial z'}\left(\frac{\omega}{c}\right)^2\frac{1}{P^2}\int \frac{d^2q}{(2\pi)^2}\,\EPpq(z')\imath\frac{q}{Q^2}\tilde{\psi}^{(1)}_\mbq(z')
\tea

We integrate by part and, ignoring the edge term, we get

\bea
\psi^{(2)}_\mbp(z) &=& -\left(\frac{\omega}{c}\right)^2\,F^{UP}_{VPI}(z)\,\int^0_{-h}\,dz'\,\int \frac{d^2q}{(2\pi)^2}\EPpq(z')\,F^{D}_{VPII}(z')\,\left[-\mbK\cdot\left(\hat{p}\times\hat{q}\right)\,\vpq^{(1)}(z)+\hat{p}\cdot\hat{q}\,\psiq^{(1)}(z)\right]\nn
&& + F^{UP}_{VPI}(z)\,\int^0_{-h}\,dz'\,\imath \left(\frac{\omega}{c}\right)^2 \frac{p}{P^2}\int \frac{d^2q}{(2\pi)^2}\,\EPpq(z')\imath\frac{q}{Q^2}\tilde{\psi}^{(1)}_\mbq(z')\,\frac{d}{dz'}F^{D}_{VPII}(z')
\tea


Thus,

\bea
\psi^{(2)}_\mbp(z) &=& -\left(\frac{\omega}{c}\right)^2\,F^{UP}_{VPI}(z)\,\int^0_{-h}\,dz'\,\int \frac{d^2q}{(2\pi)^2}\EPpq(z')\,\left\lbrace F^{D}_{VPII}(z')\,\left[-\mbK\cdot\left(\hat{p}\times\hat{q}\right)\,\vpq^{(1)}(z)+\hat{p}\cdot\hat{q}\,\psiq^{(1)}(z)\right] \right.\nn
&&\left.+\frac{p\,q}{P^2\,Q^2}\tilde{\psi}^{(1)}_\mbq(z)\,\frac{d}{dz'}F^{D}_{VPII}(z')\right\rbrace
\tea

In both $\tilde{\psi}$ as in $dF/dz'$ we will use

\be
\frac{d}{dz} F_{Q}(z) = \imath Q\,\tilde{F}
\te 

where in $\tilde{F}$ the term proportional to the transmission coefficient has a minus sign.

Putting the fields of first order in their explicit form we get

\bea
\psi^{(2)}_\mbp(z) &=&- \sqrt{2KI}\left(\frac{\omega}{c}\right)^4\,F^{UP}_{VPI}(z)\,\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz_2\,\int \frac{d^2q}{(2\pi)^2}\EPpq(z_1)\,\EPqki(z_2)\nn
&& \left\lbrace F^{D}_{VPII}(z1)\,\left[\sum_\mu\,\sum_m\,\gamma_m\,F^\mu_{mQII}(z_1)\,F^{\bar{\mu}}_{mQII}(z_2)\,\Theta_\mu(z_1,z_2)\right] \right.\nn
&&\left.+\tilde{\gamma}\,\tilde{F}^D_{VPII}(z_1)\left[\sum_\mu\,\tilde{F}^{\mu}_{VQII}(z_1)\,F^{\bar{\mu}}_{VQII}(z_2)\,\Theta_\mu(z_1,z_2) \right]\right\rbrace\,F^D_{HKII}(z_2)
\tea


where $\gamma_H = \mathbf{K}\cdot\left(\hat{p}\times\hat{q}\right)\,(\hat{q}\cdot\hat{k})$, $\gamma_V =- \left(\hat{p}\cdot\hat{q}\right)\,\mbK\cdot(\hat{q}\times\hat{k})$ and $\tilde{\gamma} = p\,q\frac{QII\,PII}{P^2\,Q^2}\,\mbK\cdot(\hat{q}\times\hat{k})$.

The above expression can be rearranged as follows:

\bea
S^{(2)}_{VH}(z) &=&- \sqrt{2KI}\left(\frac{\omega}{c}\right)^4\,F^{UP}_{V PI}(z)\,\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz_2\,\int \frac{d^2q}{(2\pi)^2}\EPpq(z_1)\,\EPqki(z_2)\nn
&& \sum_\mu\,\sum_m\,\gamma_m\,F^{D}_{V PII}(z1)\,F^\mu_{m QII}(z_1)\,F^{\bar{\mu}}_{m QII}(z_2)\,F^D_{H KII}(z_2)\,\Theta_\mu(z_1,z_2) \label{VH_O2}
\tea

where the index $m$ takes three values $\left\lbrace H, V, \tilde{V}_1 \right\rbrace$: the last index means that the two functions $F(z_1)$ have a tilde.

Thus, for the TE case, both scattered fields have the same functional expression. This issue will be important when we compute mean energy flux of each channel.


\subsection{TM Incident Mode}

To get HV channel we start from the dynamic equation given by (\ref{vpp_O2}) but we must give the corresponding current, $J^{(2)}_{HV}$:


\bea
J^{(2)}_{HV\mbp}(z) &=& \left(\frac{\omega}{c}\right)^2\,\int\,\frac{d^2q}{(2\pi)^2}\,\EPpq(z)\,\left[\hat{p}\cdot\hat{q}\,\vpq^{(1)}(z)+\mbK\cdot\left(\hat{p}\times\hat{q}\right)\,\psiq^{(1)}(z)\right]\nn
&& \nn
J^{(2)}_{HV\mbp}(z) &=&  \sqrt{2K_I}\,\left(\frac{\omega}{c}\right)^4\,\int\,\frac{d^2q}{(2\pi)^2}\,\EPpq(z)\,\int^0_{-h}\,dz'\,\EPqki(z')\nn
&& \left[(\hat{p}\cdot\hat{q})\,\mbK\cdot(\hat{q}\times\hat{k})\,\sum_\mu\,F^\mu_{H QII}(z)\,F^{\bar{\mu}}_{H QII}(z')\,F^{D}_{V KII}(z')\,\Theta_\mu(z,z')\right.\nn
&&\left. +\mbK\cdot\left(\hat{p}\times\hat{q}\right)\,\left(\hat{q}\cdot\hat{k}\right)\,\sum_{\mu}\,F^\mu_{V QII}(z)\,F^{\bar{\mu}}_{V QII}(z')\,F^{D}_{V KII}(z')\,\Theta_\mu(z,z') \right. \nn 
&& \left. -\mbK\cdot\left(\hat{p}\times\hat{q}\right)\,\frac{q\,k}{QII\,KII}\,\sum_\mu F^\mu_{V QII}(z)\,\tilde{F}^{\bar{\mu}}_{V QII}(z')\,\tilde{F}^{D}_{V KII}(z')\right]
\tea

Here we again use three indexes to reduce the notation: $m=\left\lbrace H, V, \tilde{V}_2\right\rbrace$; we define the coefficients $\left\lbrace \delta_H; \delta_V, \delta_{\tilde{V}2} \right\rbrace = \left\lbrace (\hat{p}\cdot\hat{q})\,\mbK\cdot(\hat{q}\times\hat{k}); \mbK\cdot\left(\hat{p}\times\hat{q}\right)\,\left(\hat{q}\cdot\hat{k}\right); -\mbK\cdot\left(\hat{p}\times\hat{q}\right)\,\frac{q\,k}{QII\,KII} \right\rbrace$. Then we procedure as HH case and found:

\bea
S^{(2)}_{HV}(z) &=& -\sqrt{2K_I}\,\left(\frac{\omega}{c}\right)^4\,F^{UP}_{HPI}(z)\,\int\,\frac{d^2q}{(2\pi)^2}\,\int^0_{-h}\,dz_1\,\int^{Ls(z1)}_{Li(z1)}\,dz_2\,\,\EPpq(z_1)\,\EPqki(z_2)\nn
&& \sum_\mu\,\sum_m\,\delta_m\,F^{D}_{HPII}(z_1)\,F^\mu_{mQII}(z_1)\,F^{\hat{\mu}}_{mQII}(z_2)\,F^{D}_{V KII}(z_2)\,\Theta_\mu(z_1,z_2) \label{HV_O2}
\tea


The VV channel is obtained from (\ref{psi_O2}) using the following current:

\bea
&& J^{(2)}_{VV\mbp}(z) = \left(\frac{\omega}{c}\right)^2\,\int\,\frac{d^2q}{(2\pi)^2}\,\EPpq(z)\,\left[-\mbK\cdot\left(\hat{p}\times\hat{q}\right)\,\vpq^{(1)}(z)+\hat{p}\cdot\hat{q}\,\psiq^{(1)}(z)\right]\nn
&& +\imath p\frac{\partial}{\partial z}\left(\frac{\omega}{c}\right)^2\frac{1}{P^2}\int\,\frac{d^2q}{(2\pi)^2}\EPpq(z)\,\imath\frac{q}{Q^2}\frac{d}{dz}\psi^{(1)}_\mbq(z) \nn 
&& J^{(2)}_{VV\mbp}(z) =-\sqrt{2KI} \left(\frac{\omega}{c}\right)^4\,\int\,\frac{d^2q}{(2\pi)^2}\,\EPpq(z)\,\int dz'\,\EPqki(z')\nn 
&& \left\lbrace \sum_\mu\,\sum_m \eta_m\,F^\mu_{mQII}(z)\,F^{\bar{\mu}}_{mQII}(z')\,F^D_{VKII}(z')\,\Theta_\mu(z,z') \right. \nn && \left. -\left(\hat{p}\cdot\hat{q}\right)\frac{p\,k}{PII\,KII}\,\sum_\mu F^\mu_{VQII}(z)\,\tilde{F}^{\bar{\mu}}_{VQII}(z')\,\tilde{F}^D_{VKII}(z')\,\Theta_\mu(z,z')\right\rbrace \nn
&& +\imath p\,\sqrt{2KI} \left(\frac{\omega}{c}\right)^4\,\frac{\partial}{\partial z}\frac{1}{P^2II} \int \frac{d^2q}{(2\pi)^2}\EPpq(z)\,\frac{\imath q}{Q^2II}\frac{\partial}{\partial z}\psi^{(1)}_\mbq(z)
\tea

The three first terms can be rearranged as we did for the VH channel using the index $m=\left\lbrace H, V, \tilde{V}_2 \right\rbrace$. The last term needs to be integrated twice; this will produce a term proportional to $\tilde{F}$ for the two functions evaluated at $z_1$ (then we add a index $m=\tilde{V}_1$ and a term where the four $F$ functions have tilde (index $m=\tilde{V}_{12}$). Summarizing, the amplitude for the scattered field in VV case results:


\bea
S^{(2)}_{VV}(z) &=& \sqrt{2K_I}\,\left(\frac{\omega}{c}\right)^4\,F^{UP}_{VPI}(z)\,\int\,\frac{d^2q}{(2\pi)^2}\,\int^0_{-h}\,dz_1\,\int^{Ls(z1)}_{Li(z1)}\,dz_2\,\,\EPpq(z_1)\,\EPqki(z_2)\nn
&& \sum_\mu\,\sum_m\,\eta_m\,F^{D}_{HPII}(z_1)\,F^\mu_{mQII}(z_1)\,F^{\hat{\mu}}_{mQII}(z_2)\,F^{D}_{V KII}(z_2)\,\Theta_\mu(z_1,z_2) \label{VV_O2}
\tea

Here the index $m$ takes five values: $\left\lbrace H, V, \tilde{V}_1, \tilde{V}_2, \tilde{V}_{12} \right\rbrace$; the last index means that the four functions $F$ with polarization $V$ have tilde. The geometric coefficients are: 

\bea
&& \left\lbrace
\eta_H, \eta_V, \eta_{\tilde{V}1}, \eta_{\tilde{V}2}, \eta_{\tilde{V}12} \right\rbrace =  \nn 
&& \left\lbrace -\mbK\cdot(\hat{p}\times\hat{q})\,\mbK\cdot(\hat{q}\times\hat{k}), (\hat{p}\cdot\hat{q})\,(\hat{q}\cdot\hat{k}), -\frac{(\hat{p}\cdot\hat{q})\,p\,k}{PII\,KII}, \frac{(\hat{q}\cdot\hat{k})\,p\,q}{PII\,QII},-\frac{p\,q^2\,k}{PII\,Q^2II\,KII} \right\rbrace. \nonumber
\tea 



\subsection{Computing mean values}

As we shown in equations (\ref{HH_O2}), (\ref{VH_O2}), (\ref{VH_O2}) and (\ref{VV_O2}), the four channels can be written as

\bea
&& S^{(2)}_{ab}(z) = -\sqrt{2K_I}\,\left(\frac{\omega}{c}\right)^4\,F^{UP}_{aPI}(z)\nn 
&&\int\,\frac{d^2q}{(2\pi)^2}\,\int^0_{-h}\,dz_1\,\int^{Ls(z1)}_{Li(z1)}\,dz_2\,\,\EPpq(z_1)\,\EPqki(z_2)\,
\sum_{\mu,m}\,F^{D}_{aPII}(z_1)\,\mathcal{H}^{\mu,m}_{\mbp,\mbq}(z_1,z_2)\,F^{D}_{bKII}(z_2)
\tea

where the index $a\,,\,b$ indicate the polarization of scattered and incident waves, respectively. 

Mean value:

\bea
&& \langle S^{(2)}_{ab}(z) \rangle = -\sqrt{2K_I}\,\left(\frac{\omega}{c}\right)^4\,F^{UP}_{a PI}(z)\nn 
&& \int\,\frac{d^2q}{(2\pi)^2}\,\int^0_{-h}\,dz_1\,\int^{Ls(z1)}_{Li(z1)}\,dz_2\,\langle \EPpq(z_1)\,\EPqki(z_2)\rangle 
\sum_{\mu,m}\,F^{D}_{a PII}(z_1)\,\mathcal{H}^{\mu,m}_{\mbp,\mbq}(z_1,z_2)\,F^{D}_{b KII}(z_2) \nn
&& \langle S^{(2)}_{ab}(z) \rangle = -\delta(\mbp-\mbk)\,\sqrt{2K_I}\,\left(\frac{\omega}{c}\right)^4\,F^{UP}_{a PI}(z)\nn 
&&\int\,\frac{d^2q}{(2\pi)^2}\,\int^0_{-h}\,dz_1\,\int^{Ls(z1)}_{Li(z1)}\,dz_2\,C_{\mbp-\mbq}(z_1-z_2) 
\sum_{\mu,m}\,F^{D}_{a PII}(z_1)\,\mathcal{H}^{\mu,m}_{\mbp,\mbq}(z_1,z_2)\,F^{D}_{b KII}(z_2) 
\tea 

just in the specular direction, as we expected.

Mean energy:

\bea
&& \langle |S^{(2)}_{ab}(z)|^2 \rangle = 2K_I\,\left(\frac{\omega}{c}\right)^8\,|F^{UP}_{a PI}(z)|^2\nn 
&& \int\,\frac{d^2q}{(2\pi)^2}\,\int\,\frac{d^2q'}{(2\pi)^2}\,\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz'_1\,\int^{Ls(z1)}_{Li(z1)}\,dz_2\,\int^{Ls(z'_1)}_{Li(z'_1)}\,dz'_2
\langle \EPpq(z_1)\,\EPqki(z_2)\, \epsilon^*_{\mbp-\mbq'}(z'_1)\,\epsilon^*_{\mbq'-\mbki}(z'_2)\rangle \nn
&& \left[\sum_{\mu,m}\,F^{D}_{a PII}(z_1)\,\mathcal{H}^{\mu,m}_{\mbp,\mbq}(z_1,z_2)\,F^{D}_{b KII}(z_2)\right]\,
\left[\sum_{\mu',m'}\,F^{D}_{a PII}(z'_1)\,\mathcal{H}^{\mu',m'}_{\mbp,\mbq'}(z'_1,z'_2)\,F^{D}_{b KII}(z'_2)\right]^*
\nonumber
\tea 

\bea
&&\langle |S^{(2)}_{ab}(z)|^2 \rangle = 2K_I\,\left(\frac{\omega}{c}\right)^8\,|F^{UP}_{a PI}(z)|^2\,\int\,\frac{d^2q}{(2\pi)^2}\,\int\,\frac{d^2q'}{(2\pi)^2}\,\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz'_1\,\int\,dz_2\,\int\,dz'_2\nn
&& \left[\left(\delta\left(\mbp-\mbki\right)\right)^2\,C_{\mbp-\mbq}(z_1-z_2)\,C_{\mbp-\mbq'}(z'_1-z'_2) 
+ \left(\delta\left(\mbq-\mbq'\right)\right)^2\,C_{\mbp-\mbq}(z_1-z'_1)\,C_{\mbq-\mbki}(z_2-z'_2) \right. \nn 
&& \left. +\left(\delta\left(\mbp+\mbki-\mbq-\mbq'\right)\right)^2\,C_{\mbp-\mbq}(z_1-z'_2)\,C_{\mbq-\mbki}(z_2-z'_1)  \right] \nn
&& \left[\sum_{\mu,m}\,F^{D}_{a PII}(z_1)\,\mathcal{H}^{\mu,m}_{\mbp,\mbq}(z_1,z_2)\,F^{D}_{b KII}(z_2)\right]\,
\left[\sum_{\mu',m'}\,F^{D}_{a PII}(z'_1)\,\mathcal{H}^{\mu',m'}_{\mbp,\mbq'}(z'_1,z'_2)\,F^{D}_{b KII}(z'_2)\right]^*
\tea 

\bea
&& \langle |S^{(2)}_{ab}(z)|^2 \rangle = \big\vert \langle S^{(2)}_{ab}(z) \rangle \big\vert^2 +  2K_I\,\left(\frac{\omega}{c}\right)^8\,|F^{UP}_{a PI}(z)|^2\,
\int\,\frac{d^2q}{(2\pi)^2}\,\int\,\frac{d^2q'}{(2\pi)^2}\,\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz'_1\,\int\,dz_2\,\int\,dz'_2\nn
&& \sum_{\mu,m}\,\,\sum_{\mu',m'}\,\left[\left(\delta\left(\mbq-\mbq'\right)\right)^2\,C_{\mbp-\mbq}(z_1-z'_1)\,C_{\mbq-\mbki}(z_2-z'_2) \right.\nn 
&& \left. +\left(\delta\left(\mbp+\mbki-\mbq-\mbq'\right)\right)^2\,C_{\mbp-\mbq}(z_1-z'_2)\,C_{\mbq-\mbki}(z_2-z'_1)  \right]\nn
&& \left[F^{D}_{a PII}(z_1)\,\mathcal{H}^{\mu,m}_{\mbp,\mbq}(z_1,z_2)\,F^{D}_{b KII}(z_2)\right]\,
\left[ F^{D}_{a PII}(z'_1)\,\mathcal{H}^{\mu',m'}_{\mbp,\mbq'}(z'_1,z'_2)\,F^{D}_{b KII}(z'_2)\right]^*
\tea 

Incoherent scattered field:

\bea
&& \langle |S^{(2)}_{ab}(z)|^2 \rangle - \big\vert \langle S^{(2)}_{ab}(z) \rangle \big\vert^2 =  
 2K_I\,\left(\frac{\omega}{c}\right)^8\,|F^{UP}_{a PI}(z)|^2\nn
&& \int\,\frac{d^2q}{(2\pi)^2}\,\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz'_1\,\int\,dz_2\,\int\,dz'_2\,
\,\left[\mathcal{L}_{ab}(z1-z'_1,z_2-z'_2) + \mathcal{C}_{ab}(z_1-z'_2,z_2-z'_1) \right] \nn 
\tea 

with

\bea 
&& \mathcal{L}_{ab}(z_1-z'_1,z_2-z'_2) = C_{\mbp-\mbq}(z_1-z'_1)\,C_{\mbq-\mbki}(z_2-z'_2)\nn
&&\sum_{\mu,m}\,\sum_{\mu',m'}\, \left[F^{D}_{a PII}(z_1)\,\mathcal{H}^{\mu,m}_{\mbp,\mbq}(z_1,z_2)\,F^{D}_{b KII}(z_2)\right]\,\left[ F^{D}_{a PII}(z'_1)\,\mathcal{H}^{\mu',m'}_{\mbp,\mbq}(z'_1,z'_2)\,F^{D}_{b KII}(z'_2)\right]^* \\
&& \nn
&& \mathcal{C}_{ab}(z_1-z'_2,z_2-z'_1) = C_{\mbp-\mbq}(z_1-z'_2)\,C_{\mbq-\mbki}(z_2-z'_1) \nn
&& \sum_{\mu,m}\,\sum_{\mu',m'}\,\left[F^{D}_{a PII}(z_1)\,\mathcal{H}^{\mu,m}_{\mbp,\mbq}(z_1,z_2)\,F^{D}_{b KII}(z_2)\right]\,
\left[ F^{D}_{a PII}(z'_1)\,\mathcal{H}^{\mu',m'}_{\mbp,\mathbf{r}}(z'_1,z'_2)\,F^{D}_{b KII}(z'_2)\right]^*
\tea

where $\mathbf{r} = \mbp + \mbk - \mbq$. 

\begin{figure}[H]
\centering
\includegraphics[width = 0.45\textwidth]{figures/ladder.png}\hspace{0.5cm}
\includegraphics[width = 0.45\textwidth]{figures/crossed.png}
\caption{Ladder and Crossed graphs.}
\end{figure}


Escribo de forma explicita los terminos ladder y cross para el canal $rs$.

Recordar que el indice $\mu=\{UP, DOWN\}$ indica propagacion (y que si $\mu = UP\,\,\Rightarrow \bar{\mu} = DOWN$ y viceversa). El indice $m={H,V}$ indica polarizacion. 

\vspace{2cm}

\textbf{Ladder term}

\bea
&& \mathcal{L}_{ab} =  2K_I\,\left(\frac{\omega}{c}\right)^8\,|F^{UP}_{a\,PI}(z)|^2 \int\,\frac{d^2q}{(2\pi)^2}\,\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz_2\,\int\,dz'_1\,\int\,dz'_2\nn  && \sum_{\mu,m}\,\,\sum_{\mu',m'}\, C_{\mbp-\mbq}(z_1-z'_1)\,C_{\mbq-\mbki}(z_2-z'_2)\nn
&& \left[F^{D}_{a\,PII}(z_1)\,
\beta_m\,F^\mu_{m\,QII}(z_1)\,F^{\bar{\mu}}_{m\,QII}(z_2)\,\Theta_\mu(z_1,z_2)
\,F^{D}_{b\,KII}(z_2)\right]\nn
&&\left[ F^{D}_{a\,PII}(z'_1)\,
\beta_{m'}\,F^{\mu'}_{m'\,QII}(z'_1)\,F^{\bar{\mu}'}_{m'\,QII}(z'_2)\,\Theta_{\mu'}(z'_1,z'_2)F^{D}_{b\,KII}(z'_2)\right]^*
\tea 

% \bea
% && \langle L_{HH} \rangle  =  2K_I\,\left(\frac{\omega}{c}\right)^8\,\frac{1}{2PI} \int_{q\leq Q}\,\frac{d^2q}{(2\pi)^2}\,\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz'_1\,\int\,dz_2\,\int\,dz'_2\nn 
% && \exp{\left[-l^2_r\,(\mbp-\mbq)^2\right]}\,\exp{\left[-(z_1-z'_1)^2/l^2_z\right]}\,
% \exp{\left[-l^2_r\,(\mbq-\mbki)^2\right]}\,\exp{\left[-(z_2-z'_2)^2/l^2_z\right]}\nn
% && F^{D}_{H\,PII}(z_1)\,
% \sum_\mu\,\left\lbrace (\hat{p}\cdot\hat{q})(\hat{q}\cdot\hat{k})\,F^\mu_{H\,QII}(z_1)\,F^{\bar{\mu}}_{H\,QII}(z_2) -\hat{z}\cdot(\hat{p}\times\hat{q})\,\hat{z}\cdot(\hat{q}\times\hat{k})\,F^\mu_{V\,QII}(z_1)\,F^{\bar{\mu}}_{V\,QII}(z_2) \right\rbrace\,\Theta_\mu(z_1,z_2)\,F^{D}_{H\,KII}(z_2)\nn
% && F^{D*}_{H\,PII}(z'_1)\,
% \sum_{\mu'}\,\left\lbrace (\hat{p}\cdot\hat{q})(\hat{q}\cdot\hat{k})\,F^\mu_{H\,QII}(z'_1)\,F^{\bar{\mu}}_{H\,QII}(z'_2) -\hat{z}\cdot(\hat{p}\times\hat{q})\,\hat{z}\cdot(\hat{q}\times\hat{k})\,F^\mu_{V\,QII}(z'_1)\,F^{\bar{\mu}}_{V\,QII}(z'_2) \right\rbrace^*\,\Theta_{\mu'}(z'_1,z'_2)\,F^{D\,*}_{H\,KII}(z'_2) \nonumber
% \tea 

% donde $\Theta_D(z_1,z_2) = \Theta(z_1-z_2)$ y $\Theta_{UP}(z_1,z_2) = \Theta(z_2-z_1)$ y $Q = \sqrt{\epsilon_1} k_i$ es el limite de integracion en  $d^2q$. 
% Las funciones de Green están listadas en (20) y (21) para la polarizacion H y en (23) y (24) para la polarizacion V. Cada funcion tiene dos terminos, uno proporcional a $\exp{(\imath q z)}$ y otro a $\exp{(-\imath q z)}$, con el $q$ que corresponda.


\textbf{Cross term}

\bea
&& \mathcal{C}_{ab} =  2K_I\,\left(\frac{\omega}{c}\right)^8\,|F^{UP}_{a\,PI}(z)|^2 \int\,\frac{d^2q}{(2\pi)^2}\,\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz_2\,\int\,dz'_1\,\int\,dz'_2\nn  && \sum_{\mu,m}\,\,\sum_{\mu',m'}\, C_{\mbp-\mbq}(z_1-z'_2)\,C_{\mbq-\mbki}(z_2-z'_1)\nn
&& \left[F^{D}_{a\,PII}(z_1)\,
\beta_m\,F^\mu_{m\,QII}(z_1)\,F^{\bar{\mu}}_{m\,QII}(z_2)\,\Theta_\mu(z_1,z_2)
\,F^{D}_{b\,KII}(z_2)\right]\nn
&&\left[ F^{D}_{a\,PII}(z'_1)\,
\beta_{m'}\,F^{\mu'}_{m'\,RII}(z'_1)\,F^{\bar{\mu}'}_{m'\,RII}(z'_2)\,\Theta_{\mu'}(z'_1,z'_2)F^{D}_{b\,KII}(z'_2)\right]^*
\tea 


siendo $RII = \sqrt{\epsilon_{0II} k^2_i - \mathbf{r}^2}$ con $\mathbf{r}= \mbki + \mbp - \mbq$.

% \bea
% && \langle \mathcal{C}_{HH} \rangle  =  2K_I\,\left(\frac{\omega}{c}\right)^8\,\frac{1}{2PI} \int_{q\leq Q}\,\frac{d^2q}{(2\pi)^2}\,\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz'_1\,\int\,dz_2\,\int\,dz'_2\nn 
% && C_{\mbp-\mbq}(z_1-z'_2)\,C_{\mbq-\mbki}(z_2-z'_1)\nn
% && F^{D}_{H\,PII}(z_1)\,
% \sum_\mu\,\left\lbrace (\hat{p}\cdot\hat{q})(\hat{q}\cdot\hat{k})\,F^\mu_{H\,QII}(z_1)\,F^{\bar{\mu}}_{H\,QII}(z_2) -\hat{z}\cdot(\hat{p}\times\hat{q})\,\hat{z}\cdot(\hat{q}\times\hat{k})\,F^\mu_{V\,QII}(z_1)\,F^{\bar{\mu}}_{V\,QII}(z_2) \right\rbrace\,\Theta_\mu(z_1,z_2)\,F^{D}_{H\,KII}(z_2)\nn
% && F^{D*}_{H\,PII}(z'_1)\,
% \sum_{\mu'}\,\left\lbrace (\hat{p}\cdot\hat{r})(\hat{r}\cdot\hat{k})\,F^\mu_{H\,RII}(z'_1)\,F^{\bar{\mu}}_{H\,RII}(z'_2) -\hat{z}\cdot(\hat{p}\times\hat{r})\,\hat{z}\cdot(\hat{r}\times\hat{k})\,F^\mu_{V\,RII}(z'_1)\,F^{\bar{\mu}}_{V\,RII}(z'_2) \right\rbrace^*\,\Theta_{\mu'}(z'_1,z'_2)\,F^{D\,*}_{H\,KII}(z'_2) \nonumber
% \tea 



Ahora hay que expandir la suma en $\mu, \mu' =\{\text{UP},\text{DOWN}\} = \{ \UPa, \DWa\}$ en el término ladder y en el término cross. Cada uno contribuye con 16 términos:

\bea
\mathcal{L}_{ab}  &=& \sum_{\mu,\mu'}\,\sum_{m,m'}\,I_{ab,\,mm',\,\mu\mu'} \nn
&=&   I_{ab\,HH,\UPa\,\UPa} + I_{ab\,HH,\UPa\,\DWa} + I_{ab\,HH,\DWa\,\UPa} + I_{ab\,HH,\DWa\,\DWa} \nn
&+&  I_{ab\,HV,\UPa\,\UPa} + I_{ab\,HV,\UPa\,\DWa} + I_{ab\,HV,\DWa\,\UPa} + I_{ab\,HV,\DWa\,\DWa} \nn
&+&  I_{ab\,VH,\UPa\,\UPa} + I_{ab\,VH,\UPa\,\DWa} + I_{ab\,VH,\DWa\,\UPa} + I_{ab\,VH,\DWa\,\DWa} \nn
&+&  I_{ab\,VV,\UPa\,\UPa} + I_{ab\,VV,\UPa\,\DWa} + I_{ab\,VV,\DWa\,\UPa} + I_{ab\,VV,\DWa\,\DWa} \label{combinetas_O2}
\tea

Los términos $HV$ y $VH$ deberían ser complejos conjugados, así que en principio hay que calcular doce términos que conllevan integrales 6D. Entonces, sumando ladder y cross, para completar el canal $ab$ tenemos que hacer 24 integrales 6D. 

Para completar el cálculo de la energía retrodispersada aplicaremos fase estacionaria con el fin de eliminar las integrales sobre funciones oscilatorias y llegar a una expresión aproximada en donde solo haya que integrar en la variable de impulso intermedia $\mathbf{q}$.



\subsection{Fase estacionaria all' uso nostro}

Cada función $F$ que se propaga en dirección $\mu$ a través del medio $II$, tiene polarización $m$ y está evaluada en el modo $Q$, es de la forma: 

\bea
&& F^\mu_{m\,Q}(z) = f_m(Q)\,\left[r^\mu_m(Q)\,e^{\imath Q z}+t^\mu_m(Q)\,e^{-\imath Q z}\right]  \nn 
&& F^\mu_{m\,Q}(z) = f_m(Q)\,\sum_{s=\pm 1}\,X^{\mu s}_{m\,Q}\,e^{\imath s Q z }\nn 
&& \tilde{F}^\mu_{m\,Q}(z) = f_m(Q)\,\sum_{s=\pm 1}\,s\,X^{\mu s}_{m\,Q}\,e^{\imath s Q z }\nn 
&& \text{siendo:} X^{\mu\,+1}_{m\,Q} = r^{\mu}_m(Q)\,\,,\,\,X^{\mu\,-1}_{m\,Q} = t^{\mu}_m(Q) \label{Fmu_compacta}
\tea

Desarrollo el término ladder:

\bea
&& \langle \mathcal{L}_{ab} \rangle  =  2K_I\,\left(\frac{\omega}{c}\right)^8\,|F^{UP}_{a\,PI}(z)|^2 \int\,\frac{d^2q}{(2\pi)^2}\,\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz_2\,\int\,dz'_1\,\int\,dz'_2\nn 
&& \sum_{s_1\,s_2}\,\sum_{\mu,m,s_\mu,s_{\bar{\mu}}}\,\,\sum_{\mu',m',s'_\mu,s'_{\bar{\mu}}}\,\sum_{s'_1\,s'_2}\,\, C_{\mbp-\mbq}(z_1-z'_1)\,C_{\mbq-\mbki}(z_2-z'_2)\,\Theta\left(s_\mu(z_1-z_2)\right)\,\Theta\left(s'_{\mu}(z'_1-z'_2)\right)\nn
&&\beta_m\,f_{a}(PII)\,f_{m}(QII)\,f_m(QII)\,f_{b}(KII)\,
\left[\beta_{m'}\,f_{a}(PII)\,f_{m'}(QII)\,f_{m'}(QII)\,f_{b}(KII) \right]^*\nn
&& X^{D\,s_1}_{a\,PII}\,X^{\mu\,s_\mu}_{m\,QII}\,X^{\bar{\mu}\,s_{\bar{\mu}}}_{m\,QII}\,X^{D\,s_2}_{b\,KII}\,
\left[ X^{D\,s'_1}_{a\,PII}\,X^{\mu'\,s'_{\mu}}_{m'\,QII}\,X^{\bar{\mu}'\,s'_{\bar{\mu}}}_{m'\,QII}\,X^{D\,s'_2}_{b\,KII} \right]^*\nn 
&&e^{\imath (s_1\,PII + s_\mu\,QII)z_1}\,e^{\imath (s_{\bar{\mu}}\,QII + s_2\,KII)z_2}\,
e^{-\imath (s'_1\,PII + s'_\mu\,QII)z'_1}\,e^{-\imath (s'_{\bar{\mu}}\,QII + s'_2\,KII)z'_2}
\tea

Busco los puntos de fase estacionaria: para eliminar la oscilación sobre $z_1$ necesito $s_\mu = -s_1$ (luego $PII=QII$) y para eliminar la oscilación sobre $z_2$ hay que pedir $s_2 = -s_{\bar{\mu}}$ (luego $QII = KII$); condiciones análogas salen sobre las variables primadas. Simplificamos las sumas sobre los índicces $\left\lbrace s_\mu, s_{\bar{\mu}}, s'_\mu, s'_{\bar{\mu}} \right\rbrace $.

\bea
&& \langle \mathcal{L}_{ab} \rangle  =  2K_I\,\left(\frac{\omega}{c}\right)^8\,|F^{UP}_{a\,PI}(z)|^2 \int\,\frac{d^2q}{(2\pi)^2}\,\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz_2\,\int\,dz'_1\,\int\,dz'_2\nn 
&& \sum_{s_1\,s_2}\,\sum_{\mu,m}\,\,\sum_{\mu',m'}\,\sum_{s'_1\,s'_2}\,\, C_{\mbp-\mbq}(z_1-z'_1)\,C_{\mbq-\mbki}(z_2-z'_2)\,\Theta\left(s_1(z_1-z_2)\right)\,\Theta\left(s'_1(z'_1-z'_2)\right)\nn
&&\beta_m\,\beta^*_{m'}\,|f_{a}(PII)|^2\,|f_m(QII)|^2\,|f_{m'}(QII)|^2\,|f_{b}(KII)|^2
\nn
&& X^{D\,s_1}_{a\,PII}\,X^{\mu\,-s_1}_{m\,QII}\,X^{\bar{\mu}\,-s_2}_{m\,QII}\,X^{D\,s_2}_{b\,KII}\,
\left[ X^{D\,s'_1}_{a\,PII}\,X^{\mu'\,-s'_1}_{m'\,QII}\,X^{\bar{\mu}'\,-s'_2}_{m'\,QII}\,X^{D\,s'_2}_{b\,KII} \right]^*\,
e^{\imath (PII-QII)(s_1\,z_1-s'_1\,z'_1)}\,e^{\imath(QII-\,KII)(s_2\,z_2-s'_2\,z'_2)}
\tea


Cambiamos variables: $z_j = \xi_j + \frac{1}{2} \psi_j$, $z'_j = \xi_j - \frac{1}{2} \psi_j$. 


\bea
&& \langle \mathcal{L}_{ab} \rangle  =  2K_I\,\left(\frac{\omega}{c}\right)^8\,|F^{UP}_{a\,PI}(z)|^2 \int\,\frac{d^2q}{(2\pi)^2}\,\int^0_{-h}\,d\xi_1\,\int^h_{-h}\,d\psi_1\,\int\,d\xi_2\,\int\,d\psi_2\nn 
&& \sum_{s_1\,s_2}\,\sum_{\mu,m}\,\,\sum_{\mu',m'}\,\sum_{s'_1\,s'_2}\,\, C_{\mbp-\mbq}(\psi_1)\,C_{\mbq-\mbki}(\psi_2)\,\Theta\left(s_1(\xi_1-\xi_2+\frac{1}{2}(\psi_1-\psi_2))\right)\,\Theta\left(s'_1(\xi_1-\xi_2-\frac{1}{2}(\psi_1-\psi_2))\right)\nn
&&\beta_m\,\beta^*_{m'}\,\,|f_{a}(PII)|^2\,|f_m(QII)|^2\,|f_{m'}(QII)|^2\,|f_{b}(KII)|^2
\nn
&& X^{D\,s_1}_{a\,PII}\,X^{\mu\,-s_1}_{m\,QII}\,X^{\bar{\mu}\,-s_2}_{m\,QII}\,X^{D\,s_2}_{b\,KII}\,
\left[ X^{D\,s'_1}_{a\,PII}\,X^{\mu'\,-s'_1}_{m'\,QII}\,X^{\bar{\mu}'\,-s'_2}_{m'\,QII}\,X^{D\,s'_2}_{b\,KII} \right]^*\nn 
&&e^{\imath (PII-QII)(s_1-s'_1)\xi_1}\,e^{\imath \frac{1}{2}(PII-QII)(s_1+s'_1)\psi_1}\,
e^{\imath(QII-\,KII)(s_2-s'_2)\xi_2}\,e^{\imath \frac{1}{2}(QII-\,KII)(s_2+s'_2)\psi_2}
\tea

Observaciones:

\begin{itemize}
    \item Si $s_j = s'_j$ las integrales sobre $\xi_j$ toman su màximo valor;

    \item  Cuando $\mu =\text{UP} \Rightarrow z_1 - z_2 > 0 \Rightarrow 2(\xi_1 - \xi_2) > \psi_2 - \psi_1$; y cuando $\mu' =\text{UP} \Rightarrow z'_1 - z'_2 > 0 \Rightarrow 2(\xi_1 - \xi_2) > \psi_1 - \psi_2$. Condición análoga se da cuando $\mu = \mu' = \text{DOWN}$. En ambos casos la condición $\psi_1 = \psi_2 = 0$ pertenece al dominio de integración y da la máxima contribución a la integral ya que sobre las variables $\psi$ se anulan las oscilaciones. 

    \item Cuando $\mu =\text{UP} \Rightarrow z_1 - z_2 > 0 \Rightarrow 2(\xi_1 - \xi_2) > \psi_2 - \psi_1$; y cuando $\mu' =\text{DOWN} \Rightarrow z'_1 - z'_2 < 0 \Rightarrow 2(\xi_1 - \xi_2) < \psi_1 - \psi_2$. Condición análoga se da cuando $\mu = \text{DOWN}$ y $\mu' = \text{UP}$. En ambos casos la condición $\psi_1 = \psi_2 = 0$ NO pertenece al dominio de integración y por lo tanto esta combianción de modos de propagación será subdominante en el aporte total al término ladder.
\end{itemize}

Por lo antedicho en los dos apartados de arriba, de la ecuación (\ref{combinetas_O2}) solo nos quedaremos con la mitad de los términos: todos aquellos que sean UP-UP y DOWN-DOWN sumando todas las combinaciones posibles de polarización para las ondas propagantes en el medio II, los que nos dará un total de 8 combinaciones (o 6 si mostramos que el caso HV es igual al VH para las ondas en el medio II; recordar que en (\ref{combinetas_O2}) los índices $ab$ indican polarización de onda dispersada e incidente, respectivamente).

\bigskip

El término
ladder, usando que $\mu = \mu'$, $s_1 = s'_1$, $s_2 = s'_2$ y que una de las integrales sobre $\psi$ da un factor $2h$, se reduce a,

\bea
&& \langle \mathcal{L}_{ab} \rangle  =  2K_I\,\left(\frac{\omega}{c}\right)^8\,|F^{UP}_{a\,PI}(z)|^2 \int\,\frac{d^2q}{(2\pi)^2}\,\int^h_{-h}\,d\psi\,\int^0_{-h}\,d\xi_1\,\int^0_{-h}\,d\xi_2\,\nn 
&& \sum_{s_1\,s_2}\,\sum_{\mu,m,m'}\,\, C_{\mbp-\mbq}(\psi)\,C_{\mbq-\mbki}(\psi)\,\Theta\left(s_1(\xi_1-\xi_2)\right)\nn
&&\beta_m\,\beta^*_{m'}\,\,|f_{a}(PII)|^2\,|f_m(QII)|^2\,|f_{m'}(QII)|^2\,|f_{b}(KII)|^2
\nn
&& |X^{D\,s_1}_{a\,PII}|^2\,X^{\mu\,-s_1}_{m\,QII}\,X^{\bar{\mu}\,-s_2}_{m\,QII}\,
\,X^{*\mu\,-s_1}_{m'\,QII}\,X^{*\bar{\mu}\,-s_2}_{m'\,QII}\,|X^{D\,s_2}_{b\,KII}|^2\,
e^{\imath s_1(PII-QII)\psi}\,e^{\imath s_2(QII-\,KII)\psi}
\tea


Las integrales sobre $d\xi_1\,d\xi_2$ dan la mitad del área $[-h,0]\times[-h,0]$ debido a $\Theta\left(s_1(\xi_1-\xi_2)\right)$; para simplificar la integral sobre $\psi$ vamos a decir que la longitud de correlación vertical de las fluctuaciones en la cte dieléctrica es mucho menor que el espesor de la capa por lo que esa integral puede ser aproximada por la transformada de Fouirer de la función de correlación $C_\mathbf{p}(\psi)$. Así las cosas, llegamos a la expresión más compacta que podemos dar para el término ladder:


\bea
&& \langle \mathcal{L}_{ab} \rangle  =  2K_I\,\left(\frac{\omega}{c}\right)^8\,|F^{UP}_{a\,PI}(z)|^2\,h^3\,|f_{a}(PII)|^2\,|f_{b}(KII)|^2\,\int\,\frac{d^2q}{(2\pi)^2}\, 
\hat{C}_{\perp\,\mbp-\mbq}\,\hat{C}_{\perp\,\mbq-\mbki}\nn
&&\sum_{\mu,m\,m'}\,\beta_m\,\beta^*_{m'}\,|f_m(QII)|^2\,|f_{m'}(QII)|^2\nn
&&\sum_{s_1\,s_2}\, |X^{D\,s_1}_{a\,PII}|^2\,X^{\mu\,-s_1}_{m\,QII}\,X^{\bar{\mu}\,-s_2}_{m\,QII}\,
\,X^{*\mu\,-s_1}_{m'\,QII}\,X^{*\bar{\mu}\,-s_2}_{m'\,QII}\,|X^{D\,s_2}_{b\,KII}|^2\,\hat{C}_z(s_1(PII-QII)+s_2(QII-KII)) \label{casi_Ladder_ab}
\tea


La integral en la variable de momento $\mathbf{q}$ se realiza de manera numérica y parece que no tiene términos problemáticos (solo hay que analizar con detalle el caso $q=0$). Aquí se ve que el término ladder es real: cuando $m=m'$ todos los coeficientes $X$ aparecen como módulo cuadrado; cuando $m\neq m'$ se ve que sumando los casos complemetarios se obtiene dos veces la parte real de esos términos. Así que podemos reducir la expresión eliminando la suma sobre $m'$ y en el caso en que $m'\neq m$ se usa $m' = \bar{m}$ \footnote{en el canal HH es fácil: si $m=H \Rightarrow m' = V$ y viceversa; para el VH hay que tener mas cuidado: si $m=H \Rightarrow m' = V$ o $m' = \tilde{V}1$, con lo cual resulta más práctico usar la expresión (\ref{casi_Ladder_ab}); lo mismo ocurre para los canales HV y VV.}. Entonces,

\bea
&& \langle \mathcal{L}_{ab} \rangle  =  2K_I\,\left(\frac{\omega}{c}\right)^8\,|F^{UP}_{a\,PI}(z)|^2\,h^3\,|f_{a}(PII)|^2\,|f_{b}(KII)|^2\,\int\,\frac{d^2q}{(2\pi)^2}\, 
\hat{C}_{\perp\,\mbp-\mbq}\,\hat{C}_{\perp\,\mbq-\mbki}\nn
&& \sum_{\mu,m}\,\sum_{s_1\,s_2}\,\hat{C}_z(s_1(PII-QII)+s_2(QII-KII))\, |X^{D\,s_1}_{a\,PII}|^2\,\left[|f_m(QII)|^4\,|\beta_m|^2\,|X^{\mu\,-s_1}_{m\,QII}|^2\,|X^{\bar{\mu}\,-s_2}_{m\,QII}|^2  \right. \nn 
&& \left. + 2\Re\left\lbrace \beta_m\,\beta^*_{\bar{m}}\,|f_m(QII)|^2\,|f_{\bar{m}}(QII)|^2\,X^{\mu\,-s_1}_{m\,QII}\,X^{*\mu\,-s_1}_{\bar{m}\,QII}\,X^{\bar{\mu}\,-s_2}_{m\,QII}\,X^{*\bar{\mu}\,-s_2}_{\bar{m}\,QII} \right\rbrace  \right]\,|X^{D\,s_2}_{b\,KII}|^2
\label{Ladder_ab}
\tea



El término cross se analiza de manera similar. Los detalles a cambiar son: que uno de los modos auxiliares es $\mathbf{r} = \mathbf{k}+\mathbf{p}-\mathbf{q}$ y que las coordenadas verticales en las funciones de correlación se agrupan como $z_1-z'_2$ y $z_2-z'_1$. Debido a esto, los modos de propagación que contribuyen a la fase estacionaria son $\mu \neq \mu'$. El otro detalle a tener en cuenta es que se suprimen las oscilaciones solo cuando se está en la condición de bakcscattering ($\mathbf{p} = - \mathbf{k}$), lo que implica $\mathbf{r} = -\mathbf{q}$ y $RII = QII$. Así las cosas, el término cross se reduce a,



\bea
&& \langle \mathcal{C}_{ab} \rangle  =  2K_I\,\left(\frac{\omega}{c}\right)^8\,|F^{UP}_{a\,PI}(z)|^2\,h^3\,|f_{a}(PII)|^2\,|f_{b}(KII)|^2\,\int\,\frac{d^2q}{(2\pi)^2}\, 
\hat{C}_{\perp\,\mbp-\mbq}\,\hat{C}_{\perp\,\mbq-\mbki}\nn
&& \sum_{\mu,m}\,\sum_{s_1\,s_2}\, \hat{C}_z((s_1-s_2)(KII-QII))\,|X^{D\,s_1}_{a\,PII}|^2\,\left[|f_m(QII)|^4\,|\beta_m|^2\,|X^{\mu\,-s_1}_{m\,QII}|^2\,|X^{\bar{\mu}\,-s_2}_{m\,QII}|^2  \right. \nn 
&& \left. + 2\Re\left\lbrace \beta_m\,\beta^*_{\bar{m}}\,|f_m(QII)|^2\,|f_{\bar{m}}(QII)|^2\,X^{\mu\,-s_1}_{m\,QII}\,X^{*\mu\,-s_1}_{\bar{m}\,QII}\,X^{\bar{\mu}\,-s_2}_{m\,QII}\,X^{*\bar{\mu}\,-s_2}_{\bar{m}\,QII} \right\rbrace  \right]\,|X^{D\,s_2}_{b\,KII}|^2
\label{Cross_ab}
\tea

% \bea
% && \langle \mathcal{C}_{HH} \rangle  =  2K_I\,\left(\frac{\omega}{c}\right)^8\,|F^{UP}_{H\,PI}(z)|^2\,h^3\,\int\,\frac{d^2q}{(2\pi)^2}\, 
% \hat{C}_{\perp\,\mbki-\mbq}\,\hat{C}_{\perp\,\mbq-\mbki}\nn
% &&\sum_{\mu,m}\,|f_{D}(KII)|^2\,|f_{\mu}(QII)|^2\,|f_{\bar{\mu}}(QII)|^2\,|f_{D}(KII)|^2\nn
% &&\sum_{s_1\,s_2}\, |X^{D\,s_1}_{H\,KII}|^2\,\left[ |\beta_m|^2\,|X^{\mu\,-s_1}_{m\,QII}|^2\,|X^{\bar{\mu}\,-s_2}_{m\,QII}|^2  + 2\Re\left\lbrace \beta_m\,\beta^*_{\bar{m}}\,X^{\mu\,-s_1}_{m\,QII}\,X^{*\mu\,-s_1}_{\bar{m}\,QII}\,X^{\bar{\mu}\,-s_2}_{m\,QII}\,X^{*\bar{\mu}\,-s_2}_{\bar{m}\,QII} \right\rbrace  \right]\,|X^{D\,s_2}_{H\,KII}|^2\nn
% && \hat{C}_z((s_1-s_2)(KII-QII)) \label{Cross_HH}
% \tea


Cuando $PII=KII$ (i.e. backscattering) la expresión para el término cross coincide con el ladder.


Con las expresiones (\ref{Ladder_ab}) y (\ref{Cross_ab}) se pueden calcular los términos ladder y cross de los canales cuatro canales. Solo hay que tener en cuenta que, según el canal, el índice $m$ puede tomar uno o tres valores más (VH agrega $\tilde{V}_1$, HV $\tilde{V}_2$ y VV $\tilde{V}_1, \tilde{V}_2, \tilde{V}_{12}$) que aplican un $(-1)$ al coeficiente de transmisión de la función $F^\mu_{m\,Q}$ que depende de $z_{1}$, $z_{2}$ o de las variables primadas, según corresponda (esto quedó indicado en la expresión (\ref{Fmu_compacta})).

Así las cosas, tenemos expresiones amigables para la energía dispersada tanto a primer como segundo orden.

Estoy implementano las expresiones (\ref{Ladder_ab}) y (\ref{Cross_ab}) pero por ahora son poco eficientes en el tiempo de cálculo.











% \subsubsection{Fase estacionaria - 1era version}


% Así las cosas, llegamos a:

% \bea
% && I_{AB\,HH,\UPa\,\UPa} = 2K_I\left(\frac{\omega}{c}\right)^8\,\frac{1}{2PI}\,|f_{\DWa\,B}(KII)|^2\, \int_{q\leq Q}\,\frac{d^2q}{(2\pi)^2}\,|C_H(q)|^2\,|f_{\DWa\,H}(QII)|^2\, \exp{\left[-l^2_r(\mbp-\mbq)^2-l^2_r(\mbq-\mbki)^2\right]}\nn 
% &&\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)^*(z'_1)\nn
% && \int^{z_1}_{-h}\,dz_2\,\int^{z'_1}_{-h}\,dz'_2\,\rho(z_2-z'_2) \nn 
% &&\left[ |r_{\DWa\,H}(QII)|^2\,e^{\imath QII(z_2-z'_2)}+r_{\DWa\,H}(QII)\,t^*_{\DWa\,H}(QII)\,e^{\imath QII(z_2+z'_2)}\right.\nn
% &&\left. +t_{\DWa\,H}(QII)\,r^*_{\DWa\,H}(QII)\,e^{-\imath QII(z_2+z'_2)}+|t_{\DWa\,H}(QII)|^2\,e^{-\imath QII(z_2-z'_2)}\right]\nn
% &&\left[ |r_{\DWa\,B}(KII)|^2\,e^{\imath KII(z_2-z'_2)}+r_{\DWa\,B}(KII)\,t^*_{\DWa\,B}(KII)\,e^{\imath KII(z_2+z'_2)}\right.\nn
% &&\left. +t_{\DWa\,B}(KII)\,r^*_{\DWa\,B}(KII)\,e^{-\imath KII(z_2+z'_2)}+|t_{\DWa\,B}(KII)|^2\,e^{-\imath KII(z_2-z'_2)}\right]
% \tea 
% la hipótesis básica es que la integral está dominada por los términos que no oscilan, que sólo pueden provenir de

% \bea
% && I_{AB\,HH,\UPa\,\UPa} = 2K_I\left(\frac{\omega}{c}\right)^8\,\frac{1}{2PI}\,|f_{\DWa\,B}(KII)|^2\, \int_{q\leq Q}\,\frac{d^2q}{(2\pi)^2}\,|C_H(q)|^2\,|f_{\DWa\,H}(QII)|^2\, \exp{\left[-l^2_r(\mbp-\mbq)^2-l^2_r(\mbq-\mbki)^2\right]}\nn 
% &&\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)^*(z'_1)\nn
% && \int^{z_1}_{-h}\,dz_2\,\int^{z'_1}_{-h}\,dz'_2\,\rho(z_2-z'_2) \nn 
% &&\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,e^{\imath \left(QII- KII\right)(z_2-z'_2)}+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\,e^{-\imath \left(QII- KII\right)(z_2-z'_2)}\right]
% \tea 
% Conviene separar el dominio de integración en dos triángulos

% \be
% I_{AB\,HH,\UPa\,\UPa} = 2K_I\left(\frac{\omega}{c}\right)^8\,\frac{1}{2PI}\,|f_{\DWa\,B}(KII)|^2\, \int_{q\leq Q}\,\frac{d^2q}{(2\pi)^2}\,|C_H(q)|^2\,|f_{\DWa\,H}(QII)|^2\, \exp{\left[-l^2_r(\mbp-\mbq)^2-l^2_r(\mbq-\mbki)^2\right]}\left[I_{sup}+I_{inf}\right]
% \te

% \bea
% &&I_{sup}=\int^0_{-h}\,dz_1\,\int^{z_1}_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)^*(z'_1)\nn
% && \int^{z_1}_{-h}\,dz_2\,\int^{z'_1}_{-h}\,dz'_2\,\rho(z_2-z'_2) \nn 
% &&\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,e^{\imath \left(QII- KII\right)(z_2-z'_2)}+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\,e^{-\imath \left(QII- KII\right)(z_2-z'_2)}\right]
% \tea 

% \bea
% &&I_{inf}=I_{sup}^*=\int^0_{-h}\,dz'_1\,\int^{z'_1}_{-h}\,dz_1\,\rho(z_1-z'_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)^*(z'_1)\nn
% && \int^{z_1}_{-h}\,dz_2\,\int^{z'_1}_{-h}\,dz'_2\,\rho(z_2-z'_2) \nn 
% &&\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,e^{\imath \left(QII- KII\right)(z_2-z'_2)}+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\,e^{-\imath \left(QII- KII\right)(z_2-z'_2)}\right]
% \tea 
% vamos a trabajar con $I_{sup}$. Descartamos la zona del integrando donde $z'_2<z'_1<z_2<z_1$ ya que allí el integrando es siempre oscilatorio. Por lo tanto

% \bea
% &&I_{sup}=\int^0_{-h}\,dz_1\,\int^{z_1}_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)^*(z'_1)\nn
% && \int^{z'_1}_{-h}\,dz_2\,\int^{z'_1}_{-h}\,dz'_2\,\rho(z_2-z'_2) \nn 
% &&\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,e^{\imath \left(QII- KII\right)(z_2-z'_2)}+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\,e^{-\imath \left(QII- KII\right)(z_2-z'_2)}\right]
% \tea 
% Ahora definimos

% \bea
% u_2&=&z_2-z'_2\nn
% v_2&=&\frac12\left(z_2+z'_2\right)
% \tea
% Es obvio que $dz_2dz'_2=du_2dv_2$ y que el integrando no depende de $v_2$. Tenemos que $-\left(h+z'_1\right)\le u_2\le z'_1+h$. Para un dado valor de $u_2$, 

% \be
% -h\le z'_2=v_2-\frac12u_2\le z'_1
% \te 
% y por lo tanto $u_2/2-h\le v_2\le u_2/2+z'_1$, pero también

% \be
% -h\le z_2=v_2+\frac12u_2\le z'_1
% \te 
% y entonces $-u_2/2-h\le v_2\le -u_2/2+z'_1$. Concluímos que 

% \be
% \frac12\left|u_2\right|-h\le v_2\le z'_1-\frac12\left|u_2\right|
% \te
% y entonces 
% \bea
% &&I_{sup}=\int^0_{-h}\,dz_1\,\int^{z_1}_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)^*(z'_1)\nn
% && \int^{h+z'_1}_{-h-z'_1}\,du_2\,\rho(u_2) \left(h+z'_1-\left|u_2\right|\right)\nn 
% &&\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,e^{\imath \left(QII- KII\right)u_2}+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\,e^{-\imath \left(QII- KII\right)u_2}\right]
% \tea 
% Asumiendo que $\rho\left(u_2\right)$ es par

% \bea
% &&I_{sup}=2\int^0_{-h}\,dz_1\,\int^{z_1}_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)^*(z'_1)\nn
% &&\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\right]\int^{h+z'_1}_{0}\,du_2\,\rho(u_2) \left(h+z'_1-u_2\right)\cos\left[{\left(QII- KII\right)u_2}\right]\nn
% \tea 
% Supongamos para fijar ideas que

% \be
% \rho(u_2) =\frac{L_2}{\sqrt{2\pi}\ell}e^{-u_2^2/2\ell^2}
% \te
% que converge a $L_2\delta\left(u_2\right)$ cuando $\ell\to 0$. Es coherente con lo que venimos haciendo aproximar

% \bea
% \int^{h+z'_1}_{0}\,du_2\,\rho(u_2) \left(h+z'_1-u_2\right)\cos\left[{\left(QII- KII\right)u_2}\right]&\approx&\left(h+z'_1\right)\int^{\infty}_{0}\,du_2\,\rho(u_2) \cos\left[{\left(QII- KII\right)u_2}\right]\nn
% &=&\frac12L_2\left(h+z'_1\right)e^{-\left(QII- KII\right)^2\ell^2/2}
% \tea
% hasta ahora tenemos que

% \bea 
% I_{sup}&=&L_2\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\right]e^{-\left(QII- KII\right)^2\ell^2/2}\nn
% &&\int^0_{-h}\,dz_1\,\int^{z_1}_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)^*(z'_1)\left(h+z'_1\right)
% \tea
% y ahora volvemos a usar que

% \be
% F^M_{p\,Q} = f_{Mp}(Q)\,\left[r_{Mp}(Q)\,e^{\imath Q z}+t_{Mp}(Q)\,e^{-\imath Q z}\right]
% \te


% \bea 
% I_{sup}&=&L_2\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\right]e^{-\left(QII- KII\right)^2\ell^2/2}\nn
% &&\left|f_{DA}(PII)\right|^2\left|f_{\UPa H}(QII)\right|^2\int^0_{-h}\,dz_1\,\int^{z_1}_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\left(h+z'_1\right)\nn
% &&\left[r_{DA}(PII)\,e^{\imath PII z_1}+t_{DA}(PII)\,e^{-\imath PII z_1}\right]\left[r_{\UPa H}(QII)\,e^{\imath QII z_1}+t_{\UPa H}(QII)\,e^{-\imath QII z_1}\right]\nn
% &&\left[r^*_{DA}(PII)\,e^{-\imath PII z'_1}+t^*_{DA}(PII)\,e^{\imath PII z'_1}\right]\left[r^*_{\UPa H}(QII)\,e^{-\imath QII z'_1}+t^*_{\UPa H}(QII)\,e^{\imath QII z'_1}\right]
% \tea
% Como antes, nos quedamos con los términos que exhiben puntos de fase estacionaria tanto en las integrales en $z$ como en $Q$

% \bea 
% I_{sup}&=&L_2\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\right]e^{-\left(QII- KII\right)^2\ell^2/2}\nn
% &&\left|f_{DA}(PII)\right|^2\left|f_{\UPa H}(QII)\right|^2\int^0_{-h}\,dz_1\,\int^{z_1}_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\left(h+z'_1\right)\nn
% &&\left[r_{DA}(PII)t_{\UPa H}(QII)\,e^{\imath \left(PII-QII\right) z_1}+t_{DA}(PII)r_{\UPa H}(QII)\,e^{-\imath \left(PII-QII\right) z_1}\right]\nn
% &&\left[r^*_{DA}(PII)t^*_{\UPa H}(QII)\,e^{-\imath \left(PII-QII\right) z'_1}+t^*_{DA}(PII)r^*_{\UPa H}(QII)\,e^{\imath \left(PII-QII\right) z'_1}\right]
% \tea

% \bea 
% &&I_{sup}=L_2\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\right]e^{-\left(QII- KII\right)^2\ell^2/2}\nn
% &&\left|f_{DA}(PII)\right|^2\left|f_{\UPa H}(QII)\right|^2\int^0_{-h}\,dz_1\,\int^{z_1}_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\left(h+z'_1\right)\nn
% &&\left[\left|r_{DA}(PII)\right|^2\left|t_{\UPa H}(QII)\right|^2\,e^{\imath \left(PII-QII\right) \left(z_1-z'_1\right)}+\left|t_{DA}(PII)\right|^2\left|r_{\UPa H}(QII)\right|^2\,e^{-\imath \left(PII-QII\right) \left(z_1-z'_1\right)}\right]
% \tea
% Como antes, cambiamos variables a

% \bea
% u_1&=&z_1-z'_1\nn
% v_1&=&\frac12\left(z_1+z'_1\right)
% \tea
% Entonces $0\le u_1\le h$

% \bea
% &&-h\le v_1+\frac12u_1\le 0\nn
% &&-h\le v_1-\frac12u_1\le v_1+\frac12u_1
% \tea
% o sea que $u_1/2-h\le v_1\le -u_1/2$

% \bea 
% &&I_{sup}=L_2\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\right]e^{-\left(QII- KII\right)^2\ell^2/2}\nn
% &&\left|f_{DA}(PII)\right|^2\left|f_{\UPa H}(QII)\right|^2\int^h_{0}\,du_1\,\rho(u_1)\nn
% &&\left[\left|r_{DA}(PII)\right|^2\left|t_{\UPa H}(QII)\right|^2\,e^{\imath \left(PII-QII\right) \left(u_1\right)}+\left|t_{DA}(PII)\right|^2\left|r_{\UPa H}(QII)\right|^2\,e^{-\imath \left(PII-QII\right) \left(u_1\right)}\right]\nn
% &&\int_{u_1/2-h}^{-u_1/2}dv_1\,\left(h+v_1-\frac12u_1\right)
% \tea
% Como antes, asumimos que la integral está dominada por el entorno de $u_1=0$

% \bea 
% &&I_{sup}=\frac12h^2L_2\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\right]e^{-\left(QII- KII\right)^2\ell^2/2}\nn
% &&\left|f_{DA}(PII)\right|^2\left|f_{\UPa H}(QII)\right|^2\left[\left|r_{DA}(PII)\right|^2\left|t_{\UPa H}(QII)\right|^2\,J+\left|t_{DA}(PII)\right|^2\left|r_{\UPa H}(QII)\right|^2\,J^*\right]\nn
% \tea
% donde 

% \bea 
% J&=&\int^{\infty}_{0}\,du_1\,\rho(u_1)\;e^{\imath \left(PII-QII\right) \left(u_1\right)}\nn
% &=&\frac12L_2e^{-\ell^2\left(PII-QII\right)^2/2}
% \tea
% El resultado final es 

% \bea 
% &&I_{sup}=I_{inf}=\frac14h^2L^2_2\left|f_{DA}(PII)\right|^2\left|f_{\UPa H}(QII)\right|^2\left[\left|r_{DA}(PII)\right|^2\left|t_{\UPa H}(QII)\right|^2+\left|t_{DA}(PII)\right|^2\left|r_{\UPa H}(QII)\right|^2\right]\nn
% &&\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\right]e^{-\left[\left(QII- KII\right)^2+\left(PII-QII\right)^2\right]\ell^2/2}
% \tea
% Todavía falta evaluar la integral en $Q$.



% % Los dos últimos renglones son una manera bruta de escribir que cuando $QII\neq KII$ vale el término oscilatorio en $z_1$ y cuando $QII = KII$ vale el término lineal en $z_1$.

% % Ahora hay que integrar en $z_1 \,z'_1$. Habíamos dicho de tomar el límite $h\rightarrow -\infty$ para llegar a transformadas de Fourier de $\rho(z_1-z'_1)$. Pero el término $\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)^*(z'_1)$ jode bastante a tales fines. Primero habría que hacer un cambio de variables pero no se logra desacoplar el producto de funciones, siempre queda una integral por hacer. Que no quiero hacer.

% % Mi propuesta es volver a tomar $\rho(z_1-z'_1)\sim \delta(z_1-z'_1)$, llegar así a una integral en tres dimensiones, $d^2q\,dz$ y ahí mandarlo derecho viejo a la compu. ¿Purgatorio?


% \begin{figure}
%     \centering
%     \includegraphics[scale=1.5]{figures/purgatorio.jpg}
%     \caption{Asombrados, Dante y Virgilio observan como algunos de los sufrientes en el Aqueronte han logrado (¿cómo? nadie sabe) alcanzar las llanuras ascendentes del purgatorio. Sálvenos, oh bienaventurados, claman desde las aguas no tan hostiles. Los poetas, sin embargo, continuan su imperturbable ascenso.}
%     \label{fig:my_label}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55
% Si hacemos el producto entre los dos corchetes salen 16 términos, con todas las combinaciones posibles de $\pm QII \pm KII$.

% Hasta acá, puro amasado. Ahora viene lo feo. Primero, para hacer las integrales en $dz_2\,dz'_2$ creo que es conveniente hacer un cambio de variables tipo $r=z_2-z'_2\,;\,s=z_2$. Después viene la integral en sí. De forma cerrada no sale, por el factor $\rho(z_2-z'_2)$. En el caso en que $R = \pm QII \pm KII \neq 0$ me convencí de que la integral la podemos aproximar como $\rho(x)/(\imath R)\,e^{\imath R x}$ evaluando en los extremos que corresponda a $x$. Cuando $R = \pm QII \pm KII = 0$ desarrollo $\rho(x)$ a segundo orden e integro a mano. Entonces reducimos en dos dimensiones la integral. Pero ahora hay $16\times 2$ términos luego del primer par de integrales, que dependen de $z_1$ y $z'_1$. Y todavía falta expandir el producto de las $F$ evaluadas en $z_1$ y $z'_1$, volver a acomodar el ingtegrando y volver a integrar usando las mismas aproximaciones. Si no me equivoco, habrá del orden de 64 términos para, finalmente, integrar de manera numérica en $d^2q$. 

% \bigskip
% \bigskip

% \textit{Conclusiones de verano:} 

% \begin{itemize}
%     \item Si no me equivoqué, para cada canal $AB$ hay entonces $2\times12\times64 = 1536$ términos a integrar de manera numérica.
%     \item Honestamente, no creo poder hacer esto sin equvicarme ni en el desarrollo algebraico ni en la implementación numérica.
%     \item Honestamente, no creo tener ganas de hacer todo esto de esta manera.
% \end{itemize}

% \bigskip

% Todo esto me recuerda a aquel que se atrevió a cruzar el Aqueronte y, ya siendo tarde para arrepentirse, dijo:

% \medskip

% Y después de haber puesto su mano en la mia con rostro alegre, que me reanimó, me introdujo en medio de las cosas secretas. Alli, bajo un cielo sin estrellas, resonaban suspiros, quejas y profundos gemidos, de suerte que al escucharlos comencé a llorar. Diversas lenguas, horribles blasfemias, palabras de dolor, acentos de ira, voces altas y roncas, acompañadas de palmadas, producian un tumulto que va rodando siempre por aquel espacio eternamente oscuro, como la arena impelida por un torbellino. Yo, que estaba horrorizado, dije:

% - Maestro, ¿qué es lo que oigo, y qué gente es ésa, que parece doblegada por el dolor?

% Me respondió:

% - Esta miserable suerte está reservada a las tristes almas de aquellos que vivieron sin merecer alabanzas ni vituperio; están confundidas entre el perverso coro de los ángeles que no fueron rebeldes ni fieles a Dios, sino que sólo vivieron para si. El Cielo los lanzó de su seno por no ser menos hermoso, pero el profundo Infierno no quiere recibirlos por la gloria que con ello podrían reportar los demás culpables.

% Y yo repuse:

% - Maestro, ¿qué cruel dolor les hace lamentarse tanto?

% A lo que me contestó:

% - Te lo diré brevemente. Éstos no esperan morir; y su ceguedad es tanta, que se muestran envidiosos de cualquier otra suerte. El mundo no conserva ningún recuerdo suyo; la misericordia y la justicia los desdeñan: no hablemos más de ellos, míralos y pasa adelante.


% \begin{figure}
%     \centering
%     \includegraphics[width = \textwidth]{figures/aqueronte.jpg}
%     \caption{Aquellos que quisieron integrar en seis dimensiones 1536 términos oscilatorios. Dante y Virgilio los observan sin sentir pena ni misericordia. Culpa de ellos por atreverse a tanto.}
% \end{figure}






















% A note for Oscar:

% \bea
% && \langle |S^{(2)}_{rs}(z)|^2 \rangle \propto
%  \int\,\frac{d^2q}{(2\pi)^2}\,\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz_2\,\int^0_{-h}\,dz'_1\,\int^0_{-h}\,dz'_2\,\sum_{\mu,m}\,\,\sum_{\mu',m'}\,\,\mathcal{C}^{\mu,m;\mu',m'}_{L,\mbp\,\mbq}(z1-z'_1,z_2-z'_2) \nn
% && \propto \int_{q^2\leq \epsilon_1 k^2_i}\,\frac{d^2q}{(2\pi)^2}\,\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz_2\,\int^0_{-h}\,dz'_1\,\int^0_{-h}\,dz'_2\nn
% && \exp{\left(-(\mbp-\mbq)^2(z_1-z'_1)^2\right)}\,\exp{\left(-(\mbq-\mbki)^2(z_2-z'_2)^2\right)}\,\frac{1}{QII}\left[\left(\hat{p}\cdot\hat{q}\right)\,\left(\hat{q}\cdot\hat{k}_i\right)\right]^2\nn
% &&\left[R(PII)\,e^{\imath PII z_1}+ T(PII)\,e^{-\imath PII z_1} \right] \,\,\left[R(QII)\,e^{\imath QII z_1}+T(QII)\,e^{-\imath QII z_1} \right]
% \nn
% && \left[r(QII)\,e^{\imath QII z_2}+t(QII)\,e^{-\imath QII z_2} \right]\,
% \left[R(KII)\,e^{\imath KII z_2}+ T(KII)\,e^{-\imath KII z_2} \right]\,\Theta(z_1-z_2) \nn
% &&\left[R(PII)\,e^{\imath PII z'_1}+ T(PII)\,e^{-\imath PII z'_1} \right]^* \,\left[R(QII)\,e^{\imath QII z'_1}+T(QII)\,e^{-\imath QII z'_1} \right]^*
% \nn 
% && \left[r(QII)\,e^{\imath QII z'_2}+t(QII)\,e^{-\imath QII z'_2} \right]^*\,
% \left[R(KII)\,e^{\imath KII z'_2}+ T(KII)\,e^{-\imath KII z'_2} \right]^*\,\Theta(z'_1-z'_2)
% \tea 


% $k_i = \frac{2\pi}{\lambda}$: numero de onda incidente;\\

% $KII = k_i\sqrt{1-\sin^2\theta_i}$: modo vertical en la dirección incidente dentro del medio dielectrico con fluctuaciones;\\

% $PII = k_i\,\sqrt{\epsilon_1 - \sin^2\theta_s}$, modo vertical en la dirección dispersada dentro del medio dielectrico con fluctuaciones;\\

% $QII = k_i\,\sqrt{\epsilon_1 - \sin^2\theta_q}$: modo auxiliar (a ser integrado). se puede integrar en cartesianas sobre $q^2_x + q^2_y \leq \epsilon_1\,k^2_i$ o bien en polares sobre $[q,\phi_q]:[0,\sqrt{\epsilon_1}k_i]\times[0,2\pi]$. El ángulo $\theta_q$ se calcula a partir del modulo  $q$ y el ángulo $\phi_q$.\\

% Los coeficientes $R,T$ o $r,t$ dependen de los modos verticale en donde estan evaluados. El factor dependiendo de $Q$ queda puesto de forma explicita delante de las exponenciales.



==> Sections/not_used/version_compacta.tex <==
\section{Cálculo orden a orden de los campos dispersados}

% \def\vpp{\varphi_\mathbf{p}}
% \def\vpq{\varphi_\mathbf{q}}
% \def\psip{\psi_\mathbf{p}}
% \def\psiq{\psi_\mathbf{q}}

\subsection{Incidencia en modo TE (pol H)}


\subsubsection{Orden Cero}

\bea 
&& \vpp^{(0)}(z) = (2\pi)^2\,\delta(\mbp-\mbk)\,\sqrt{2KI}\,F^{D}_{H\,K}(z) \nn
&& \psip^{(0)} = 0\nn 
&& E^{(0)}_{z\,\mbp} = 0 \nonumber
\tea 

\subsubsection{Orden Uno}

Corrientes para $\vpp$ y $\psip$, respectivamente:

\bea
&& J^{(1)}_{HH\,,\mbp} (z) = \left(\frac{\omega}{c}\right)^2\,\sqrt{2KI}\,\EPpk(z)\,\left(\hat{p}\cdot\hat{k}\right)\,F^D_{H\,K}(z) \nn
&& J^{(1)}_{VH\,,\mbp} (z) = - \left(\frac{\omega}{c}\right)^2\,\sqrt{2KI}\,\EPpk(z)\,\hat{z}\cdot\left(\hat{p}\times\hat{k}\right)\,F^D_{H\,K}(z)
\tea 

\textbf{Campos dispersados:}

\textsc{En el medio I:}

\bea 
&& \vpp^{(1)}(z) = \sqrt{2KI}\left(\frac{\omega}{c}\right)^2\,\left(\hat{p}\cdot\hat{k}\right) F^U_{H\,PI}(z)\,\int^0_{-H}\,dz'\,\EPpk(z')\,F^D_{H\,PII}(z')\,F^D_{H\,KII}(z') \nn
&& \psip^{(1)}(z) = - \sqrt{2KI}\left(\frac{\omega}{c}\right)^2\,\hat{z}\cdot\left(\hat{p}\times\hat{k}\right) F^U_{V\,PI}(z)\,\int^0_{-H}\,dz'\,\EPpk(z')\,F^D_{V\,PII}(z')\,F^D_{H\,KII}(z')
\tea

\textsc{En el medio II:}

\bea 
&& \vpp^{(1)}(z) = \sqrt{2KI}\left(\frac{\omega}{c}\right)^2\,\left(\hat{p}\cdot\hat{k}\right)\, \sum_\mu\, F^\mu_{H\,PII}(z)\,\int^0_{-H}\,dz'\,\EPpk(z')\,F^{\bar{\mu}}_{H\,PII}(z')\,F^D_{H\,KII}(z')\,\Theta_\mu(z,z') \nn
&& \psip^{(1)}(z) = - \sqrt{2KI}\left(\frac{\omega}{c}\right)^2\,\hat{z}\cdot\left(\hat{p}\times\hat{k}\right) \,\sum_\mu\,F^\mu_{V\,PII}(z)\,\int^0_{-H}\,dz'\,\EPpk(z')\,F^{\bar{\mu}}_{V\,PII}(z')\,F^D_{H\,KII}(z')\,\Theta_\mu(z,z')
\tea


donde $\mu = \left\lbrace \text{UP}, \text{DOWN}\right\rbrace \,\,\rightarrow\,\,\bar{\mu} = \left\lbrace \text{DOWN},\text{UP} \right\rbrace$ son las dos posibles propagaciones en le medio II: $\Theta_{\text{UP}} = \Theta(z>z')$ y  $\Theta_{\text{DOWN}} = \Theta(z<z')$.


\subsubsection{Orden Dos:}

Corriente para $\vpp^{(2)}$:

\bea
J^{(2)}_{HH\,\mbp}(z) = -\sqrt{2KI}\left(\frac{\omega}{c}\right)^4 && \int  \frac{d^2q}{(2\pi)^2}\,\,\EPpq(z)\nn && \left[\left(\hat{p}\cdot\hat{q}\right)\,\left(\hat{q}\cdot\hat{k}\right)\,\sum_\mu\,F^\mu_{H\,QII}(z)\int dz'\EPqki(z')\,F^{\bar{\mu}}_{H\,QII}(z')\,F^D_{H\,KII}(z')\,\Theta_\mu(z,z') \right. \nn 
&& \left. +\hat{z}\cdot\left(\hat{p}\times\hat{q}\right)\,\hat{z}\cdot\left(\hat{q}\times\hat{k}\right)\,\sum_\mu\,F^\mu_{V\,QII}(z)\int dz'\EPqki(z')\,F^{\bar{\mu}}_{V\,QII}(z')\,F^D_{H\,KII}(z')\,\Theta_\mu(z,z')\right] \nonumber
\tea

\textsc{Campo dispersado en el medio I:}

\bea
&& \vpp^{(2)}(z) = -\sqrt{2KI}\left(\frac{\omega}{c}\right)^4\,F^U_{H\,PI}(z)  \int  \frac{d^2q}{(2\pi)^2}\,\int dz_1\,\int dz_2 \,\EPpq(z_1)\,\EPqki(z_2)\nn  && F^D_{H\,PII}(z_1)\sum_\mu\,\Theta_\mu(z_1,z_2)\,\left[\left(\hat{p}\cdot\hat{q}\right)\,\left(\hat{q}\cdot\hat{k}\right)\,F^\mu_{H\,QII}(z_1)\,F^{\bar{\mu}}_{H\,QII}(z_2)\right. \nn 
&& \left. +\hat{z}\cdot\left(\hat{p}\times\hat{q}\right)\,\hat{z}\cdot\left(\hat{q}\times\hat{k}\right)\,F^\mu_{V\,QII}(z_1))\,F^{\bar{\mu}}_{V\,QII}(z_2)\right]\,F^D_{H\,KII}(z_2) \nonumber
\tea

Mas compactamente:

\bea
&& \vpp^{(2)}(z) = -\sqrt{2KI}\left(\frac{\omega}{c}\right)^4\,F^U_{H\,PI}(z)  \int  \frac{d^2q}{(2\pi)^2}\,\int dz_1\,\int dz_2 \,\EPpq(z_1)\,\EPqki(z_2)\nn  && F^D_{H\,PII}(z_1)\sum_{\mu,m}\,\Theta_\mu(z_1,z_2)\,\left[\beta_m\,F^\mu_{m\,QII}(z_1)\,F^{\bar{\mu}}_{m\,QII}(z_2)\right]\,F^D_{H\,KII}(z_2) \nonumber
\tea

donde $m = \left\lbrace H, V \right\rbrace$, $\beta_H = \left(\hat{p}\cdot\hat{q}\right)\,\left(\hat{q}\cdot\hat{k}\right)$ y $\beta_V = \hat{z}\cdot\left(\hat{p}\times\hat{q}\right)\,\hat{z}\cdot\left(\hat{q}\times\hat{k}\right)$.


Corriente para $\psip^{(2)}:$


\bea
J^{(2)}_{VH\,\mbp}(z) = -\sqrt{2KI}\left(\frac{\omega}{c}\right)^4 && \int  \frac{d^2q}{(2\pi)^2}\,\,\EPpq(z)\nn && \left[\hat{z}\cdot\left(\hat{p}\times\hat{q}\right)\,\left(\hat{q}\cdot\hat{k}\right)\,\sum_\mu\,F^\mu_{H\,QII}(z)\int dz'\EPqki(z')\,F^{\bar{\mu}}_{H\,QII}(z')\,F^D_{H\,KII}(z')\,\Theta_\mu(z,z') \right. \nn 
&& \left. +\left(\hat{p}\cdot\hat{q}\right)\,\hat{z}\cdot\left(\hat{q}\times\hat{k}\right)\,\sum_\mu\,F^\mu_{V\,QII}(z)\int dz'\EPqki(z')\,F^{\bar{\mu}}_{V\,QII}(z')\,F^D_{H\,KII}(z')\,\Theta_\mu(z,z')\right]  \nonumber
\tea
\bea
&& +\sqrt{2KI}\left(\frac{\omega}{c}\right)^4\,\frac{\partial}{\partial z} \frac{\imath p}{P^2}\int \frac{d^2q}{(2\pi)^2}\,\EPpq(z)\,\frac{\imath q}{Q^2}  \hat{z}\cdot\left(\hat{q}\times\hat{k}\right)\,\frac{\partial}{\partial z}\sum_\mu\,F^\mu_{V\,QII}(z)\,\int dz' \EPqki(z')\,F^{\bar{\mu}}_{V\,QII}(z')\,F^D_{H\,KII}(z')\,\Theta_\mu(z,z') \nonumber
\tea

\textsc{Campo dispersado en el medio I:}

\bea
&& \psip^{(2)}(z) = -\sqrt{2KI}\left(\frac{\omega}{c}\right)^4\,F^U_{V\,PI}(z)  \int  \frac{d^2q}{(2\pi)^2}\,\int dz_1\,\int dz_2 \,\EPpq(z_1)\,\EPqki(z_2)\nn  && F^D_{V\,PII}(z_1)\sum_\mu\,\Theta_\mu(z_1,z_2)\,\left[\hat{z}\cdot\left(\hat{p}\times\hat{q}\right)\,\left(\hat{q}\cdot\hat{k}\right)\,F^\mu_{H\,QII}(z_1)\,F^{\bar{\mu}}_{H\,QII}(z_2)\right. \nn 
&& \left. -\left(\hat{p}\cdot\hat{q}\right)\,\hat{z}\cdot\left(\hat{q}\times\hat{k}\right)\,F^\mu_{V\,QII}(z_1))\,F^{\bar{\mu}}_{V\,QII}(z_2)\right]\,F^D_{H\,KII}(z_2) \nn
&& -\sqrt{2KI}\left(\frac{\omega}{c}\right)^4\,F^U_{V\,PI}(z)\int dz_1 F^D_{V\,PII}(z_1)\,\frac{\partial}{\partial z_1} \frac{\imath p}{P^2}\int \frac{d^2q}{(2\pi)^2}\,\EPpq(z_1)\,\frac{\imath q}{Q^2}  \hat{z}\cdot\left(\hat{q}\times\hat{k}\right)\nn 
&& \frac{\partial}{\partial z_1}\sum_\mu\,F^\mu_{V\,QII}(z_1)\,\int dz_2\, \EPqki(z_2)\,F^{\bar{\mu}}_{V\,QII}(z_2)\,F^D_{H\,KII}(z_2)\,\Theta_\mu(z_1,z_2) \nonumber
\tea

En el último término hay dos derivadas respecto a $z_1$: la segunda, más interna en el integral, solo afecta a $F^\mu_{V\,QII}(z_1)$; entonces $\partial_{z1}F^\mu_{V\,QII}(z_1) = \imath QII \tilde{F}^\mu_{V\,QII}(z_1)$. La primera derivada la elimimo integrando por partes y tirando el término de borde. Entonces llegamos a:



\bea
&& \psip^{(2)}(z) = -\sqrt{2KI}\left(\frac{\omega}{c}\right)^4\,F^U_{V\,PI}(z)  \int  \frac{d^2q}{(2\pi)^2}\,\int dz_1\,\int dz_2 \,\EPpq(z_1)\,\EPqki(z_2)\nn  
&& \sum_{\mu}\,\Theta_\mu(z_1,z_2)\,\left\lbrace F^D_{V\,PII}(z_1)\,\sum_m\,\gamma_m\,F^\mu_{m\,QII}(z_1)\,F^{\bar{\mu}}_{m\,QII}(z_2) + \right. \nn
&& \left. + \tilde{\gamma}\tilde{F}^D_{V\,PII}(z_1)\,\tilde{F}^{\mu}_{V\,QII}(z_1)
\,F^{\bar{\mu}}_{V\,QII}(z_2)\right\rbrace F^D_{H\,KII}(z_2) \nonumber
\tea



donde $\gamma_H = \hat{z}\cdot\left(\hat{p}\times\hat{q}\right)\,\left(\hat{q}\cdot\hat{k}\right)$, $\gamma_V = -\left(\hat{p}\cdot\hat{q}\right)\,\hat{z}\cdot\left(\hat{q}\times\hat{k}\right)$,
$\tilde{\gamma} = \frac{p\,q}{PII\,QII}\,\hat{z}\cdot\left(\hat{q}\times\hat{k}\right)$


\subsection{Incidencia en modo TM (pol V)}

\subsubsection{Orden Cero}

\bea
&& \vpp^{(0)} = 0 \nn
&& \psip^{(0)}(z) = (2\pi)^2\,\delta(\mbp-\mbk)\,\sqrt{2KI}\,F^{D}_{V\,K}(z) \nn
&& E^{(0)}_{z\,\mbp}(z) = \frac{\imath p}{P^2}\frac{\partial}{\partial z}\psip^{(0)}(z) = -(2\pi)^2\,\delta(\mbp-\mbk)\,\sqrt{2KI}\,\frac{p K}{P^2}\,\tilde{F}^{D}_{V\,K}(z) \nonumber
\tea


\subsubsection{Orden Uno}

Corriente para $\vpp^{(1)}$:

\be 
J^{(1)}_{HV\,\mbp}(z) = \sqrt{2KI}\,\left(\frac{\omega}{c}\right)^2\,\hat{z}\cdot\left(\hat{p}\times\hat{k}\right)\,\EPpk(z)\,F^D_{V\,KII}(z) \nonumber
\te 


Corriente para $\psip^{(1)}$:

\be 
J^{(1)}_{VV\,\mbp}(z) = \sqrt{2KI}\,\left(\frac{\omega}{c}\right)^2\,\left(\hat{p}\cdot\hat{k}\right)\,\EPpk(z)\,F^D_{V\,KII}(z)  + \sqrt{2KI}\,\left(\frac{\omega}{c}\right)^2 \frac{\partial}{\partial z}\frac{\imath p}{P^2} \frac{k}{KII}\,\EPpk(z)\,\tilde{F}^D_{V\,KII}(z) \nonumber
\te


\textsc{Campos dispersados en el medio I:}

\be 
\vpp^{(1)}(z) = -\sqrt{2KI}\,\left(\frac{\omega}{c}\right)^2\,\hat{z}\cdot\left(\hat{p}\times\hat{k}\right)\,F^U_{H\,PI}(z)\int dz'\,\EPpk(z')\,F^D_{H\,PII}(z')\,F^D_{V\,KII}(z') \nonumber
\te 


\bea
&& \psip^{(1)}(z) = -\sqrt{2KI}\,\left(\frac{\omega}{c}\right)^2\,\left(\hat{p}\cdot\hat{k}\right)\,F^U_{V\,PI}(z)\int dz'\,\EPpk(z')\,F^D_{V\,PII}(z')\,F^D_{V\,KII}(z') \nn
&& -\sqrt{2KI}\,\left(\frac{\omega}{c}\right)^2\,F^U_{V\,PI}(z)\int dz'\,F^D_{V\,PII}(z')\frac{\partial}{\partial z'}\frac{\imath p\,k}{P^2\,KII}\EPpk(z')\,\,\tilde{F}^D_{V\,KII}(z')
\tea 

Integro por partes, ignoro el término de borde y llego a:

\bea
&& \psip^{(1)}(z) = -\sqrt{2KI}\,\left(\frac{\omega}{c}\right)^2\,F^U_{V\,PI}(z)\int dz'\,\EPpk(z')\nn 
&& \left[\left(\hat{p}\cdot\hat{k}\right)\,F^D_{V\,PII}(z')\,F^D_{V\,KII}(z')  -\frac{p\,k}{PII\,KII}\tilde{F}^D_{V\,PII}(z')\,\tilde{F}^D_{V\,KII}(z')\right]
\tea 


\textsc{Campos dispersados en el medio II:}

\be 
\vpp^{(1)}(z) = -\sqrt{2KI}\,\left(\frac{\omega}{c}\right)^2\,\hat{z}\cdot\left(\hat{p}\times\hat{k}\right)\,\sum_\mu\,F^\mu_{H\,PII}(z)\int dz'\,\EPpk(z')\,F^{\bar{\mu}}_{H\,PII}(z')\,F^D_{V\,KII}(z') \Theta_\mu(z,z') \nonumber
\te 


\bea
&& \psip^{(1)}(z) = -\sqrt{2KI}\,\left(\frac{\omega}{c}\right)^2\,\sum_\mu\,F^\mu_{V\,PII}(z)\int dz'\,\EPpk(z')\nn 
&& \left[\left(\hat{p}\cdot\hat{k}\right)\,F^{\bar{\mu}}_{V\,PII}(z')\,F^D_{V\,KII}(z') -\frac{p\,k}{PII\,KII}\tilde{F}^{\bar{\mu}}_{V\,PII}(z')\,\tilde{F}^D_{V\,KII}(z')\right]
\tea 


\subsubsection{Orden Dos}


Corriente para $\vpp^{(2)}$:


\bea
&& J^{(2)}_{HV\,\mbp}(z) = - \sqrt{2KI}\left(\frac{\omega}{c}\right)^4\,\int \frac{d^2q}{(2\pi)^2} \EPpq(z_1)\nn 
&& \sum_\mu \left[ \left(\hat{p}\cdot\hat{q}\right)\,\hat{z}\cdot\left(\hat{q}\times\hat{k}\right)\,F^\mu_{H\,QII}(z_1)\,\int dz_2\,\EPqki(z_2)\,F^{\bar{\mu}}_{H\,QII}(z_2)\,F^D_{V\,KII}(z_2)\,\Theta_\mu(z_1,z_2) \right. \nn
&& \left. + \hat{z}\cdot\left(\hat{p}\times\hat{q}\right)\,\left(\hat{q}\cdot\hat{k}\right)\,F^\mu_{V\,QII}(z_1)\,\int dz_2\,\EPqki(z_2)\,F^{\bar{\mu}}_{V\,QII}(z_2)\,F^D_{V\,KII}(z_2)\,\Theta_\mu(z_1,z_2)  \right. \nn
&& \left. - \hat{z}\cdot\left(\hat{p}\times\hat{q}\right)\,\frac{p\,k}{PII\,KII}\,F^\mu_{V\,QII}(z_1)\,\int dz_2\,\EPqki(z_2)\,\tilde{F}^{\bar{\mu}}_{V\,QII}(z_2)\,\tilde{F}^D_{V\,KII}(z_2)\,\Theta_\mu(z_1,z_2) \right] 
\tea 

\textsc{Lo que nos lleva al campo dispersado en el medio I:}

\bea
&& \vpp^{(2)}(z) = - \sqrt{2KI}\left(\frac{\omega}{c}\right)^4\,F^U_{H\,PI}(z)\,\int \frac{d^2q}{(2\pi)^2}\,\int dz_1\,\int dz_2\, \EPpq(z_1)\,\EPqki(z_2)\nn 
&&F^D_{H\,PII}(z_1) \sum_\mu \Theta_\mu(z_1,z_2) \left[\sum_m \eta_m \,F^\mu_{m\,QII}(z_1)\,F^{\bar{\mu}}_{m\,QII}(z_2)\,F^D_{V\,KII}(z_2)
+\tilde{\eta}\,F^\mu_{V\,QII}(z_1)\,\tilde{F}^{\bar{\mu}}_{V\,QII}(z_2)\,\tilde{F}^D_{V\,KII}(z_2) \right] 
\tea 

$\eta_H = \left(\hat{p}\cdot\hat{q}\right)\,\hat{z}\cdot\left(\hat{q}\times\hat{k}\right)$, $\eta_V = \hat{z}\cdot\left(\hat{p}\times\hat{q}\right)\,\left(\hat{q}\cdot\hat{k}\right)$ y $\tilde{\eta} = - \hat{z}\cdot\left(\hat{p}\times\hat{q}\right)\,\frac{p\,k}{PII\,KII}$.


Corriente para $\psip^{(2)}$:


\bea
&& J^{(2)}_{VV\,\mbp}(z) = -\sqrt{2KI}\left(\frac{\omega}{c}\right)^4\,\int \frac{d^2q}{(2\pi)^2}\,\EPpq(z)\nn 
&& \sum_\mu \left\lbrace \sum_m \zeta_m\,F^\mu_{m\,QII}(z)\,\int dz'\,\EPqki(z')\,F^{\bar{\mu}}_{m\,QII}(z')\,F^D_{V\,KII}(z')\,\Theta_\mu(z,z') \right. \nn
&& \left. + \tilde{\zeta}\,F^\mu_{V\,QII}(z)\,\int dz'\,\EPqki(z')\,\tilde{F}^{\bar{\mu}}_{V\,QII}(z')\,\tilde{F}^D_{V\,KII}(z')\,\Theta_\mu(z,z') \right\rbrace \nn 
&&+ \sqrt{2KI}\left(\frac{\omega}{c}\right)^4 \frac{\partial}{\partial z} \frac{\imath p}{P^2} \int \frac{d^2q}{2\pi)^2} \EPpq(z)\,\frac{\imath q}{Q^2} \frac{\partial}{\partial z} \psip^{(1)}(z) \nonumber
\tea 

$\zeta_H = -\hat{z}\cdot\left(\hat{p}\times\hat{q}\right)\,\hat{z}\cdot\left(\hat{q}\times\hat{k}\right)$, $\zeta_V = \left(\hat{p}\cdot\hat{q}\right)\,\left(\hat{q}\cdot\hat{k}\right)$ y $\tilde{\zeta} = -\left(\hat{p}\cdot\hat{q}\right)\frac{p\,k}{PII\,KII}$.


El campo dispersado en el medio I es:



\bea
&& \psip^{(2)}(z) = \sqrt{2KI}\left(\frac{\omega}{c}\right)^4\,F^U_{V\,PI}(z)\int \frac{d^2q}{(2\pi)^2}\,\int dz_1\,\int dz_2\,\EPpq(z)\,\EPqki(z_2)\nn 
&& \sum_\mu\,\Theta_\mu(z_1,z_2) F^D_{V\,PII}(z_1)\,\left[ \sum_m \zeta_m\,F^\mu_{m\,QII}(z)\,F^{\bar{\mu}}_{m\,QII}(z')\,F^D_{V\,KII}(z')\,\Theta_\mu(z,z') \right. \nn
&&  \left. + \tilde{\zeta}\,F^\mu_{V\,QII}(z)\,\tilde{F}^{\bar{\mu}}_{V\,QII}(z')\,\tilde{F}^D_{V\,KII}(z') \right] \nn
&& +\sqrt{2KI}\left(\frac{\omega}{c}\right)^4\,F^U_{V\,PI}(z)\int dz_1\,F^D_{V\,PII}(z_1)\,\frac{\partial}{\partial z_1} \frac{p}{P^2} \int \frac{d^2q}{2\pi)^2} \EPpq(z_1)\,\frac{q}{Q^2} \frac{\partial}{\partial z_1} \psiq^{(1)}(z_1) \nonumber
\tea 



En el último término procedo de igual manera con las derivadas: la más interna la aplico sobre $\psi^{(1)}_\mbq$ y con la más externa integro por partes e igonoro el término de borde. LLego a:


\bea
&& \psip^{(2)}(z) = \sqrt{2KI}\left(\frac{\omega}{c}\right)^4\,F^U_{V\,PI}(z)\int \frac{d^2q}{(2\pi)^2}\,\int dz_1\,\int dz_2\,\EPpq(z)\,\EPqki(z_2)\nn 
&& \sum_\mu\,\Theta_\mu(z_1,z_2)\left\lbrace F^D_{V\,PII}(z_1)\,\left[ \sum_m \zeta_m\,F^\mu_{m\,QII}(z)\,F^{\bar{\mu}}_{m\,QII}(z')\,F^D_{V\,KII}(z')\,\Theta_\mu(z,z') \right. \right.\nn
&& \left. \left. + \tilde{\zeta}\,F^\mu_{V\,QII}(z)\,\tilde{F}^{\bar{\mu}}_{V\,QII}(z')\,\tilde{F}^D_{V\,KII}(z') \right] \right.\nn 
&& \left. + \tilde{F}^D_{V\,PII}(z_1)\,\tilde{F}^\mu_{V\,QII}(z_1)\,\left[\zeta_4\,F^{\bar{\mu}}_{V\,QII}(z_2)\,F^D_{V\,KII}(z_2)+\zeta_5\,\tilde{F}^{\bar{\mu}}_{V\,QII}(z_2)\,\tilde{F}^D_{V\,KII}(z_2) \right] \right\rbrace
\tea 


$\zeta_4 = \left(\hat{q}\cdot\hat{k}\right)\,\frac{p\,q}{PII\,QII}$ y $\zeta_5 =- \frac{p\,q}{PII\,QII}\,\frac{q\,k}{QII\,KII}$.


\subsection{Resumen de la situación}

Nos habìamos quedado en que para el canal $AB$ (pol dispersada $A$, pol indicente $B$) teníamos:

\bea
&& \langle L_{AB} \rangle  =  2K_I\,\omega^8\,\frac{1}{2PI} \int_{q\leq Q}\,\frac{d^2q}{(2\pi)^2}\,\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz'_1\,\int\,dz_2\,\int\,dz'_2\nn 
&& \exp{\left[-l^2_r\,(\mbp-\mbq)^2\right]}\,\rho(z_1-z'_1)\,
\exp{\left[-l^2_r\,(\mbq-\mbki)^2\right]}\,\rho(z_2-z'_2)\nn
&& F^{D}_{A\,PII}(z_1)\,
\sum_\mu\,\left\lbrace (\hat{p}\cdot\hat{q})(\hat{q}\cdot\hat{k})\,F^\mu_{H\,QII}(z_1)\,F^{\bar{\mu}}_{H\,QII}(z_2) -\hat{z}\cdot(\hat{p}\times\hat{q})\,\hat{z}\cdot(\hat{q}\times\hat{k})\,F^\mu_{V\,QII}(z_1)\,F^{\bar{\mu}}_{V\,QII}(z_2) \right\rbrace\,\Theta_\mu(z_1,z_2)\,F^{D}_{B\,KII}(z_2)\nn
&& F^{D*}_{A\,PII}(z'_1)\,
\sum_{\mu'}\,\left\lbrace (\hat{p}\cdot\hat{q})(\hat{q}\cdot\hat{k})\,F^\mu_{H\,QII}(z'_1)\,F^{\bar{\mu}}_{H\,QII}(z'_2) -\hat{z}\cdot(\hat{p}\times\hat{q})\,\hat{z}\cdot(\hat{q}\times\hat{k})\,F^\mu_{V\,QII}(z'_1)\,F^{\bar{\mu}}_{V\,QII}(z'_2) \right\rbrace^*\,\Theta_{\mu'}(z'_1,z'_2)\,F^{D\,*}_{B\,KII}(z'_2) \nonumber
\tea 

Definimos los coeficientes $C_H(q) = (\hat{p}\cdot\hat{q})(\hat{q}\cdot\hat{k})$ y $C_V(q) = -\hat{z}\cdot(\hat{p}\times\hat{q})\,\hat{z}\cdot(\hat{q}\times\hat{k})$ y nos queda:


\bea
&& \langle L_{AB} \rangle  =  2K_I\omega^8\,\frac{1}{2PI} \int_{q\leq Q}\,\frac{d^2q}{(2\pi)^2}\,  \exp{\left[-l^2_r(\mbp-\mbq)^2-l^2_r(\mbq-\mbki)^2\right]}\nn 
&&\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\sum_{\mu,\mu'}
\int\,dz_2\,\int\,dz'_2\,\rho(z_2-z'_2)\,\Theta_\mu(z_1,z_2)\,\Theta_{\mu'}(z'_1,z'_2) \nn
&& 
\left\lbrace |C_H(q)|^2\,\left(F^{D}_{A\,PII}F^\mu_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^{\mu'}_{H\,QII}\right)^*(z'_1)
\,\left(F^{\bar\mu}_{H\,QII}F^D_{B\,KII}\right)(z_2)\,\left(F^{\bar\mu'}_{H\,QII}F^D_{B\,KII}\right)^*(z'_2) \right.\nn
&&\left.+C_H(q)\,C^*_V(q)\,\left(F^{D}_{A\,PII}F^\mu_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^{\mu'}_{V\,QII}\right)^*(z'_1)
\,\left(F^{\bar\mu}_{H\,QII}F^D_{B\,KII}\right)(z_2)\,\left(F^{\bar\mu'}_{V\,QII}F^D_{B\,KII}\right)^*(z'_2) \right.\nn
&&\left.+C_V(q)\,C^*_H(q)\,\left(F^{D}_{A\,PII}F^\mu_{V\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^{\mu'}_{H\,QII}\right)^*(z'_1)
\,\left(F^{\bar\mu}_{V\,QII}F^D_{B\,KII}\right)(z_2)\,\left(F^{\bar\mu'}_{H\,QII}F^D_{B\,KII}\right)^*(z'_2) \right.\nn
&&\left.+|C_V(q)|^2\,\left(F^{D}_{A\,PII}F^\mu_{V\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^{\mu'}_{V\,QII}\right)^*(z'_1)
\,\left(F^{\bar\mu}_{V\,QII}F^D_{B\,KII}\right)(z_2)\,\left(F^{\bar\mu'}_{V\,QII}F^D_{B\,KII}\right)^*(z'_2) \right\rbrace \nonumber
\tea 

Ahora hay que expandir la suma en $\mu, \mu' =\{\text{UP},\text{DOWN}\} = \{ \UPa, \DWa\}$. Van a quedar 16 términos:

\bea
\langle L_{AB} \rangle = &&  I_{AB\,HH,\UPa\,\UPa} + I_{AB\,HH,\UPa\,\DWa} + I_{AB\,HH,\DWa\,\UPa} + I_{AB\,HH,\DWa\,\DWa} \nn
&&+  I_{AB\,HV,\UPa\,\UPa} + I_{AB\,HV,\UPa\,\DWa} + I_{AB\,HV,\DWa\,\UPa} + I_{AB\,HV,\DWa\,\DWa} \nn
&&+  I_{AB\,VH,\UPa\,\UPa} + I_{AB\,VH,\UPa\,\DWa} + I_{AB\,VH,\DWa\,\UPa} + I_{AB\,VH,\DWa\,\DWa} \nn
&&+  I_{AB\,VV,\UPa\,\UPa} + I_{AB\,VV,\UPa\,\DWa} + I_{AB\,VV,\DWa\,\UPa} + I_{AB\,VV,\DWa\,\DWa} \nonumber
\tea

Los términos $HV$ y $VH$ deberían ser iguales, así que en principio hay que calcular doce términos que conllevan integrales 6D. Además hay que considerar que esto es solo para el término Ladder, hay un análogo para el Cross. Entoces, para completar el canal $AB$ tenemos que hacer 24 integrales 6D. 

Veamos una de estas integrales. Tomemos el primero de los términos de la última igualdad. Cuando $\mu=\mu'=\text{UP}$ significa que las funciones escalón se prenden para $z_1 > z_2$ y para $z'_1 > z'_2$. Entonces nos queda:

\bea
&& I_{AB\,HH,\UPa\,\UPa} = 2K_I\omega^8\,\frac{1}{2PI} \int_{q\leq Q}\,\frac{d^2q}{(2\pi)^2}\,  \exp{\left[-l^2_r(\mbp-\mbq)^2-l^2_r(\mbq-\mbki)^2\right]}\nn 
&&\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\int^{z_1}_{-h}\,dz_2\,\int^{z'_1}_{-h}\,dz'_2\,\rho(z_2-z'_2) \nn
&& 
|C_H(q)|^2\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)^*(z'_1)
\,\left(F^\DWa_{H\,QII}F^D_{B\,KII}\right)(z_2)\,\left(F^\DWa_{H\,QII}F^D_{B\,KII}\right)^*(z'_2) \nonumber
\tea 

Reacomodamos:

\bea
&& I_{AB\,HH,\UPa\,\UPa} = 2K_I\omega^8\,\frac{1}{2PI} \int_{q\leq Q}\,\frac{d^2q}{(2\pi)^2}\,|C_H(q)|^2\,  \exp{\left[-l^2_r(\mbp-\mbq)^2-l^2_r(\mbq-\mbki)^2\right]}\nn 
&&\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)^*(z'_1)\nn
&& \int^{z_1}_{-h}\,dz_2\,\int^{z'_1}_{-h}\,dz'_2\,\rho(z_2-z'_2) \,\left(F^\DWa_{H\,QII}F^D_{B\,KII}\right)(z_2)\,\left(F^\DWa_{H\,QII}F^D_{B\,KII}\right)^*(z'_2) \nonumber
\tea 

Cada función $F$, que se propaga en la dirección $M$, tiene polarización $p$ y estaá evaluada en el mode $Q$, es de la forma: $F^M_{p\,Q} = f_{Mp}(Q)\,\left[r_{Mp}(Q)\,e^{\imath Q z}+t_{Mp}(Q)\,e^{-\imath Q z}\right]$. Así las cosas, llegamos a:

\bea
&& I_{AB\,HH,\UPa\,\UPa} = 2K_I\omega^8\,\frac{1}{2PI}\,|f_{\DWa\,B}(KII)|^2\, \int_{q\leq Q}\,\frac{d^2q}{(2\pi)^2}\,|C_H(q)|^2\,|f_{\DWa\,H}(QII)|^2\, \exp{\left[-l^2_r(\mbp-\mbq)^2-l^2_r(\mbq-\mbki)^2\right]}\nn 
&&\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)^*(z'_1)\nn
&& \int^{z_1}_{-h}\,dz_2\,\int^{z'_1}_{-h}\,dz'_2\,\rho(z_2-z'_2) \nn 
&&\left[ |r_{\DWa\,H}(QII)|^2\,e^{\imath QII(z_2-z'_2)}+r_{\DWa\,H}(QII)\,t^*_{\DWa\,H}(QII)\,e^{\imath QII(z_2+z'_2)}\right.\nn
&&\left. +t_{\DWa\,H}(QII)\,r^*_{\DWa\,H}(QII)\,e^{-\imath QII(z_2+z'_2)}+|t_{\DWa\,H}(QII)|^2\,e^{-\imath QII(z_2-z'_2)}\right]\nn
&&\left[ |r_{\DWa\,B}(KII)|^2\,e^{\imath KII(z_2-z'_2)}+r_{\DWa\,B}(KII)\,t^*_{\DWa\,B}(KII)\,e^{\imath KII(z_2+z'_2)}\right.\nn
&&\left. +t_{\DWa\,B}(KII)\,r^*_{\DWa\,B}(KII)\,e^{-\imath KII(z_2+z'_2)}+|t_{\DWa\,B}(KII)|^2\,e^{-\imath KII(z_2-z'_2)}\right]
\tea 


Las integrales en $z_2\,z'_2$ las hacemos tomando la aproximación $ \rho(z_2-z'_2) \sim L_2 \delta(z_2-z'_2)$, válida cuando $h\gg l_z$, donde $L_2$ es una longitud típica a determinar. Eliminamos la integral en $z'_2$ con la delta de Dirac y luego integramos en $z_2$. 

Llegamos a:

\bea
&& I_{AB\,HH,\UPa\,\UPa} = 2K_I\omega^8\,\frac{1}{2PI}\,|f_{\DWa\,B}(KII)|^2\, \int_{q\leq Q}\,\frac{d^2q}{(2\pi)^2}\,|C_H(q)|^2\,|f_{\DWa\,H}(QII)|^2\, \exp{\left[-l^2_r(\mbp-\mbq)^2-l^2_r(\mbq-\mbki)^2\right]}\nn 
&&\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)^*(z'_1)\nn
&& L_2\, \left\lbrace (H+z_1)\,\left[|r_{\DWa\,H}|^2+|t_{\DWa\,H}|^2 \right]\,\left[|r_{\DWa\,B}|^2+|t_{\DWa\,B}|^2 \right]\right.\nn
&&\left.+\frac{1}{2\imath KII}\left[|r_{\DWa\,H}|^2+|t_{\DWa\,H}|^2\right]\,
\left[r_{\DWa\,B}t^*_{\DWa\,B}\left(e^{2\imath KII\, z_1}-e^{-2\imath KII\,H}\right)-
t_{\DWa\,B}r^*_{\DWa\,B}\left(e^{-2\imath KII\, z_1}-e^{2\imath KII\,H}\right)\right] \right.\nn 
&&\left.+\frac{1}{2\imath QII}\left[|r_{\DWa\,B}|^2+|t_{\DWa\,B}|^2\right]\,
\left[r_{\DWa\,H}t^*_{\DWa\,H}\left(e^{2\imath QII\, z_1}-e^{-2\imath QII\,H}\right)-
t_{\DWa\,H}r^*_{\DWa\,H}\left(e^{-2\imath QII\, z_1}-e^{2\imath QII\,H}\right)\right]\right.\nn 
&&\left.+\frac{1}{2\imath(QII+KII)}\,
\left[r_{\DWa\,H}t^*_{\DWa\,H}\,r_{\DWa\,B}t^*_{\DWa\,B}\left(e^{2\imath(QII+KII)\, z_1}-e^{-2\imath(QII+KII)\,H}\right)\right.\right.\nn
&&\left.\left.-
t_{\DWa\,H}r^*_{\DWa\,H}\,t_{\DWa\,B}r^*_{\DWa\,B}\left(e^{-2\imath(QII+KII)\, z_1}-e^{2\imath (QII+KII)\,H}\right)\right]\right.\nn
&&\left.+\frac{1-\delta(QII-KII)}{2\imath(QII-KII)}\,
\left[r_{\DWa\,H}t^*_{\DWa\,H}\,t_{\DWa\,B}r^*_{\DWa\,B}\left(e^{2\imath(QII-KII)\, z_1}-e^{-2\imath(QII-KII)\,H}\right)\right.\right.\nn
&&\left.\left.-
t_{\DWa\,H}r^*_{\DWa\,H}\,r_{\DWa\,B}t^*_{\DWa\,B}\left(e^{-2\imath(QII-KII)\, z_1}-e^{2\imath (QII-KII)\,H}\right)\right] \right.\nn 
&&\left.+\delta(QII-KII)
(H+z_1)\left[r_{\DWa\,H}t^*_{\DWa\,H}\,t_{\DWa,B}r^*_{\DWa,B}+t_{\DWa\,H}r^*_{\DWa\,H}\,r_{\DWa,B}t^*_{\DWa,B} \right]\right\rbrace
\tea 

Volvemos a usar que $\rho(z_1-z'_1) ~ L_1\,\delta(z_1-z'_1)$. Desarrollamos el término $\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)^*(z_1)$ para que quede como una función Real explícita. Lo mismo con los términos que vienen de la integral en $z_2$. Después de mucho amasado llegamos a:


\bea
&& I_{AB\,HH,\UPa\,\UPa} = 2K_I\omega^8\,\frac{1}{2PI}\,|f_{\DWa\,A}(PII)|^2\,|f_{\DWa\,B}(KII)|^2\,L_1\,L_2 \nn 
&&\int_{q\leq Q}\,\frac{d^2q}{(2\pi)^2}\,|C_H(q)|^2\,|f_{\UPa\,H}(QII)|^2\,|f_{\DWa\,H}(QII)|^2\, \exp{\left[-l^2_r(\mbp-\mbq)^2-l^2_r(\mbq-\mbki)^2\right]}\nn 
&&\int^0_{-h}\,dz_1\, \left\lbrace |r_{\DWa\,A}|^2\,|r_{\UPa\,H}|^2 + |r_{\DWa\,A}|^2\,|t_{\UPa\,H}|^2 + 
|t_{\DWa\,A}|^2\,|r_{\UPa\,H}|^2 + |t_{\DWa\,A}|^2\,|t_{\UPa\,H}|^2 \right.\nn 
&&\left.+2|r_{\DWa\,A}|^2\,|r_{\UPa\,H}t^*_{\UPa\,H}|\,\cos\left[2QII\,z_1+\phi_1\right]
+2|t_{\DWa\,A}|^2\,|r_{\UPa\,H}t^*_{\UPa\,H}|\,\cos\left[2QII\,z_1+\phi_2\right]\right.\nn
&&\left.+2|r_{\UPa\,H}|^2\,|r_{\DWa\,A}t^*_{\DWa\,A}|\,\cos\left[2PII\,z_1+\phi_3\right]
+2|t_{\UPa\,H}|^2\,|r_{\DWa\,A}t^*_{\DWa\,A}|\,\cos\left[2PII\,z_1+\phi_4\right]\right.\nn
&&\left.+2|r_{\DWa\,A}t^*_{\DWa\,A}r_{\UPa\,H}t^*_{\UPa\,H}|\,\cos\left[2(PII+QII)z_1 +\phi_5\right]
+2|r_{\DWa\,A}t^*_{\DWa\,A}r^*_{\UPa\,H}t_{\UPa\,H}|\,\cos\left[2(PII-QII)z_1 +\phi_6\right]\right\rbrace\nn
&& \left\lbrace (H+z_1)\,\left[|r_{\DWa\,H}|^2+|t_{\DWa\,H}|^2 \right]\,\left[|r_{\DWa\,B}|^2+|t_{\DWa\,B}|^2 \right]\right.\nn
&&\left.+\frac{1}{KII}\left[|r_{\DWa\,H}|^2+|t_{\DWa\,H}|^2\right]\,
|r_{\DWa\,B}t^*_{\DWa\,B}|\left[\sin\left(2KII\,z_1+\phi_7\right)+\sin\left(2KII\,H-\phi_7\right)\right] \right.\nn 
&&\left.+\frac{1}{QII}\left[|r_{\DWa\,B}|^2+|t_{\DWa\,B}|^2\right]\,|r_{\DWa\,H}t^*_{\DWa\,H}|
\left[\sin\left(2QII\, z_1+\phi_8\right)+\sin\left(2QII\,H-\phi_8\right)\right]\right.\nn 
&&\left.+\frac{1}{(QII+KII)}\,|r_{\DWa\,H}t^*_{\DWa\,H}\,r_{\DWa\,B}t^*_{\DWa\,B}|
\left[\sin\left(2(QII+KII)\,z_1+\phi_9\right)+\sin\left(2(QII+KII)\,H-\phi_9\right)\right]\right.\nn
&&\left.+\frac{1-\delta(QII-KII)}{(QII-KII)}\,|r_{\DWa\,H}t^*_{\DWa\,H}\,t_{\DWa\,B}r^*_{\DWa\,B}|
\left[\sin\left(2(QII-KII)\,z_1+\phi_{10}\right)+\sin\left(2(QII-KII)\,H-\phi_{10}\right)\right]\right.\nn 
&&\left.+\delta(QII-KII)
(H+z_1)\,2\Re\{r_{\DWa\,H}t^*_{\DWa\,H}\,t_{\DWa,B}r^*_{\DWa,B}\}\right\rbrace
\tea 

\section{Fase estacionaria all' uso nostro}

Cada función $F$, que se propaga en la dirección $M$, tiene polarización $p$ y está evaluada en el mode $Q$, es de la forma: $F^M_{p\,Q} = f_{Mp}(Q)\,\left[r_{Mp}(Q)\,e^{\imath Q z}+t_{Mp}(Q)\,e^{-\imath Q z}\right]$. Así las cosas, llegamos a:

\bea
&& I_{AB\,HH,\UPa\,\UPa} = 2K_I\omega^8\,\frac{1}{2PI}\,|f_{\DWa\,B}(KII)|^2\, \int_{q\leq Q}\,\frac{d^2q}{(2\pi)^2}\,|C_H(q)|^2\,|f_{\DWa\,H}(QII)|^2\, \exp{\left[-l^2_r(\mbp-\mbq)^2-l^2_r(\mbq-\mbki)^2\right]}\nn 
&&\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)^*(z'_1)\nn
&& \int^{z_1}_{-h}\,dz_2\,\int^{z'_1}_{-h}\,dz'_2\,\rho(z_2-z'_2) \nn 
&&\left[ |r_{\DWa\,H}(QII)|^2\,e^{\imath QII(z_2-z'_2)}+r_{\DWa\,H}(QII)\,t^*_{\DWa\,H}(QII)\,e^{\imath QII(z_2+z'_2)}\right.\nn
&&\left. +t_{\DWa\,H}(QII)\,r^*_{\DWa\,H}(QII)\,e^{-\imath QII(z_2+z'_2)}+|t_{\DWa\,H}(QII)|^2\,e^{-\imath QII(z_2-z'_2)}\right]\nn
&&\left[ |r_{\DWa\,B}(KII)|^2\,e^{\imath KII(z_2-z'_2)}+r_{\DWa\,B}(KII)\,t^*_{\DWa\,B}(KII)\,e^{\imath KII(z_2+z'_2)}\right.\nn
&&\left. +t_{\DWa\,B}(KII)\,r^*_{\DWa\,B}(KII)\,e^{-\imath KII(z_2+z'_2)}+|t_{\DWa\,B}(KII)|^2\,e^{-\imath KII(z_2-z'_2)}\right]
\tea 
la hipótesis básica es que la integral está dominada por los términos que no oscilan, que sólo pueden provenir de

\bea
&& I_{AB\,HH,\UPa\,\UPa} = 2K_I\omega^8\,\frac{1}{2PI}\,|f_{\DWa\,B}(KII)|^2\, \int_{q\leq Q}\,\frac{d^2q}{(2\pi)^2}\,|C_H(q)|^2\,|f_{\DWa\,H}(QII)|^2\, \exp{\left[-l^2_r(\mbp-\mbq)^2-l^2_r(\mbq-\mbki)^2\right]}\nn 
&&\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)^*(z'_1)\nn
&& \int^{z_1}_{-h}\,dz_2\,\int^{z'_1}_{-h}\,dz'_2\,\rho(z_2-z'_2) \nn 
&&\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,e^{\imath \left(QII- KII\right)(z_2-z'_2)}+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\,e^{-\imath \left(QII- KII\right)(z_2-z'_2)}\right]
\tea 
Conviene separar el dominio de integración en dos triángulos

\be
I_{AB\,HH,\UPa\,\UPa} = 2K_I\omega^8\,\frac{1}{2PI}\,|f_{\DWa\,B}(KII)|^2\, \int_{q\leq Q}\,\frac{d^2q}{(2\pi)^2}\,|C_H(q)|^2\,|f_{\DWa\,H}(QII)|^2\, \exp{\left[-l^2_r(\mbp-\mbq)^2-l^2_r(\mbq-\mbki)^2\right]}\left[I_{sup}+I_{inf}\right]
\te

\bea
&&I_{sup}=\int^0_{-h}\,dz_1\,\int^{z_1}_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)^*(z'_1)\nn
&& \int^{z_1}_{-h}\,dz_2\,\int^{z'_1}_{-h}\,dz'_2\,\rho(z_2-z'_2) \nn 
&&\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,e^{\imath \left(QII- KII\right)(z_2-z'_2)}+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\,e^{-\imath \left(QII- KII\right)(z_2-z'_2)}\right]
\tea 

\bea
&&I_{inf}=I_{sup}^*=\int^0_{-h}\,dz'_1\,\int^{z'_1}_{-h}\,dz_1\,\rho(z_1-z'_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)^*(z'_1)\nn
&& \int^{z_1}_{-h}\,dz_2\,\int^{z'_1}_{-h}\,dz'_2\,\rho(z_2-z'_2) \nn 
&&\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,e^{\imath \left(QII- KII\right)(z_2-z'_2)}+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\,e^{-\imath \left(QII- KII\right)(z_2-z'_2)}\right]
\tea 
vamos a trabajar con $I_{sup}$. Descartamos la zona del integrando donde $z'_2<z'_1<z_2<z_1$ ya que allí el integrando es siempre oscilatorio. Por lo tanto

\bea
&&I_{sup}=\int^0_{-h}\,dz_1\,\int^{z_1}_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)^*(z'_1)\nn
&& \int^{z'_1}_{-h}\,dz_2\,\int^{z'_1}_{-h}\,dz'_2\,\rho(z_2-z'_2) \nn 
&&\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,e^{\imath \left(QII- KII\right)(z_2-z'_2)}+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\,e^{-\imath \left(QII- KII\right)(z_2-z'_2)}\right]
\tea 
Ahora definimos

\bea
u_2&=&z_2-z'_2\nn
v_2&=&\frac12\left(z_2+z'_2\right)
\tea
Es obvio que $dz_2dz'_2=du_2dv_2$ y que el integrando no depende de $v_2$. Tenemos que $-\left(h+z'_1\right)\le u_2\le z'_1+h$. Para un dado valor de $u_2$, 

\be
-h\le z'_2=v_2-\frac12u_2\le z'_1
\te 
y por lo tanto $u_2/2-h\le v_2\le u_2/2+z'_1$, pero también

\be
-h\le z_2=v_2+\frac12u_2\le z'_1
\te 
y entonces $-u_2/2-h\le v_2\le -u_2/2+z'_1$. Concluímos que 

\be
\frac12\left|u_2\right|-h\le v_2\le z'_1-\frac12\left|u_2\right|
\te
y entonces 
\bea
&&I_{sup}=\int^0_{-h}\,dz_1\,\int^{z_1}_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)^*(z'_1)\nn
&& \int^{h+z'_1}_{-h-z'_1}\,du_2\,\rho(u_2) \left(h+z'_1-\left|u_2\right|\right)\nn 
&&\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,e^{\imath \left(QII- KII\right)u_2}+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\,e^{-\imath \left(QII- KII\right)u_2}\right]
\tea 
Asumiendo que $\rho\left(u_2\right)$ es par

\bea
&&I_{sup}=2\int^0_{-h}\,dz_1\,\int^{z_1}_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)^*(z'_1)\nn
&&\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\right]\int^{h+z'_1}_{0}\,du_2\,\rho(u_2) \left(h+z'_1-u_2\right)\cos\left[{\left(QII- KII\right)u_2}\right]\nn
\tea 
Supongamos para fijar ideas que

\be
\rho(u_2) =\frac{L_2}{\sqrt{2\pi}\ell}e^{-u_2^2/2\ell^2}
\te
que converge a $L_2\delta\left(u_2\right)$ cuando $\ell\to 0$. Es coherente con lo que venimos haciendo aproximar

\bea
\int^{h+z'_1}_{0}\,du_2\,\rho(u_2) \left(h+z'_1-u_2\right)\cos\left[{\left(QII- KII\right)u_2}\right]&\approx&\left(h+z'_1\right)\int^{\infty}_{0}\,du_2\,\rho(u_2) \cos\left[{\left(QII- KII\right)u_2}\right]\nn
&=&\frac12L_2\left(h+z'_1\right)e^{-\left(QII- KII\right)^2\ell^2/2}
\tea
hasta ahora tenemos que

\bea 
I_{sup}&=&L_2\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\right]e^{-\left(QII- KII\right)^2\ell^2/2}\nn
&&\int^0_{-h}\,dz_1\,\int^{z_1}_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)^*(z'_1)\left(h+z'_1\right)
\tea
y ahora volvemos a usar que

\be
F^M_{p\,Q} = f_{Mp}(Q)\,\left[r_{Mp}(Q)\,e^{\imath Q z}+t_{Mp}(Q)\,e^{-\imath Q z}\right]
\te


\bea 
I_{sup}&=&L_2\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\right]e^{-\left(QII- KII\right)^2\ell^2/2}\nn
&&\left|f_{DA}(PII)\right|^2\left|f_{\UPa H}(QII)\right|^2\int^0_{-h}\,dz_1\,\int^{z_1}_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\left(h+z'_1\right)\nn
&&\left[r_{DA}(PII)\,e^{\imath PII z_1}+t_{DA}(PII)\,e^{-\imath PII z_1}\right]\left[r_{\UPa H}(QII)\,e^{\imath QII z_1}+t_{\UPa H}(QII)\,e^{-\imath QII z_1}\right]\nn
&&\left[r^*_{DA}(PII)\,e^{-\imath PII z'_1}+t^*_{DA}(PII)\,e^{\imath PII z'_1}\right]\left[r^*_{\UPa H}(QII)\,e^{-\imath QII z'_1}+t^*_{\UPa H}(QII)\,e^{\imath QII z'_1}\right]
\tea
Como antes, nos quedamos con los términos que exhiben puntos de fase estacionaria tanto en las integrales en $z$ como en $Q$

\bea 
I_{sup}&=&L_2\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\right]e^{-\left(QII- KII\right)^2\ell^2/2}\nn
&&\left|f_{DA}(PII)\right|^2\left|f_{\UPa H}(QII)\right|^2\int^0_{-h}\,dz_1\,\int^{z_1}_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\left(h+z'_1\right)\nn
&&\left[r_{DA}(PII)t_{\UPa H}(QII)\,e^{\imath \left(PII-QII\right) z_1}+t_{DA}(PII)r_{\UPa H}(QII)\,e^{-\imath \left(PII-QII\right) z_1}\right]\nn
&&\left[r^*_{DA}(PII)t^*_{\UPa H}(QII)\,e^{-\imath \left(PII-QII\right) z'_1}+t^*_{DA}(PII)r^*_{\UPa H}(QII)\,e^{\imath \left(PII-QII\right) z'_1}\right]
\tea

\bea 
&&I_{sup}=L_2\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\right]e^{-\left(QII- KII\right)^2\ell^2/2}\nn
&&\left|f_{DA}(PII)\right|^2\left|f_{\UPa H}(QII)\right|^2\int^0_{-h}\,dz_1\,\int^{z_1}_{-h}\,dz'_1\,\rho(z_1-z'_1)\,\left(h+z'_1\right)\nn
&&\left[\left|r_{DA}(PII)\right|^2\left|t_{\UPa H}(QII)\right|^2\,e^{\imath \left(PII-QII\right) \left(z_1-z'_1\right)}+\left|t_{DA}(PII)\right|^2\left|r_{\UPa H}(QII)\right|^2\,e^{-\imath \left(PII-QII\right) \left(z_1-z'_1\right)}\right]
\tea
Como antes, cambiamos variables a

\bea
u_1&=&z_1-z'_1\nn
v_1&=&\frac12\left(z_1+z'_1\right)
\tea
Entonces $0\le u_1\le h$

\bea
&&-h\le v_1+\frac12u_1\le 0\nn
&&-h\le v_1-\frac12u_1\le v_1+\frac12u_1
\tea
o sea que $u_1/2-h\le v_1\le -u_1/2$

\bea 
&&I_{sup}=L_2\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\right]e^{-\left(QII- KII\right)^2\ell^2/2}\nn
&&\left|f_{DA}(PII)\right|^2\left|f_{\UPa H}(QII)\right|^2\int^h_{0}\,du_1\,\rho(u_1)\nn
&&\left[\left|r_{DA}(PII)\right|^2\left|t_{\UPa H}(QII)\right|^2\,e^{\imath \left(PII-QII\right) \left(u_1\right)}+\left|t_{DA}(PII)\right|^2\left|r_{\UPa H}(QII)\right|^2\,e^{-\imath \left(PII-QII\right) \left(u_1\right)}\right]\nn
&&\int_{u_1/2-h}^{-u_1/2}dv_1\,\left(h+v_1-\frac12u_1\right)
\tea
Como antes, asumimos que la integral está dominada por el entorno de $u_1=0$

\bea 
&&I_{sup}=\frac12h^2L_2\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\right]e^{-\left(QII- KII\right)^2\ell^2/2}\nn
&&\left|f_{DA}(PII)\right|^2\left|f_{\UPa H}(QII)\right|^2\left[\left|r_{DA}(PII)\right|^2\left|t_{\UPa H}(QII)\right|^2\,J+\left|t_{DA}(PII)\right|^2\left|r_{\UPa H}(QII)\right|^2\,J^*\right]\nn
\tea
donde 

\bea 
J&=&\int^{\infty}_{0}\,du_1\,\rho(u_1)\;e^{\imath \left(PII-QII\right) \left(u_1\right)}\nn
&=&\frac12L_2e^{-\ell^2\left(PII-QII\right)^2/2}
\tea
El resultado final es 

\bea 
&&I_{sup}=I_{inf}=\frac14h^2L^2_2\left|f_{DA}(PII)\right|^2\left|f_{\UPa H}(QII)\right|^2\left[\left|r_{DA}(PII)\right|^2\left|t_{\UPa H}(QII)\right|^2+\left|t_{DA}(PII)\right|^2\left|r_{\UPa H}(QII)\right|^2\right]\nn
&&\left[ |r_{\DWa\,H}(QII)|^2\,|t_{\DWa\,B}(KII)|^2\,+|t_{\DWa\,H}(QII)|^2\,|r_{\DWa\,B}(KII)|^2\right]e^{-\left[\left(QII- KII\right)^2+\left(PII-QII\right)^2\right]\ell^2/2}
\tea
Todavía falta evaluar la integral en $Q$.



% Los dos últimos renglones son una manera bruta de escribir que cuando $QII\neq KII$ vale el término oscilatorio en $z_1$ y cuando $QII = KII$ vale el término lineal en $z_1$.

% Ahora hay que integrar en $z_1 \,z'_1$. Habíamos dicho de tomar el límite $h\rightarrow -\infty$ para llegar a transformadas de Fourier de $\rho(z_1-z'_1)$. Pero el término $\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)(z_1)\,\left(F^{D}_{A\,PII}F^\UPa_{H\,QII}\right)^*(z'_1)$ jode bastante a tales fines. Primero habría que hacer un cambio de variables pero no se logra desacoplar el producto de funciones, siempre queda una integral por hacer. Que no quiero hacer.

% Mi propuesta es volver a tomar $\rho(z_1-z'_1)\sim \delta(z_1-z'_1)$, llegar así a una integral en tres dimensiones, $d^2q\,dz$ y ahí mandarlo derecho viejo a la compu. ¿Purgatorio?


\begin{figure}
    \centering
    \includegraphics[scale=1.5]{figures/purgatorio.jpg}
    \caption{Asombrados, Dante y Virgilio observan como algunos de los sufrientes en el Aqueronte han logrado (¿cómo? nadie sabe) alcanzar las llanuras ascendentes del purgatorio. Sálvenos, oh bienaventurados, claman desde las aguas no tan hostiles. Los poetas, sin embargo, continuan su imperturbable ascenso.}
    \label{fig:my_label}
\end{figure}


% Si hacemos el producto entre los dos corchetes salen 16 términos, con todas las combinaciones posibles de $\pm QII \pm KII$.

% Hasta acá, puro amasado. Ahora viene lo feo. Primero, para hacer las integrales en $dz_2\,dz'_2$ creo que es conveniente hacer un cambio de variables tipo $r=z_2-z'_2\,;\,s=z_2$. Después viene la integral en sí. De forma cerrada no sale, por el factor $\rho(z_2-z'_2)$. En el caso en que $R = \pm QII \pm KII \neq 0$ me convencí de que la integral la podemos aproximar como $\rho(x)/(\imath R)\,e^{\imath R x}$ evaluando en los extremos que corresponda a $x$. Cuando $R = \pm QII \pm KII = 0$ desarrollo $\rho(x)$ a segundo orden e integro a mano. Entonces reducimos en dos dimensiones la integral. Pero ahora hay $16\times 2$ términos luego del primer par de integrales, que dependen de $z_1$ y $z'_1$. Y todavía falta expandir el producto de las $F$ evaluadas en $z_1$ y $z'_1$, volver a acomodar el ingtegrando y volver a integrar usando las mismas aproximaciones. Si no me equivoco, habrá del orden de 64 términos para, finalmente, integrar de manera numérica en $d^2q$. 

% \bigskip
% \bigskip

% \textit{Conclusiones de verano:} 

% \begin{itemize}
%     \item Si no me equivoqué, para cada canal $AB$ hay entonces $2\times12\times64 = 1536$ términos a integrar de manera numérica.
%     \item Honestamente, no creo poder hacer esto sin equvicarme ni en el desarrollo algebraico ni en la implementación numérica.
%     \item Honestamente, no creo tener ganas de hacer todo esto de esta manera.
% \end{itemize}

% \bigskip

% Todo esto me recuerda a aquel que se atrevió a cruzar el Aqueronte y, ya siendo tarde para arrepentirse, dijo:

% \medskip

% Y después de haber puesto su mano en la mia con rostro alegre, que me reanimó, me introdujo en medio de las cosas secretas. Alli, bajo un cielo sin estrellas, resonaban suspiros, quejas y profundos gemidos, de suerte que al escucharlos comencé a llorar. Diversas lenguas, horribles blasfemias, palabras de dolor, acentos de ira, voces altas y roncas, acompañadas de palmadas, producian un tumulto que va rodando siempre por aquel espacio eternamente oscuro, como la arena impelida por un torbellino. Yo, que estaba horrorizado, dije:

% - Maestro, ¿qué es lo que oigo, y qué gente es ésa, que parece doblegada por el dolor?

% Me respondió:

% - Esta miserable suerte está reservada a las tristes almas de aquellos que vivieron sin merecer alabanzas ni vituperio; están confundidas entre el perverso coro de los ángeles que no fueron rebeldes ni fieles a Dios, sino que sólo vivieron para si. El Cielo los lanzó de su seno por no ser menos hermoso, pero el profundo Infierno no quiere recibirlos por la gloria que con ello podrían reportar los demás culpables.

% Y yo repuse:

% - Maestro, ¿qué cruel dolor les hace lamentarse tanto?

% A lo que me contestó:

% - Te lo diré brevemente. Éstos no esperan morir; y su ceguedad es tanta, que se muestran envidiosos de cualquier otra suerte. El mundo no conserva ningún recuerdo suyo; la misericordia y la justicia los desdeñan: no hablemos más de ellos, míralos y pasa adelante.


% \begin{figure}
%     \centering
%     \includegraphics[width = \textwidth]{figures/aqueronte.jpg}
%     \caption{Aquellos que quisieron integrar en seis dimensiones 1536 términos oscilatorios. Dante y Virgilio los observan sin sentir pena ni misericordia. Culpa de ellos por atreverse a tanto.}
% \end{figure}






















% A note for Oscar:

% \bea
% && \langle |S^{(2)}_{rs}(z)|^2 \rangle \propto
%  \int\,\frac{d^2q}{(2\pi)^2}\,\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz_2\,\int^0_{-h}\,dz'_1\,\int^0_{-h}\,dz'_2\,\sum_{\mu,m}\,\,\sum_{\mu',m'}\,\,\mathcal{C}^{\mu,m;\mu',m'}_{L,\mbp\,\mbq}(z1-z'_1,z_2-z'_2) \nn
% && \propto \int_{q^2\leq \epsilon_1 k^2_i}\,\frac{d^2q}{(2\pi)^2}\,\int^0_{-h}\,dz_1\,\int^0_{-h}\,dz_2\,\int^0_{-h}\,dz'_1\,\int^0_{-h}\,dz'_2\nn
% && \exp{\left(-(\mbp-\mbq)^2(z_1-z'_1)^2\right)}\,\exp{\left(-(\mbq-\mbki)^2(z_2-z'_2)^2\right)}\,\frac{1}{QII}\left[\left(\hat{p}\cdot\hat{q}\right)\,\left(\hat{q}\cdot\hat{k}_i\right)\right]^2\nn
% &&\left[R(PII)\,e^{\imath PII z_1}+ T(PII)\,e^{-\imath PII z_1} \right] \,\,\left[R(QII)\,e^{\imath QII z_1}+T(QII)\,e^{-\imath QII z_1} \right]
% \nn
% && \left[r(QII)\,e^{\imath QII z_2}+t(QII)\,e^{-\imath QII z_2} \right]\,
% \left[R(KII)\,e^{\imath KII z_2}+ T(KII)\,e^{-\imath KII z_2} \right]\,\Theta(z_1-z_2) \nn
% &&\left[R(PII)\,e^{\imath PII z'_1}+ T(PII)\,e^{-\imath PII z'_1} \right]^* \,\left[R(QII)\,e^{\imath QII z'_1}+T(QII)\,e^{-\imath QII z'_1} \right]^*
% \nn 
% && \left[r(QII)\,e^{\imath QII z'_2}+t(QII)\,e^{-\imath QII z'_2} \right]^*\,
% \left[R(KII)\,e^{\imath KII z'_2}+ T(KII)\,e^{-\imath KII z'_2} \right]^*\,\Theta(z'_1-z'_2)
% \tea 


% $k_i = \frac{2\pi}{\lambda}$: numero de onda incidente;\\

% $KII = k_i\sqrt{1-\sin^2\theta_i}$: modo vertical en la dirección incidente dentro del medio dielectrico con fluctuaciones;\\

% $PII = k_i\,\sqrt{\epsilon_1 - \sin^2\theta_s}$, modo vertical en la dirección dispersada dentro del medio dielectrico con fluctuaciones;\\

% $QII = k_i\,\sqrt{\epsilon_1 - \sin^2\theta_q}$: modo auxiliar (a ser integrado). se puede integrar en cartesianas sobre $q^2_x + q^2_y \leq \epsilon_1\,k^2_i$ o bien en polares sobre $[q,\phi_q]:[0,\sqrt{\epsilon_1}k_i]\times[0,2\pi]$. El ángulo $\theta_q$ se calcula a partir del modulo  $q$ y el ángulo $\phi_q$.\\

% Los coeficientes $R,T$ o $r,t$ dependen de los modos verticale en donde estan evaluados. El factor dependiendo de $Q$ queda puesto de forma explicita delante de las exponenciales.





